Formalisation in Constructive Type Theory of Barendregt's Variable Convention for Generic Structures with Binders

We introduce a universe of regular datatypes with variable binding information, for which we define generic formation and elimination (i.e. induction /recursion) operators. We then define a generic alpha-equivalence relation over the types of the universe based on name-swapping, and derive iteration and induction principles which work modulo alpha-conversion capturing Barendregt's Variable Convention. We instantiate the resulting framework so as to obtain the Lambda Calculus and System F, for which we derive substitution operations and substitution lemmas for alpha-conversion and substitution composition. The whole work is carried out in Constructive Type Theory and machine-checked by the system Agda.

==> GenericProgramming/Alpha.tex <==
\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{Alpha} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{GPBindings}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Atom}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Swap}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Fresh}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Chi}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{FreeVariables}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{List.ListProperties}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{OccurBind}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Unit} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{setoid}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{unfold}\AgdaSymbol{;}\AgdaFunction{any}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.All}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.Any} \AgdaSymbol{as} \AgdaModule{any} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{tail}\AgdaSymbol{;}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{any.}\AgdaModule{Membership-≡}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaSymbol{as} \AgdaModule{PropEq} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]} \AgdaSymbol{to} \AgdaInductiveConstructor{[\_]ᵢ}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{PropEq.}\AgdaModule{≡-Reasoning} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{begin\_} \AgdaSymbol{to} \AgdaFunction{begin≡\_}\AgdaSymbol{;}\AgdaFunction{\_∎} \AgdaSymbol{to} \AgdaFunction{\_□}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary}\<%
\\
%
\\
%
\\
\>\AgdaComment{-- \{- Sorts matters -\}}\<%
\\
\>\AgdaComment{-- ∼data ∼α' (S : Sort)\{F : Functor\} : (G : Functor) → ⟦ G ⟧ (μ F) →  ⟦ G ⟧ (μ F) → Set where}\<%
\\
\>\AgdaComment{--   ∼αV    : \{n : V\}\{S' : Sort\}    → ∼α' S (|v| S') n      n}\<%
\\
\>\AgdaComment{--   ∼α1    :                         ∼α' S |1|      tt     tt}\<%
\\
\>\AgdaComment{--   ∼αE    : \{B : Set\}\{b : B\}      → ∼α' S (|E| B)  b      b}\<%
\\
\>\AgdaComment{--   ∼αEf   : \{G : Functor\}\{e e' : ⟦ G ⟧ (μ G)\}}\<%
\\
\>\AgdaComment{--          → ∼α' S G e e'          → ∼α' S (|Ef| G) (⟨ e ⟩) (⟨ e' ⟩)}\<%
\\
\>\AgdaComment{--   ∼αR    : \{e e' : ⟦ F ⟧ (μ F)\}     }\<%
\\
\>\AgdaComment{--          → ∼α' S F e e'          → ∼α' S |R|      (⟨ e ⟩) (⟨ e' ⟩)}\<%
\\
\>\AgdaComment{--   ∼αinj₁ : \{F₁ F₂ : Functor\}\{e e' : ⟦ F₁ ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--          → ∼α'  S F₁ e e'        → ∼α' S (F₁ |+| F₂) (inj₁ e) (inj₁ e')}\<%
\\
\>\AgdaComment{--   ∼αinj₂ : \{F₁ F₂ : Functor\}\{e e' : ⟦ F₂ ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--          → ∼α'  S F₂ e e'        → ∼α' S (F₁ |+| F₂) (inj₂ e) (inj₂ e')}\<%
\\
\>\AgdaComment{--   ∼αx    : \{F₁ F₂ : Functor\}\{e₁ e₁'  : ⟦ F₁ ⟧ (μ F)\}\{e₂ e₂'  : ⟦ F₂ ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--          → ∼α'  S F₁ e₁ e₁' → ∼α'  S F₂ e₂ e₂'}\<%
\\
\>\AgdaComment{--                                  → ∼α' S (F₁ |x| F₂) (e₁ , e₂) (e₁' , e₂')}\<%
\\
\>\AgdaComment{--   ∼αb≡S  : (xs : List V)\{a b : V\}\{G : Functor\}\{e e' : ⟦ G ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--          → ((c : V) → c ∉ xs → ∼α' S \{F\} G (swapF' F G S a c e) (swapF' F G S b c e')) }\<%
\\
\>\AgdaComment{--                                  → ∼α' S (|B| S G)   (a , e)   (b   , e')  }\<%
\\
\>\AgdaComment{--   ∼αb≢S  : \{S' : Sort\}\{a : V\}\{G : Functor\}\{e e' : ⟦ G ⟧ (μ F)\} → S ≢ S'           -- This is the only rule that Sort matters !}\<%
\\
\>\AgdaComment{--          → ∼α' S G e e'          → ∼α' S (|B| S' G)  (a , e)   (a   , e')  }\<%
\\
%
\\
\>\AgdaComment{-- ∼α : (S : Sort)\{F : Functor\} → μ F → μ F → Set}\<%
\\
\>\AgdaComment{-- ∼α S \{F\} ⟨ e ⟩ ⟨ e' ⟩ = ∼α' S F e e'}\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{10} \AgdaFunction{\_∼α\_}\<%
\end{code}

Sort independent

%<*alpha>
\begin{code}%
\>\AgdaKeyword{data} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \<[56]%
\>[56]\AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaPrimitiveType{Set} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼α1} \<[11]%
\>[11]\AgdaSymbol{:} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaInductiveConstructor{|1|} \<[55]%
\>[55]\AgdaInductiveConstructor{tt} \<[66]%
\>[66]\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αR} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \<[39]%
\>[39]\<%
\\
\>[4]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e'} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaInductiveConstructor{|R|} \<[55]%
\>[55]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[66]%
\>[66]\AgdaInductiveConstructor{⟨} \AgdaBound{e'} \AgdaInductiveConstructor{⟩}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αE} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{B} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}\{}\AgdaBound{b} \AgdaSymbol{:} \AgdaBound{B}\AgdaSymbol{\}} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{B}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{b} \<[66]%
\>[66]\AgdaBound{b}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αEf} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{G}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e'} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[66]%
\>[66]\AgdaInductiveConstructor{⟨} \AgdaBound{e'} \AgdaInductiveConstructor{⟩}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼α+₁} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{F₁} \AgdaBound{F₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F₁} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaDatatype{∼αF} \AgdaBound{F₁} \AgdaBound{e} \AgdaBound{e'} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaBound{F₁} \AgdaInductiveConstructor{|+|} \<[50]%
\>[50]\AgdaBound{F₂}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼α+₂} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{F₁} \AgdaBound{F₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F₂} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaDatatype{∼αF} \AgdaBound{F₂} \AgdaBound{e} \AgdaBound{e'} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaBound{F₁} \AgdaInductiveConstructor{|+|} \<[50]%
\>[50]\AgdaBound{F₂}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αx} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{F₁} \AgdaBound{F₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e₁} \AgdaBound{e₁'} \<[40]%
\>[40]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F₁} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{e₂} \AgdaBound{e₂'} \<[23]%
\>[23]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F₂} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[0]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaDatatype{∼αF} \AgdaBound{F₁} \AgdaBound{e₁} \AgdaBound{e₁'} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaBound{F₂} \AgdaBound{e₂} \AgdaBound{e₂'}\<%
\\
\>[11]\AgdaIndent{34}{}\<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaBound{F₁} \AgdaInductiveConstructor{|x|} \<[50]%
\>[50]\AgdaBound{F₂}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaBound{e₁'} \AgdaInductiveConstructor{,} \AgdaBound{e₂'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αV} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \<[66]%
\>[66]\AgdaBound{x} \<[101]%
\>[101]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{∼αB} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \<[14]%
\>[14]\AgdaSymbol{((}\AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{z} \AgdaFunction{∉} \AgdaBound{xs} \<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaBound{G} \<[44]%
\>[44]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e'}\AgdaSymbol{))} \<[82]%
\>[82]\<%
\\
\>[11]\AgdaIndent{34}{}\<[34]%
\>[34]\AgdaSymbol{→} \<[37]%
\>[37]\AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaBound{y} \<[71]%
\>[71]\AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{)} \<[78]%
\>[78]\<%
\\
%
\\
\>\AgdaFunction{\_∼α\_} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{\_∼α\_} \AgdaSymbol{=} \AgdaDatatype{∼αF} \AgdaInductiveConstructor{|R|}\<%
\end{code}
%</alpha>

\begin{code}%
\>\AgdaFunction{lemma-∼αEf} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{\}} \<[43]%
\>[43]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{F}\AgdaSymbol{)} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \<[75]%
\>[75]\AgdaBound{e′} \<[79]%
\>[79]\<%
\\
\>\AgdaFunction{lemma-∼αEf} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e′}\<%
\\
%
\\
\>\AgdaFunction{lemma-∼αR} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{F}\AgdaSymbol{)} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>\AgdaFunction{lemma-∼αR} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e′}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaComment{-- terminates as the induction is over functor G, no necessary length induction !!!!!}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{z}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaInductiveConstructor{∼αV} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaBound{e∼e'} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaBound{e∼e'}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[67]%
\>[67]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{B}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaBound{e∼e'} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaBound{e∼e'}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \<[67]%
\>[67]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{F₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[67]%
\>[67]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \<[95]%
\>[95]\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{F₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[67]%
\>[67]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \<[95]%
\>[95]\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{F₁} \AgdaInductiveConstructor{|x|} \AgdaBound{F₂}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e'} \AgdaBound{e∼e''}\AgdaSymbol{)} \<[55]%
\>[55]\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[67]%
\>[67]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e''} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{.\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \<[59]%
\>[59]\AgdaSymbol{.\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[83]%
\>[83]\<%
\\
\>[13]\AgdaIndent{37}{}\<[37]%
\>[37]\AgdaBound{x} \AgdaBound{y} \<[41]%
\>[41]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{S}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{.\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \<[59]%
\>[59]\AgdaSymbol{.\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[83]%
\>[83]\<%
\\
\>[2]\AgdaIndent{37}{}\<[37]%
\>[37]\AgdaBound{x} \AgdaBound{y} \<[41]%
\>[41]\<%
\\
\> \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[13]%
\>[13]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \<[32]%
\>[32]\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∉x∷y∷xs} \AgdaSymbol{→} \AgdaFunction{subst₂} \<[43]%
\>[43]\AgdaSymbol{(}\AgdaDatatype{∼αF} \AgdaBound{G}\AgdaSymbol{)} \<[51]%
\>[51]\<%
\\
\>[19]\AgdaIndent{43}{}\<[43]%
\>[43]\AgdaSymbol{(}\AgdaFunction{trans} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \<[84]%
\>[84]\<%
\\
\>[43]\AgdaIndent{51}{}\<[51]%
\>[51]\AgdaSymbol{(}\AgdaFunction{cong} \<[58]%
\>[58]\AgdaSymbol{(λ} \AgdaBound{w} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{a}\AgdaSymbol{)} \AgdaBound{w} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))} \<[111]%
\>[111]\<%
\\
\>[51]\AgdaIndent{58}{}\<[58]%
\>[58]\AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢a} \AgdaBound{c∉x∷y∷xs} \AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{c∉x∷y∷xs}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{43}{}\<[43]%
\>[43]\AgdaSymbol{(}\AgdaFunction{trans} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \<[84]%
\>[84]\<%
\\
\>[43]\AgdaIndent{51}{}\<[51]%
\>[51]\AgdaSymbol{(}\AgdaFunction{cong} \<[58]%
\>[58]\AgdaSymbol{(λ} \AgdaBound{w} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{b}\AgdaSymbol{)} \AgdaBound{w} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e'}\AgdaSymbol{))} \<[112]%
\>[112]\<%
\\
\>[51]\AgdaIndent{58}{}\<[58]%
\>[58]\AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢a} \AgdaBound{c∉x∷y∷xs} \AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{c∉x∷y∷xs}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{43}{}\<[43]%
\>[43]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d∉xs} \AgdaBound{c∉x∷y∷xs}\AgdaSymbol{))} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{.\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \<[59]%
\>[59]\AgdaSymbol{.\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[83]%
\>[83]\<%
\\
\>[0]\AgdaIndent{37}{}\<[37]%
\>[37]\AgdaBound{x} \AgdaBound{y} \<[41]%
\>[41]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \<[13]%
\>[13]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∉xs} \AgdaSymbol{→} \AgdaFunction{subst₂} \<[42]%
\>[42]\AgdaSymbol{(}\AgdaDatatype{∼αF} \AgdaBound{G}\AgdaSymbol{)} \<[50]%
\>[50]\<%
\\
\>[2]\AgdaIndent{42}{}\<[42]%
\>[42]\AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)} \<[81]%
\>[81]\<%
\\
\>[2]\AgdaIndent{42}{}\<[42]%
\>[42]\AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)} \<[81]%
\>[81]\<%
\\
\>[2]\AgdaIndent{42}{}\<[42]%
\>[42]\AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{c∉xs}\AgdaSymbol{)} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaFunction{lemma∼swapEquiv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \<[16]%
\>[16]\AgdaBound{e} \AgdaFunction{∼α} \<[22]%
\>[22]\AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{∼α} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼swapEquiv} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaFunction{lemma∼swapEquivF} \<[56]%
\>[56]\AgdaBound{e∼e'} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma∼+B} \AgdaSymbol{:} \<[12]%
\>[12]\AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)} \<[120]%
\>[120]\<%
\\
\>\AgdaFunction{lemma∼+B} \AgdaSymbol{\{}\AgdaArgument{a} \AgdaSymbol{=} \AgdaBound{a}\AgdaSymbol{\}} \AgdaBound{e∼e'} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaInductiveConstructor{[]} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{\_} \AgdaSymbol{→} \AgdaFunction{lemma∼swapEquivF} \AgdaBound{e∼e'} \AgdaBound{a} \AgdaBound{c}\AgdaSymbol{)} \<[68]%
\>[68]\<%
\\
%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Reflexive} \<[34]%
\>[34]\AgdaSymbol{(}\AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[36]%
\>[36]\AgdaFunction{ρF}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \AgdaFunction{ρF}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{x}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \AgdaFunction{ρF}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{y}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \AgdaFunction{ρF}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G} \AgdaInductiveConstructor{|x|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[36]%
\>[36]\AgdaFunction{ρF} \AgdaFunction{ρF}\<%
\\
\>\AgdaFunction{ρF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaInductiveConstructor{[]} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{\_} \AgdaSymbol{→} \AgdaFunction{lemma∼swapEquivF} \AgdaFunction{ρF} \AgdaBound{a} \AgdaBound{c}\AgdaSymbol{)} \<[72]%
\>[72]\<%
\\
%
\\
\>\AgdaFunction{ρ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Reflexive} \AgdaSymbol{(}\AgdaFunction{\_∼α\_} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{ρ} \AgdaSymbol{=} \AgdaFunction{ρF}\<%
\\
%
\\
\>\AgdaComment{-- automatically derived}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Symmetric} \<[34]%
\>[34]\AgdaSymbol{(}\AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaInductiveConstructor{∼αV} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{σF} \AgdaInductiveConstructor{∼α1} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{σF} \AgdaInductiveConstructor{∼αE} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \<[28]%
\>[28]\AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[28]%
\>[28]\AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[28]%
\>[28]\AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[28]%
\>[28]\AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e'} \AgdaBound{e∼e''}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[28]%
\>[28]\AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{e∼e''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{σF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{f}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∉xs} \AgdaSymbol{→} \AgdaFunction{σF} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{c∉xs}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaFunction{σ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Symmetric} \<[31]%
\>[31]\AgdaSymbol{(}\AgdaFunction{\_∼α\_} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{σ} \AgdaSymbol{=} \AgdaFunction{σF}\<%
\\
%
\\
\>\AgdaFunction{τF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Transitive} \AgdaSymbol{(}\AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaInductiveConstructor{∼αV} \<[21]%
\>[21]\AgdaInductiveConstructor{∼αV} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{τF} \AgdaInductiveConstructor{∼α1} \<[21]%
\>[21]\AgdaInductiveConstructor{∼α1} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{τF} \AgdaInductiveConstructor{∼αE} \<[21]%
\>[21]\AgdaInductiveConstructor{∼αE} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e'∼e''}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e'} \AgdaBound{e'∼e''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e'∼e''}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e'} \AgdaBound{e'∼e''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e'∼e''}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e'} \AgdaBound{e'∼e''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e'∼e''}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e'} \AgdaBound{e'∼e''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e'} \AgdaBound{e∼e''}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e'∼e''} \AgdaBound{e'∼e'''}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e'} \AgdaBound{e'∼e''}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{τF} \AgdaBound{e∼e''} \AgdaBound{e'∼e'''}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{τF} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{f}\AgdaSymbol{)} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{ys} \AgdaBound{g}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{ys}\AgdaSymbol{)} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∉xsys} \AgdaSymbol{→} \AgdaFunction{τF} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{c∉xsys}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{g} \AgdaBound{c} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{c∉xsys}\AgdaSymbol{))} \AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{τ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Transitive} \AgdaSymbol{(}\AgdaFunction{\_∼α\_} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{τ} \AgdaSymbol{=} \AgdaFunction{τF}\<%
\\
%
\\
\>\AgdaKeyword{module} \AgdaModule{∼F-Reasoning} \AgdaSymbol{(}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≈-preorder} \AgdaSymbol{:} \AgdaRecord{Preorder} \AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≈-preorder} \AgdaSymbol{=} \<[16]%
\>[16]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaKeyword{record} \AgdaSymbol{\{} \<[22]%
\>[22]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{Carrier} \AgdaSymbol{=} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{);}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{\_≈\_} \AgdaSymbol{=} \AgdaDatatype{\_≡\_}\AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{\_∼\_} \AgdaSymbol{=} \AgdaDatatype{∼αF} \AgdaBound{G}\AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{isPreorder} \AgdaSymbol{=} \<[27]%
\>[27]\AgdaKeyword{record} \AgdaSymbol{\{}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{isEquivalence} \AgdaSymbol{=} \AgdaField{Relation.Binary.Setoid.isEquivalence} \AgdaSymbol{(}\AgdaFunction{setoid} \AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)))} \AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{reflexive} \AgdaSymbol{=} \AgdaSymbol{λ} \AgdaSymbol{\{} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{M}\AgdaSymbol{\}} \AgdaInductiveConstructor{refl} \AgdaSymbol{→} \AgdaFunction{ρF}\AgdaSymbol{\};}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{trans} \AgdaSymbol{=} \AgdaFunction{τF} \AgdaSymbol{\}} \AgdaSymbol{\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{import} \AgdaModule{Relation.Binary.PreorderReasoning} \AgdaSymbol{as} \AgdaModule{PreR}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{PreR} \AgdaFunction{≈-preorder} \AgdaKeyword{public}\<%
\\
%
\\
\>\AgdaKeyword{module} \AgdaModule{∼-Reasoning} \AgdaSymbol{(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≈-preorder} \AgdaSymbol{:} \AgdaRecord{Preorder} \AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≈-preorder} \AgdaSymbol{=} \<[16]%
\>[16]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaKeyword{record} \AgdaSymbol{\{} \<[22]%
\>[22]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{Carrier} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{\_≈\_} \AgdaSymbol{=} \AgdaDatatype{\_≡\_}\AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{\_∼\_} \AgdaSymbol{=} \AgdaFunction{\_∼α\_}\AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{isPreorder} \AgdaSymbol{=} \<[27]%
\>[27]\AgdaKeyword{record} \AgdaSymbol{\{}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{isEquivalence} \AgdaSymbol{=} \AgdaField{Relation.Binary.Setoid.isEquivalence} \AgdaSymbol{(}\AgdaFunction{setoid} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{;}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{reflexive} \AgdaSymbol{=} \AgdaSymbol{λ} \AgdaSymbol{\{} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{M}\AgdaSymbol{\}} \AgdaInductiveConstructor{refl} \AgdaSymbol{→} \AgdaFunction{ρ}\AgdaSymbol{\};}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaField{trans} \AgdaSymbol{=} \AgdaFunction{τ} \AgdaSymbol{\}} \AgdaSymbol{\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{import} \AgdaModule{Relation.Binary.PreorderReasoning} \AgdaSymbol{as} \AgdaModule{PreR}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{PreR} \AgdaFunction{≈-preorder} \AgdaKeyword{public}\<%
\\
%
\\
\>\AgdaKeyword{mutual}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[2]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[2]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{z\#e} \AgdaBound{y\#e} \<[61]%
\>[61]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{z\#e} \AgdaBound{x\#e} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin} \<[13]%
\>[13]\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \<[43]%
\>[43]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdemComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{⟩} \<[44]%
\>[44]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaFunction{⟩} \<[32]%
\>[32]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{x} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where} \AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaBound{z\#e} \AgdaBound{y\#e} \<[57]%
\>[57]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z} \<[78]%
\>[78]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x\#e} \AgdaBound{y\#e} \<[58]%
\>[58]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[78]%
\>[78]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin} \<[13]%
\>[13]\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)} \<[43]%
\>[43]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}))} \AgdaFunction{⟩} \<[62]%
\>[62]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where} \AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaBound{z\#e} \AgdaBound{y\#e} \<[57]%
\>[57]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z} \<[87]%
\>[87]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{y\#e} \AgdaSymbol{\_} \<[56]%
\>[56]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin} \<[13]%
\>[13]\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \<[43]%
\>[43]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{⟩} \<[38]%
\>[38]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where} \AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaBound{z\#e} \AgdaBound{y\#e} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢} \AgdaBound{z≢e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢} \AgdaBound{y≢e}\AgdaSymbol{)} \<[82]%
\>[82]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[120]%
\>[120]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐcancel} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{y≢e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{z≢e}\AgdaSymbol{)))} \AgdaFunction{ρF}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢} \AgdaBound{z≢e}\AgdaSymbol{)} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢S} \AgdaBound{S≢S}\AgdaSymbol{)} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢S} \AgdaBound{S≢S}\AgdaSymbol{)} \<[57]%
\>[57]\AgdaBound{y\#e} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaBound{z\#e} \<[57]%
\>[57]\AgdaBound{y\#e} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaFunction{ρF}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaBound{z\#e} \<[57]%
\>[57]\AgdaBound{y\#e} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshR} \AgdaBound{z\#e}\AgdaSymbol{)} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaInductiveConstructor{freshR} \AgdaBound{y\#e}\AgdaSymbol{)} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[122]%
\>[122]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{A}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaBound{z\#e} \<[57]%
\>[57]\AgdaBound{y\#e} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaBound{z\#e}\AgdaSymbol{)} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaBound{y\#e}\AgdaSymbol{)} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \<[122]%
\>[122]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaBound{z\#e}\AgdaSymbol{)} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaBound{y\#e}\AgdaSymbol{)} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[122]%
\>[122]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaBound{z\#e}\AgdaSymbol{)} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaBound{y\#e}\AgdaSymbol{)} \<[76]%
\>[76]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[122]%
\>[122]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{F₁} \AgdaInductiveConstructor{|x|} \AgdaBound{F₂}\AgdaSymbol{\}} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaBound{z\#e₁} \AgdaBound{z\#e₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaBound{y\#e₁} \AgdaBound{y\#e₂}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[114]%
\>[114]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[122]%
\>[122]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e₁} \AgdaBound{y\#e₁}\AgdaSymbol{)} \<[271]%
\>[271]\AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e₂} \AgdaBound{y\#e₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \AgdaBound{y\#we} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaInductiveConstructor{freshb≡} \<[62]%
\>[62]\AgdaBound{y\#we} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \<[114]%
\>[114]\AgdaSymbol{=} \<[117]%
\>[117]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \<[62]%
\>[62]\AgdaInductiveConstructor{freshb≡} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \<[114]%
\>[114]\AgdaSymbol{=} \<[117]%
\>[117]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#e}\AgdaSymbol{)} \<[62]%
\>[62]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \<[112]%
\>[112]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \AgdaBound{y\#we} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#xe} \AgdaBound{y\#xe} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠x} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≠x} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[18]%
\>[18]\AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{z} \<[30]%
\>[30]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{...} \<[18]%
\>[18]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{z≠z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{z≠z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{...} \<[18]%
\>[18]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[27]%
\>[27]\AgdaSymbol{=} \AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelFƛ} \AgdaBound{z\#xe} \AgdaBound{y\#xe}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \AgdaBound{y\#we} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#ze} \AgdaInductiveConstructor{freshb≡} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[93]%
\>[93]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[122]%
\>[122]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≠y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#ze} \AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[133]%
\>[133]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin} \<[13]%
\>[13]\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \<[69]%
\>[69]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \<[11]%
\>[11]\AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡b} \AgdaBound{x} \AgdaBound{z} \AgdaBound{z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[96]%
\>[96]\AgdaFunction{⟩} \<[98]%
\>[98]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \<[58]%
\>[58]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \<[11]%
\>[11]\AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaBound{x≠z} \AgdaBound{x≠y}\AgdaSymbol{)} \<[86]%
\>[86]\AgdaFunction{⟩} \<[88]%
\>[88]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \<[47]%
\>[47]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaInductiveConstructor{∼αB} \<[15]%
\>[15]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{lemmaAux} \AgdaFunction{⟩} \<[50]%
\>[50]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{y≠z}\AgdaSymbol{)))} \<[89]%
\>[89]\AgdaFunction{⟩} \<[91]%
\>[91]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where} \<[10]%
\>[10]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{lemmaAux} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{u} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{u∉xyzfve} \AgdaSymbol{:} \AgdaBound{u} \AgdaFunction{∉} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{lemmaAux} \AgdaBound{u} \AgdaBound{u∉xyfve} \<[23]%
\>[23]\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{=} \<[9]%
\>[9]\AgdaFunction{begin}\<%
\\
\>[6]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{X}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaBound{x≠z} \AgdaBound{x≠y}\AgdaSymbol{)} \<[113]%
\>[113]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[53]%
\>[53]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡a} \AgdaBound{z} \AgdaBound{y} \AgdaBound{z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[99]%
\>[99]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[53]%
\>[53]\AgdaBound{y} \<[70]%
\>[70]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{x}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \<[70]%
\>[70]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \<[69]%
\>[69]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡a} \AgdaBound{x} \AgdaBound{u} \AgdaBound{x} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[114]%
\>[114]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{u∉xyfve}\AgdaSymbol{)))} \<[133]%
\>[133]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[40]%
\>[40]\AgdaBound{y} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \<[72]%
\>[72]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{u} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{u} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{u} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \<[53]%
\>[53]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢a} \AgdaBound{u∉xyfve}\AgdaSymbol{))} \AgdaBound{x≠y}\AgdaSymbol{)} \<[139]%
\>[139]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{u} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡a} \AgdaBound{u} \AgdaBound{y} \AgdaBound{u} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[99]%
\>[99]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[40]%
\>[40]\AgdaBound{y} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{X}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[40]%
\>[40]\AgdaBound{y} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{y\#e} \AgdaFunction{u\#e}\AgdaSymbol{)} \AgdaBound{x} \AgdaBound{y} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \<[40]%
\>[40]\AgdaBound{y} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{y≠z}\AgdaSymbol{))} \<[111]%
\>[111]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \<[39]%
\>[39]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{u}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢a} \AgdaBound{u∉xyfve}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{u∉xyfve}\AgdaSymbol{))} \<[120]%
\>[120]\AgdaFunction{⟩}\<%
\\
\>[10]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{u\#e} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{u} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{u\#e} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{u}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d∉xs} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{u∉xyfve}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \AgdaBound{y\#we} \<[70]%
\>[70]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}} \<[49]%
\>[49]\AgdaInductiveConstructor{freshb≡} \<[62]%
\>[62]\AgdaBound{y\#ye} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[88]%
\>[88]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≠y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#e}\AgdaSymbol{)} \AgdaBound{y\#ye} \<[70]%
\>[70]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \<[11]%
\>[11]\AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠y}\AgdaSymbol{)} \AgdaBound{y≠z}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \<[21]%
\>[21]\AgdaBound{y} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡b} \AgdaBound{z} \AgdaBound{y} \AgdaBound{y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaBound{z} \<[35]%
\>[35]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaInductiveConstructor{∼αB} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{lemmaAux} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaBound{x} \<[35]%
\>[35]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[59]%
\>[59]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡b} \AgdaBound{x} \AgdaBound{y} \AgdaBound{y} \AgdaInductiveConstructor{refl}\AgdaSymbol{))} \AgdaFunction{⟩} \<[81]%
\>[81]\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{y} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[58]%
\>[58]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎} \<[15]%
\>[15]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{lemmaAux} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{u} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{u∉xyfve} \AgdaSymbol{:} \AgdaBound{u} \AgdaFunction{∉} \AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{lemmaAux} \AgdaBound{u} \AgdaBound{u∉xyfve} \<[23]%
\>[23]\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{=} \<[9]%
\>[9]\AgdaFunction{begin}\<%
\\
\>[6]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡a} \AgdaBound{z} \AgdaBound{u} \AgdaBound{z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaBound{y≠z} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{u∉xyfve}\AgdaSymbol{)))} \AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[37]%
\>[37]\AgdaBound{y} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaFunction{u\#e}\AgdaSymbol{)} \AgdaBound{u} \AgdaBound{y} \AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[37]%
\>[37]\AgdaBound{y} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d≢b} \AgdaBound{u∉xyfve}\AgdaSymbol{))))} \<[121]%
\>[121]\AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \<[37]%
\>[37]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{)} \<[70]%
\>[70]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≡a} \AgdaBound{x} \AgdaBound{u} \AgdaBound{x} \AgdaInductiveConstructor{refl}\AgdaSymbol{))} \<[101]%
\>[101]\AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{u} \AgdaFunction{）ₐ} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{)} \<[69]%
\>[69]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{≈⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{⟩}\<%
\\
\>[9]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{u\#e} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{u} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{u\#e} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{u}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{d∉ab∷xs→d∉xs} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{u∉xyfve}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaInductiveConstructor{freshb≡} \<[61]%
\>[61]\AgdaBound{y\#we} \<[78]%
\>[78]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{z≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{z≠z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaBound{z\#we} \<[61]%
\>[61]\AgdaInductiveConstructor{freshb≡} \<[78]%
\>[78]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[132]%
\>[132]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≠y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \<[78]%
\>[78]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠w} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≠y}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{=} \<[6]%
\>[6]\AgdaFunction{begin}\<%
\\
\>[3]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≈⟨} \<[10]%
\>[10]\AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠w}\AgdaSymbol{)} \AgdaBound{w≠z}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \<[20]%
\>[20]\AgdaBound{w} \<[33]%
\>[33]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaBound{w≠z} \AgdaBound{w≠y}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{w} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{w} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[58]%
\>[58]\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaBound{X} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐc≢a∧c≢b} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≠w}\AgdaSymbol{)} \AgdaBound{w≠y}\AgdaSymbol{))} \AgdaFunction{⟩} \<[88]%
\>[88]\<%
\\
\>[6]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{w} \<[33]%
\>[33]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[57]%
\>[57]\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaBound{S'} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[65]%
\>[65]\<%
\\
\>[2]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaBound{z\#xe} \AgdaBound{y\#xe} \<[64]%
\>[64]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'} \<[17]%
\>[17]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \<[56]%
\>[56]\AgdaInductiveConstructor{freshb≡} \<[70]%
\>[70]\AgdaBound{y\#xe} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#xe}\AgdaSymbol{)} \AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#e}\AgdaSymbol{)} \<[70]%
\>[70]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaInductiveConstructor{freshb≡} \<[70]%
\>[70]\AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{X} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{ρF}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{.\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaInductiveConstructor{freshb≡} \<[70]%
\>[70]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{X}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{ρF}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#xe}\AgdaSymbol{)} \AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{subst₂} \AgdaSymbol{(λ} \AgdaBound{X} \AgdaBound{Y} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{X} \AgdaBound{Y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}))} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\})} \AgdaFunction{ρF}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼swapCancelFƛ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[56]%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{z\#e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemma∼swapCancelF} \AgdaBound{z\#e} \AgdaBound{y\#e}\<%
\\
%
\\
%
\\
%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e'}\<%
\\
\>[4]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{x} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[4]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{x} \AgdaBound{G} \AgdaBound{e'}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaInductiveConstructor{∼αV} \<[26]%
\>[26]\AgdaBound{x\#e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaBound{x\#e}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaInductiveConstructor{∼α1} \<[26]%
\>[26]\AgdaBound{x\#e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaBound{x\#e}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaInductiveConstructor{∼αE} \<[26]%
\>[26]\AgdaBound{x\#e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaBound{x\#e}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaBound{x\#e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{freshEf} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e'} \AgdaBound{x\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{freshR} \AgdaBound{x\#e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{freshR} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e'} \AgdaBound{x\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaBound{x\#e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{freshinj₁} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e'} \AgdaBound{x\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaBound{x\#e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{freshinj₂} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e'} \AgdaBound{x\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e'} \AgdaBound{e∼e''}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaBound{x\#e} \AgdaBound{x\#e₁}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{freshx} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e'} \AgdaBound{x\#e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaBound{e∼e''} \AgdaBound{x\#e₁}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[8]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[49]%
\>[49]\AgdaBound{x\#ye} \AgdaKeyword{with} \<[60]%
\>[60]\AgdaBound{S'} \AgdaFunction{≟S} \AgdaBound{S} \<[68]%
\>[68]\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[8]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[49]%
\>[49]\AgdaInductiveConstructor{freshb≡} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S'≠S} \AgdaSymbol{=} \<[77]%
\>[77]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S'≠S} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[8]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[49]%
\>[49]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S'≠S} \<[74]%
\>[74]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{χ'} \AgdaBound{xs} \AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaBound{xs}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{u} \AgdaSymbol{|} \AgdaBound{u∉xs}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{freshb} \AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#≢S→} \AgdaBound{S'≠S} \AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{u} \<[48]%
\>[48]\AgdaBound{u∉xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#≢S←} \AgdaBound{S'≠S} \AgdaBound{x\#e}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[52]%
\>[52]\AgdaBound{x\#ye} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[52]%
\>[52]\AgdaBound{x\#ye} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[52]%
\>[52]\AgdaBound{x\#ye} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaInductiveConstructor{freshb≡} \<[117]%
\>[117]\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[52]%
\>[52]\AgdaBound{x\#ye} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠z} \<[103]%
\>[103]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{χ'} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{xs} \AgdaFunction{++} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{xs} \AgdaFunction{++} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{u} \AgdaSymbol{|} \AgdaBound{u∉yxs}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{freshb} \AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#≢→} \<[27]%
\>[27]\AgdaBound{y≠z} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{u∉yxs}\AgdaSymbol{))} \<[57]%
\>[57]\<%
\\
\>[2]\AgdaIndent{27}{}\<[27]%
\>[27]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \<[38]%
\>[38]\AgdaSymbol{(}\AgdaBound{f} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b∉xs} \AgdaBound{u∉yxs}\AgdaSymbol{)))} \<[80]%
\>[80]\<%
\\
\>[27]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#} \AgdaSymbol{(}\AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaBound{xs}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b∉xs} \AgdaBound{u∉yxs}\AgdaSymbol{))))))}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y}\AgdaSymbol{\}} \<[33]%
\>[33]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[52]%
\>[52]\AgdaInductiveConstructor{freshb≡} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≠y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≠y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \<[32]%
\>[32]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \<[32]%
\>[32]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaInductiveConstructor{freshb≡}\<%
\\
\>\AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \<[32]%
\>[32]\<%
\\
\>[0]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{f}\AgdaSymbol{)} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[64]%
\>[64]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≠z} \<[93]%
\>[93]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{χ'} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{z} \AgdaInductiveConstructor{∷} \AgdaBound{xs} \AgdaFunction{++} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{z} \AgdaInductiveConstructor{∷} \AgdaBound{xs} \AgdaFunction{++} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{u} \AgdaSymbol{|} \AgdaBound{u∉}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{freshb} \AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#≢→} \<[27]%
\>[27]\AgdaBound{x≠z} \<[31]%
\>[31]\<%
\\
\>[2]\AgdaIndent{27}{}\<[27]%
\>[27]\AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{u∉}\AgdaSymbol{))} \<[50]%
\>[50]\<%
\\
\>[2]\AgdaIndent{27}{}\<[27]%
\>[27]\AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaSymbol{(}\AgdaFunction{d∉abc∷xs→d∉xs} \AgdaBound{u∉}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaFunction{lemmaSwapF\#≢←} \AgdaBound{x≠y} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{u∉}\AgdaSymbol{))} \AgdaBound{x\#e}\AgdaSymbol{)))} \<[129]%
\>[129]\<%
\\
%
\\
%
\\
%
\\
\>\AgdaFunction{lemma∼B} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼B} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{f}\AgdaSymbol{)} \AgdaBound{z\#xe} \<[57]%
\>[57]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{χ'} \AgdaSymbol{(}\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{u} \AgdaSymbol{|} \AgdaBound{u∉fvxe++xs} \<[22]%
\>[22]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin} \<[11]%
\>[11]\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e} \<[23]%
\>[23]\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{σF} \AgdaSymbol{(}\AgdaFunction{lemma∼swapCancelFƛ} \AgdaFunction{u\#xe} \AgdaBound{z\#xe}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{z} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{u} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{u} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)\}} \AgdaBound{u∉fvxe++xs}\AgdaSymbol{))} \AgdaBound{u} \AgdaBound{z} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{u} \AgdaBound{z} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{u} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapCancelFƛ} \AgdaFunction{u\#ye'} \AgdaFunction{z\#ye'} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e'}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎} \<[7]%
\>[7]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{u\#xe} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{u} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{u\#xe} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{u∉fvxe++xs}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{u\#ye'} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{u} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{u\#ye'} \AgdaSymbol{=} \AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{f}\AgdaSymbol{)} \AgdaFunction{u\#xe}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z\#ye'} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z\#ye'} \AgdaSymbol{=} \AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{f}\AgdaSymbol{)} \AgdaBound{z\#xe}\<%
\\
%
\\
\>\AgdaFunction{lemma∼Bswap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaBound{e′}\<%
\\
\>\AgdaFunction{lemma∼Bswap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{xe∼ye′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼B} \AgdaSymbol{\{}\AgdaArgument{x} \AgdaSymbol{=} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{xe∼ye′} \AgdaSymbol{(}\AgdaFunction{lemma∼\#F} \AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{xe∼ye′}\AgdaSymbol{)} \AgdaInductiveConstructor{freshb≡}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{y} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\})} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma∼+Brec} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{a} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>\AgdaFunction{lemma∼+Brec} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaBound{ae\textasciitilde{}ae′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{a} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼Bswap} \AgdaBound{ae\textasciitilde{}ae′} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>\<%
\end{code}

%<*lemafoldmapfalpha>
\begin{code}%
\>\AgdaFunction{lemma-foldmapfα} \<[17]%
\>[17]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{\{}\AgdaBound{f} \AgdaBound{f'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \<[18]%
\>[18]\AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \<[28]%
\>[28]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f'} \AgdaBound{e'}\AgdaSymbol{)} \<[70]%
\>[70]\<%
\\
\>[0]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \<[18]%
\>[18]\AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaBound{f'} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaInductiveConstructor{|1|} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{p} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{F} \<[31]%
\>[31]\AgdaBound{p} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE} \<[50]%
\>[50]\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{ρF} \<[49]%
\>[49]\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[25]%
\>[25]\AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{G₁} \<[31]%
\>[31]\AgdaBound{p} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[25]%
\>[25]\AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{G₂} \<[31]%
\>[31]\AgdaBound{p} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[25]%
\>[25]\AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{G₁} \<[31]%
\>[31]\AgdaBound{p} \AgdaBound{e₁}\AgdaSymbol{)} \<[37]%
\>[37]\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{G₂} \<[31]%
\>[31]\AgdaBound{p} \AgdaBound{e₂}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapfα} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \<[25]%
\>[25]\AgdaBound{G}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{p} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaInductiveConstructor{[]} \AgdaSymbol{(λ} \AgdaBound{y} \AgdaBound{\_} \AgdaSymbol{→} \AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{(}\AgdaFunction{lemma-foldmapfα} \AgdaBound{G} \AgdaBound{p} \AgdaBound{e}\AgdaSymbol{)} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)}\<%
\end{code}
%</lemafoldmapfalpha>


%<*lemma-foldfalpha>
\begin{code}%
\>\AgdaFunction{lemma-fold-alpha} \<[18]%
\>[18]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{f} \AgdaBound{f'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \<[26]%
\>[26]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f'} \AgdaBound{e'}\AgdaSymbol{)} \<[68]%
\>[68]\<%
\\
\>[2]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{fold} \AgdaBound{F} \AgdaBound{f} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{fold} \AgdaBound{F} \AgdaBound{f'} \AgdaBound{e}\<%
\end{code}
%</lemma-foldfalpha>

\begin{code}%
\>\AgdaFunction{lemma-fold-alpha} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{p} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{lemma-foldmapfα} \AgdaInductiveConstructor{|R|} \AgdaBound{p} \AgdaBound{e}\<%
\end{code}
-- lemma-foldmapSCtx  : {F H C : Functor}(G : Functor){f : μ C → ⟦ F ⟧ (μ H) → μ H}{c c′ : μ C}
--               → ({e e′ :  ⟦ F ⟧ (μ H)}{c c′ : μ C} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)               
--               → c ∼α c′
--               → (e : ⟦ G ⟧ (μ F)) → ∼αF G (foldmapCtx F G f c e) (foldmapCtx F G f c′ e)
-- lemma-foldmapSCtx (|v| S)      prf c∼c′  e          = ∼αV
-- lemma-foldmapSCtx |1|          prf c∼c′  e          = ∼α1
-- lemma-foldmapSCtx {F} |R|      prf c∼c′  ⟨ e ⟩      = prf c∼c′ (lemma-foldmapSCtx F prf c∼c′ e)
-- lemma-foldmapSCtx (|E| x)      prf c∼c′  e          = ∼αE 
-- lemma-foldmapSCtx (|Ef| G)     prf c∼c′  e          = ρF 
-- lemma-foldmapSCtx (G₁ |+| G₂)  prf c∼c′  (inj₁ e)   = ∼α+₁  (lemma-foldmapSCtx G₁ prf c∼c′  e)
-- lemma-foldmapSCtx (G₁ |+| G₂)  prf c∼c′  (inj₂ e)   = ∼α+₂  (lemma-foldmapSCtx G₂ prf c∼c′  e)
-- lemma-foldmapSCtx (G₁ |x| G₂)  prf c∼c′  (e₁ , e₂)  = ∼αx   (lemma-foldmapSCtx G₁ prf c∼c′  e₁) (lemma-foldmapSCtx G₂ prf c∼c′  e₂)
-- lemma-foldmapSCtx (|B| S G)    prf c∼c′  (x , e)    = ∼αB   [] (λ y y∉[] → lemma∼swapEquivF (lemma-foldmapSCtx G prf c∼c′  e) x y)


%<*lemmafoldCtxalphactx>
\begin{code}%
\>\AgdaFunction{lemma-foldCtx-alpha-Ctx} \<[25]%
\>[25]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaBound{C} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e′}\AgdaSymbol{)} \<[92]%
\>[92]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \<[16]%
\>[16]\AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-foldCtx-alpha-Ctx} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{f} \AgdaSymbol{=} \AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c′}\AgdaSymbol{\}} \AgdaBound{p} \AgdaBound{c∼c′} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{lemma-fold-alpha} \AgdaSymbol{(}\AgdaBound{p} \AgdaBound{c∼c′}\AgdaSymbol{)} \AgdaBound{e} \<[85]%
\>[85]\<%
\end{code}
%</lemmafoldCtxalphactx>

\begin{code}%
\>\AgdaFunction{lemma-B\#} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{G} \AgdaBound{e} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \<[120]%
\>[120]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-B\#} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{y\#e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaSymbol{(}\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(λ} \AgdaBound{z} \AgdaBound{z∉fve} \AgdaSymbol{→}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{begin}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapCancelF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{y\#e} \AgdaSymbol{(}\AgdaFunction{lemmafvSF\#} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{z∉fve}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma-B\#'} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{G} \AgdaBound{e} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-B\#'} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{y\#e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma-B\#} \AgdaBound{y\#e} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{x} \AgdaBound{G} \AgdaBound{e} \AgdaSymbol{→} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{G} \AgdaBound{e} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \<[129]%
\>[129]\AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{x\#e} \<[71]%
\>[71]\AgdaBound{y\#e} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshR} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshR} \AgdaBound{y\#e}\AgdaSymbol{)} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{A}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{x\#e} \<[71]%
\>[71]\AgdaBound{y\#e} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaBound{y\#e}\AgdaSymbol{)} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaBound{y\#e}\AgdaSymbol{)} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaBound{y\#e}\AgdaSymbol{)} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|x|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaBound{x\#e₁} \AgdaBound{x\#e₂}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaBound{y\#e₁} \AgdaBound{y\#e₂}\AgdaSymbol{)} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e₁} \AgdaBound{y\#e₁}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e₂} \AgdaBound{y\#e₂}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S′}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{x\#e} \<[71]%
\>[71]\AgdaBound{y\#e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{swapF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S′}\AgdaSymbol{)} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{|} \AgdaFunction{lemmaSwap\#Var} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{x\#e} \AgdaBound{y\#e}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{z} \AgdaSymbol{|} \AgdaInductiveConstructor{refl} \<[91]%
\>[91]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV} \<[97]%
\>[97]\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S′} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{x\#e} \<[71]%
\>[71]\AgdaBound{y\#e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{S′} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaInductiveConstructor{freshb≡} \AgdaBound{y\#e} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S} \<[95]%
\>[95]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S≢S} \<[95]%
\>[95]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S′} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \<[33]%
\>[33]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[95]%
\>[95]\AgdaSymbol{=} \AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaInductiveConstructor{freshb≡} \<[71]%
\>[71]\AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{z} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaFunction{lemma（aa）b≡b} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{z} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}))} \AgdaFunction{⟩} \<[67]%
\>[67]\<%
\\
\>[5]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where} \<[8]%
\>[8]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaInductiveConstructor{freshb≡} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{（} \AgdaBound{z} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaSymbol{|} \AgdaFunction{lemma（ab）a≡b} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \<[8]%
\>[8]\AgdaSymbol{.}\AgdaBound{y} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{lemma-B\#} \<[31]%
\>[31]\AgdaBound{y\#e}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaInductiveConstructor{freshb≡} \<[84]%
\>[84]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaSymbol{|} \AgdaFunction{lemma（ab）b≡a} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \<[8]%
\>[8]\AgdaSymbol{.}\AgdaBound{x} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{lemma-B\#'} \<[32]%
\>[32]\AgdaBound{x\#e}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）ₐ} \AgdaBound{z} \AgdaSymbol{|} \AgdaFunction{lemma∙ₐ} \AgdaBound{x} \AgdaBound{y} \AgdaBound{z}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[72]%
\>[72]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[97]%
\>[97]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{y} \AgdaSymbol{|} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{refl} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaFunction{lemma-B\#} \AgdaBound{y\#e}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[72]%
\>[72]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[96]%
\>[96]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{x} \AgdaSymbol{|} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{refl} \AgdaInductiveConstructor{,} \AgdaBound{z≢x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{refl}\AgdaSymbol{))} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaFunction{lemma-B\#'} \AgdaBound{x\#e}\<%
\\
\>\AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{x\#e}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{freshb} \AgdaBound{y\#e}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[96]%
\>[96]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{z} \AgdaSymbol{|} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{z≢x} \<[26]%
\>[26]\AgdaInductiveConstructor{,} \AgdaBound{z≢y} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{refl}\AgdaSymbol{))} \<[42]%
\>[42]\AgdaSymbol{=} \AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#F} \AgdaBound{x\#e} \AgdaBound{y\#e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\<%
\\
\>\AgdaFunction{lemma-swap\#} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{fresh} \AgdaBound{S} \AgdaBound{x} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{fresh} \AgdaBound{S} \AgdaBound{y} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-swap\#} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{lemma-swap\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}}\<%
\\
%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[4]\AgdaIndent{26}{}\<[26]%
\>[26]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{xs} \AgdaSymbol{→} \AgdaBound{y} \AgdaFunction{∉} \AgdaBound{xs}\<%
\\
\>[4]\AgdaIndent{26}{}\<[26]%
\>[26]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBindF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>[4]\AgdaIndent{26}{}\<[26]%
\>[26]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBindF} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-binds1}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaSymbol{\_\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-bindsE}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-bindsEf} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindF} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-binds+1} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-binds+2} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|x|} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{\}} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-binds×} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaBound{xs∉be}\AgdaSymbol{))} \AgdaSymbol{((}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaBound{xs∉be}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaSymbol{=} \AgdaFunction{lemma-bindsv}\<%
\\
\>\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S′} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaBound{xs∉be} \AgdaKeyword{with} \AgdaBound{S′} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemma-bindsB} \AgdaSymbol{(}\AgdaFunction{lemma∉swap} \AgdaBound{y∉ys} \AgdaBound{x∉xs} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{xs∉be}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemma-bindsB} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{xs∉be}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaBound{x∉xs} \AgdaBound{y∉ys} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaBound{xs∉be}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaComment{-- lemma-foldmapα  : \{F H C : Functor\}(G : Functor)\{f : μ C → ⟦ F ⟧ (μ H) → μ H\}\{c c' : μ C\}\{e e' : ⟦ G ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--                → (\{e e′ :  ⟦ F ⟧ (μ H)\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)}\<%
\\
\>\AgdaComment{--                → (\{c : μ C\}\{S : Sort\}\{x y : V\}\{e : ⟦ F ⟧ (μ H)\} → f (swap S x y c) (swapF F S x y e) ≡ swap S x y (f c e))}\<%
\\
\>\AgdaComment{--                → ListNotOccurBindF G (fv c)   e}\<%
\\
\>\AgdaComment{--                → ListNotOccurBindF G (fv c')  e'}\<%
\\
\>\AgdaComment{--                → c ∼α c'}\<%
\\
\>\AgdaComment{--                → ∼αF G e e'  }\<%
\\
\>\AgdaComment{--                → ∼αF G (foldmapCtx F G f c e) (foldmapCtx F G f c' e')}\<%
\\
\>\AgdaComment{-- lemma-foldmapα (|v| S)        prf \_ nb nb' \_    ∼αV         = ∼αV  }\<%
\\
\>\AgdaComment{-- lemma-foldmapα |1|            prf \_ nb nb' \_    ∼α1         = ∼α1 }\<%
\\
\>\AgdaComment{-- lemma-foldmapα \{F\} |R|        prf prf2  nb nb' c∼c' (∼αR e∼e')}\<%
\\
\>\AgdaComment{--   = prf c∼c' (lemma-foldmapα F prf prf2 (lemmalistNotOccurBindFR→ListNotOccurBindF nb) (lemmalistNotOccurBindFR→ListNotOccurBindF nb') c∼c' e∼e')  }\<%
\\
\>\AgdaComment{-- lemma-foldmapα (|E| x)        prf \_ nb nb' \_    ∼αE         = ρF }\<%
\\
\>\AgdaComment{-- lemma-foldmapα (|Ef| G)       prf \_ nb nb' \_    (∼αEf e∼e') = ∼αEf e∼e'}\<%
\\
\>\AgdaComment{-- lemma-foldmapα (G₁ |+| G₂)    prf prf2 nb nb' c∼c' (∼α+₁ e∼e')}\<%
\\
\>\AgdaComment{--   = ∼α+₁  (lemma-foldmapα G₁ prf prf2 (listNotOccurBinj₁inv nb) (listNotOccurBinj₁inv nb') c∼c' e∼e')  }\<%
\\
\>\AgdaComment{-- lemma-foldmapα (G₁ |+| G₂)    prf prf2 nb nb' c∼c' (∼α+₂ e∼e')}\<%
\\
\>\AgdaComment{--   = ∼α+₂  (lemma-foldmapα G₂ prf prf2 (listNotOccurBinj₂inv nb) (listNotOccurBinj₂inv nb') c∼c' e∼e') }\<%
\\
\>\AgdaComment{-- lemma-foldmapα (G₁ |x| G₂)    prf prf2 nb nb' c∼c' (∼αx α₁ α₂)}\<%
\\
\>\AgdaComment{--   = ∼αx   (lemma-foldmapα G₁ prf prf2 (listNotOccurBx₁inv nb) (listNotOccurBx₁inv nb') c∼c' α₁)}\<%
\\
\>\AgdaComment{--           (lemma-foldmapα G₂ prf prf2 (listNotOccurBx₂inv nb) (listNotOccurBx₂inv nb') c∼c' α₂)  }\<%
\\
\>\AgdaComment{-- lemma-foldmapα \{F\} \{H\} \{C\} (|B| S G) \{f\} \{c\} \{c'\}  \{y , e\} \{z , e'\}}\<%
\\
\>\AgdaComment{--                prf prf2 nb nb' c∼c' (∼αB xs fα)  }\<%
\\
\>\AgdaComment{--   = ∼αB  (fv c ++ fv c' ++ xs)}\<%
\\
\>\AgdaComment{--          (λ x x∉ → begin}\<%
\\
\>\AgdaComment{--                      swapF G S y x (foldmapCtx F G f c e)}\<%
\\
\>\AgdaComment{--                    ≈⟨ sym (lemmaSwapFoldSEquivF \{C\} \{H\} \{F\} \{G\} prf2)  ⟩}\<%
\\
\>\AgdaComment{--                      foldmapCtx F G f (swap S y x c) (swapF G S y x e)}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-foldmapSCtx G prf}\<%
\\
\>\AgdaComment{--                                         (lemma-swap\# (lemmafvF\# (listNotOccurBBinv∉fv nb)) (lemmafvF\# (c∉xs++ys→c∉xs x∉)))}\<%
\\
\>\AgdaComment{--                                         (swapF G S y x e) ⟩}\<%
\\
\>\AgdaComment{--                      foldmapCtx F G f c              (swapF G S y x e)}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-foldmapα  G prf prf2}\<%
\\
\>\AgdaComment{--                                       (lemma-swapListNotOccurBind (c∉xs++ys→c∉xs x∉) (listNotOccurBBinv∉fv nb) (listNotOccurBBinv nb))}\<%
\\
\>\AgdaComment{--                                       (lemma-swapListNotOccurBind (c∉xs++ys→c∉xs (c∉xs++ys→c∉ys \{xs = fv c\} x∉)) (listNotOccurBBinv∉fv nb') (listNotOccurBBinv nb'))}\<%
\\
\>\AgdaComment{--                                       c∼c'}\<%
\\
\>\AgdaComment{--                                       (fα x (c∉xs++ys→c∉ys \{xs = fv c'\} (c∉xs++ys→c∉ys \{xs = fv c\} x∉))) ⟩}\<%
\\
\>\AgdaComment{--                      foldmapCtx F G f c'             (swapF G S z x e')}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-foldmapSCtx  G prf (σ (lemma-swap\#  (lemmafvF\# (listNotOccurBBinv∉fv nb'))}\<%
\\
\>\AgdaComment{--                                                                 (lemmafvF\# (c∉xs++ys→c∉xs (c∉xs++ys→c∉ys \{xs = fv c\} x∉)))))}\<%
\\
\>\AgdaComment{--                                          (swapF G S z x e') ⟩}\<%
\\
\>\AgdaComment{--                      foldmapCtx F G f (swap S z x c') (swapF G S z x e')}\<%
\\
\>\AgdaComment{--                    ≈⟨ lemmaSwapFoldSEquivF \{C\} \{H\} \{F\} \{G\} prf2 ⟩}\<%
\\
\>\AgdaComment{--                      swapF G S z x (foldmapCtx F G f c' e')}\<%
\\
\>\AgdaComment{--                    ∎)}\<%
\\
\>\AgdaComment{--      where}\<%
\\
\>\AgdaComment{--      open ∼F-Reasoning(H)(G)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \<[16]%
\>[16]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaBound{C} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaBound{c'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \AgdaSymbol{→}\<%
\\
\>[2]\AgdaIndent{17}{}\<[17]%
\>[17]\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaFunction{ListNotOccurBindF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \<[34]%
\>[34]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaFunction{ListNotOccurBindF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c'}\AgdaSymbol{)} \<[34]%
\>[34]\AgdaBound{e'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c'} \<[14]%
\>[14]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e'} \<[28]%
\>[28]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c'}\AgdaSymbol{)} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaSymbol{\_} \AgdaBound{nb} \AgdaBound{nb'} \AgdaSymbol{\_} \<[48]%
\>[48]\AgdaInductiveConstructor{∼αV} \<[60]%
\>[60]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV} \<[67]%
\>[67]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaInductiveConstructor{|1|} \<[30]%
\>[30]\AgdaBound{prf} \AgdaSymbol{\_} \AgdaBound{nb} \AgdaBound{nb'} \AgdaSymbol{\_} \<[48]%
\>[48]\AgdaInductiveConstructor{∼α1} \<[60]%
\>[60]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1} \<[66]%
\>[66]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[30]%
\>[30]\AgdaBound{prf} \AgdaBound{prf2} \<[40]%
\>[40]\AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{prf} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaFunction{lemma-foldmapα} \AgdaBound{F} \AgdaBound{prf} \AgdaBound{prf2} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaBound{c∼c'} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[147]%
\>[147]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaSymbol{\_} \AgdaBound{nb} \AgdaBound{nb'} \AgdaSymbol{\_} \<[48]%
\>[48]\AgdaInductiveConstructor{∼αE} \<[60]%
\>[60]\AgdaSymbol{=} \AgdaFunction{ρF} \<[65]%
\>[65]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaSymbol{\_} \AgdaBound{nb} \AgdaBound{nb'} \AgdaSymbol{\_} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapα} \AgdaBound{G₁} \AgdaBound{prf} \AgdaBound{prf2} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaBound{c∼c'} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[103]%
\>[103]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapα} \AgdaBound{G₂} \AgdaBound{prf} \AgdaBound{prf2} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaBound{c∼c'} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[102]%
\>[102]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{α₁} \AgdaBound{α₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapα} \AgdaBound{G₁} \AgdaBound{prf} \AgdaBound{prf2} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaBound{c∼c'} \AgdaBound{α₁}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-foldmapα} \AgdaBound{G₂} \AgdaBound{prf} \AgdaBound{prf2} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaBound{c∼c'} \AgdaBound{α₂}\AgdaSymbol{)} \<[97]%
\>[97]\<%
\\
\>\AgdaFunction{lemma-foldmapα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{\{}\AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c'}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{\{}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}}\<%
\\
\>[10]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{fα}\AgdaSymbol{)} \<[49]%
\>[49]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \<[9]%
\>[9]\AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{c'} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(λ} \AgdaBound{x} \AgdaBound{x∉} \AgdaSymbol{→} \AgdaFunction{begin}\<%
\\
\>[9]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{≈⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{f} \AgdaSymbol{=} \AgdaSymbol{λ} \AgdaBound{y} \AgdaBound{x} \AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{c}\AgdaSymbol{)\}} \AgdaSymbol{\{}\AgdaArgument{g} \AgdaSymbol{=} \AgdaBound{f} \AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{prf2}\AgdaSymbol{)} \<[110]%
\>[110]\AgdaFunction{⟩}\<%
\\
\>[19]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{c}\AgdaSymbol{))} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{∼⟨} \AgdaFunction{lemma-foldmapfα} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{prf} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#} \AgdaSymbol{(}\AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{nb}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{x∉}\AgdaSymbol{))))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[19]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{x} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{∼⟨} \AgdaFunction{lemma-foldmapα} \<[38]%
\>[38]\AgdaBound{G} \AgdaBound{prf} \AgdaBound{prf2}\<%
\\
\>[19]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{x∉}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{nb}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaBound{nb}\AgdaSymbol{))}\<%
\\
\>[19]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaSymbol{(}\AgdaFunction{lemma-swapListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{x∉}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{nb'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaBound{nb'}\AgdaSymbol{))}\<%
\\
\>[19]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaBound{c∼c'}\<%
\\
\>[19]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaSymbol{(}\AgdaBound{fα} \AgdaBound{x} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaBound{c'}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{x∉}\AgdaSymbol{)))} \AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c'}\AgdaSymbol{)} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{∼⟨} \AgdaFunction{lemma-foldmapfα} \AgdaBound{G} \<[41]%
\>[41]\AgdaSymbol{(}\AgdaBound{prf} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemma-swap\#} \<[63]%
\>[63]\AgdaSymbol{(}\AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaBound{nb'}\AgdaSymbol{))}\<%
\\
\>[19]\AgdaIndent{63}{}\<[63]%
\>[63]\AgdaSymbol{(}\AgdaFunction{lemmafvF\#} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{x∉}\AgdaSymbol{))))))} \<[125]%
\>[125]\<%
\\
\>[0]\AgdaIndent{41}{}\<[41]%
\>[41]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaBound{e'}\AgdaSymbol{)} \<[61]%
\>[61]\AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaBound{c'}\AgdaSymbol{))} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{≈⟨} \AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{f} \AgdaSymbol{=} \AgdaSymbol{λ} \AgdaBound{z} \AgdaBound{x} \AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaBound{c'}\AgdaSymbol{)\}} \AgdaSymbol{\{}\AgdaArgument{g} \AgdaSymbol{=} \AgdaBound{f} \AgdaBound{c'}\AgdaSymbol{\}} \AgdaBound{prf2} \<[106]%
\>[106]\AgdaFunction{⟩}\<%
\\
\>[19]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{x} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c'}\AgdaSymbol{)} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaFunction{∎}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{H}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\end{code}

%<*lemmafoldCtxalpha>
\begin{code}%
\>\AgdaFunction{lemma-foldCtx-alpha} \<[21]%
\>[21]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaBound{C} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaBound{c'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \<[14]%
\>[14]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{S} \<[18]%
\>[18]\AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c'}\AgdaSymbol{)} \<[60]%
\>[60]\AgdaBound{e'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c'} \AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'} \AgdaSymbol{→} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c'} \AgdaBound{e'}\<%
\end{code}
%</lemmafoldCtxalpha>

\begin{code}%
\>\AgdaFunction{lemma-foldCtx-alpha} \AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaBound{e∼e'} \AgdaSymbol{=} \AgdaFunction{lemma-foldmapα} \AgdaInductiveConstructor{|R|} \AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{nb'} \AgdaBound{c∼c'} \AgdaBound{e∼e'} \<%
\end{code}

\begin{code}%
\>\AgdaKeyword{mutual}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaBound{e\textasciitilde{}e′} \<[67]%
\>[67]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \<[67]%
\>[67]\AgdaSymbol{=} \AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaBound{e\textasciitilde{}e′} \<[67]%
\>[67]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e′}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e′}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{\}} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{e₁′} \AgdaInductiveConstructor{,} \AgdaBound{e₂′}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e₁\textasciitilde{}e₁′} \AgdaBound{e₂\textasciitilde{}e₂′}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaFunction{\_++\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₁′}\AgdaSymbol{\}} \AgdaBound{e₁\textasciitilde{}e₁′}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e₂′}\AgdaSymbol{\}} \AgdaBound{e₂\textasciitilde{}e₂′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S′}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{e}\AgdaSymbol{\}} \<[56]%
\>[56]\AgdaInductiveConstructor{∼αV} \<[68]%
\>[68]\AgdaSymbol{=} \<[71]%
\>[71]\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S′} \AgdaBound{G}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{\}} \<[56]%
\>[56]\AgdaBound{xe∼ye′} \AgdaKeyword{with} \AgdaBound{S′} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{S′≢S} \<[18]%
\>[18]\AgdaSymbol{=} \AgdaFunction{lemmafvswapBF≢} \AgdaBound{S′≢S} \AgdaBound{xe∼ye′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaSymbol{.}\AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{\}} \<[56]%
\>[56]\AgdaBound{xe∼ye′} \<[63]%
\>[63]\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaInductiveConstructor{refl} \<[18]%
\>[18]\AgdaSymbol{=} \AgdaFunction{lemmafvswapBF} \AgdaBound{xe∼ye′}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF≢} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaBound{S′} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaBound{S′} \AgdaFunction{≢} \AgdaBound{S} \<[22]%
\>[22]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S′} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S′}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{S′≢S} \AgdaBound{xe\textasciitilde{}ye′} \AgdaSymbol{=} \<[65]%
\>[65]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{begin≡}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{lemma-swapfvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S′}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{S′≢S}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S′} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma∼Bswap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S′}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{xe\textasciitilde{}ye′}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{□}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \<[73]%
\>[73]\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e} \AgdaFunction{-} \AgdaBound{x} \AgdaDatatype{≡} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′} \AgdaFunction{-} \AgdaBound{y} \<[60]%
\>[60]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[34]%
\>[34]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′} \AgdaKeyword{with} \AgdaFunction{lemma∼\#F} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{σF} \AgdaBound{∼αBxeye′}\AgdaSymbol{)} \AgdaInductiveConstructor{freshb≡}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x}\AgdaSymbol{\}} \<[34]%
\>[34]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′} \AgdaSymbol{|} \AgdaInductiveConstructor{freshb≡} \<[69]%
\>[69]\AgdaSymbol{=} \<[71]%
\>[71]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{begin≡}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e} \<[24]%
\>[24]\AgdaFunction{-} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{-} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmafvα} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma∼+Brec} \AgdaBound{∼αBxeye′}\AgdaSymbol{))} \AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′} \AgdaFunction{-} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{□}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemmafvswapBF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[34]%
\>[34]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′} \AgdaSymbol{|} \AgdaInductiveConstructor{freshb} \AgdaBound{y\#e} \AgdaSymbol{=} \<[71]%
\>[71]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{begin≡}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e} \AgdaFunction{-} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{lemmafvswap-} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{y\#e} \AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{-} \AgdaBound{y}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaFunction{\_-\_}\AgdaSymbol{)} \AgdaSymbol{\{}\AgdaArgument{u} \AgdaSymbol{=} \AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemmafvα} \AgdaSymbol{(}\AgdaFunction{lemma∼Bswap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′}\AgdaSymbol{))} \AgdaInductiveConstructor{refl} \<[87]%
\>[87]\AgdaFunction{⟩} \<[93]%
\>[93]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e′} \AgdaFunction{-} \AgdaBound{y}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{□}\<%
\\
%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{:} \<[13]%
\>[13]\AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)} \<[27]%
\>[27]\<%
\\
\>[4]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>[4]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e′}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{\_} \<[54]%
\>[54]\AgdaBound{e\textasciitilde{}e′} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{\_} \<[54]%
\>[54]\AgdaBound{e\textasciitilde{}e′} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaSymbol{.(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{\_)}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaSymbol{.(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{\_)}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaSymbol{.(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{\_)}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaSymbol{.(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{\_)}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e\textasciitilde{}e′}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e\textasciitilde{}e′}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G} \AgdaInductiveConstructor{|x|} \AgdaBound{G₁}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₁′}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{e₂} \AgdaInductiveConstructor{,} \AgdaBound{e₂′}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e₁\textasciitilde{}e₁′} \AgdaBound{e₂\textasciitilde{}e₂′}\AgdaSymbol{)} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaFunction{\_++\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e₁\textasciitilde{}e₁′}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼fvF} \AgdaBound{xs} \AgdaBound{e₂\textasciitilde{}e₂′}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{e}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaSymbol{\_} \<[54]%
\>[54]\AgdaInductiveConstructor{∼αV} \<[75]%
\>[75]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{\}} \<[51]%
\>[51]\AgdaBound{xs} \AgdaBound{∼αBxeye′} \AgdaKeyword{with} \AgdaFunction{any} \AgdaSymbol{(}\AgdaFunction{\_≟S\_} \AgdaBound{S}\AgdaSymbol{)} \AgdaBound{xs}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S∈xs} \AgdaSymbol{=} \<[17]%
\>[17]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{begin≡}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{≡⟨} \AgdaFunction{lemma-swapfvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{S∈xs} \<[55]%
\>[55]\AgdaFunction{⟩}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{≡⟨} \AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{lemma∼Bswap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{□} \<[6]%
\>[6]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{S∉xs} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaFunction{\_++\_}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{(}\AgdaFunction{begin≡} \AgdaComment{-- analogous to previous proof}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{S} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{≡⟨} \AgdaFunction{lemma-swapfvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{here} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaFunction{⟩}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{S} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{≡⟨} \AgdaFunction{lemma∼fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{S} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼Bswap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[3]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{S} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e′}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{□}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmafvswapBF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e′}\AgdaSymbol{\}} \AgdaBound{∼αBxeye′}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma∼fv} \AgdaSymbol{:} \<[12]%
\>[12]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[3]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'}\<%
\\
\>[3]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaFunction{fv} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{fv} \AgdaBound{e'}\<%
\\
\>\AgdaFunction{lemma∼fv} \AgdaSymbol{=} \AgdaFunction{lemma∼fvF} \AgdaInductiveConstructor{[]}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaComment{--lemmafv-∉ : \{F : Functor\}\{S : Sort\}\{e : ⟦ F ⟧ (μ F)\}\{x y : V\} → x ≢ y → x ∉ fvF \{|B| S F\} S (y , e) → x ∉ fv \{F\} S ⟨ e ⟩}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaComment{-- lemma-foldSfv : \{C H : Functor\}\{F : Functor\}\{f : μ C → ⟦ F ⟧ (μ H) → μ H\}\{c : μ C\}\{e : μ F\}\{S : Sort\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaComment{--                 → fv (foldS F f c e) ⊆ fv c ++ fv e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\<%
\end{code}


==> GenericProgramming/AlphaInduction.tex <==
\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{AlphaInduction} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{GPBindings}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Alpha}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{OccurBind}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{FreeVariables}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Swap}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Fresh}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{List.ListProperties}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{List.NotInList}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Chi}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Function}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Unit}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.All}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.Any} \AgdaSymbol{as} \AgdaModule{Any} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{tail}\AgdaSymbol{;}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{Any.}\AgdaModule{Membership-≡}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]} \AgdaSymbol{to} \AgdaInductiveConstructor{[\_]ᵢ}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{:} \<[20]%
\>[20]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{e'} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBindF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaBound{e} \<[42]%
\>[42]\AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaFunction{lemma-bindsv}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaInductiveConstructor{|1|} \<[33]%
\>[33]\AgdaBound{xs} \AgdaBound{e} \<[42]%
\>[42]\AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaFunction{lemma-binds1}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaBound{e} \<[42]%
\>[42]\AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaFunction{lemma-bindsE}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \AgdaSymbol{(}\AgdaInductiveConstructor{accEf} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{Data.Product.map} \<[22]%
\>[22]\AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \<[28]%
\>[28]\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaFunction{lemma-bindsEf}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[33]%
\>[33]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \AgdaSymbol{(}\AgdaInductiveConstructor{accR} \AgdaBound{acce}\AgdaSymbol{)} \<[59]%
\>[59]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{Data.Product.map} \<[22]%
\>[22]\AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \<[28]%
\>[28]\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaFunction{lemma-bindsR}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{F} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₁} \AgdaBound{acce}\AgdaSymbol{)} \<[59]%
\>[59]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{Data.Product.map} \<[22]%
\>[22]\AgdaInductiveConstructor{inj₁} \<[27]%
\>[27]\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaFunction{lemma-binds+1} \<[36]%
\>[36]\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₂} \AgdaBound{acce}\AgdaSymbol{)} \<[59]%
\>[59]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{Data.Product.map} \<[22]%
\>[22]\AgdaInductiveConstructor{inj₂}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaFunction{lemma-binds+2} \<[36]%
\>[36]\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accx} \AgdaBound{acce₁} \AgdaBound{acce₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \<[8]%
\>[8]\AgdaFunction{bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e₁} \AgdaBound{acce₁} \AgdaSymbol{|} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e₂} \AgdaBound{acce₂}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{e₁′} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₁}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{e₂′} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaSymbol{(}\AgdaBound{e₁′} \AgdaInductiveConstructor{,} \AgdaBound{e₂′}\AgdaSymbol{)} \AgdaInductiveConstructor{,} \AgdaFunction{lemma-binds×} \AgdaBound{notOccur₁} \AgdaBound{notOccur₂}\<%
\\
\>\AgdaFunction{bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accB} \AgdaBound{facc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[38]%
\>[38]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{zs}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{χ'} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{z} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaBound{z∉xs++fv}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{Data.Product.map} \<[22]%
\>[22]\AgdaSymbol{(λ} \AgdaBound{e'} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{lemma-bindsB} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{z∉xs++fv}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facc} \AgdaBound{z}\AgdaSymbol{))}\<%
\end{code}

%<*bindersfreealphaelem>
\begin{code}%
\>\AgdaFunction{bindersFreeElem} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{e'} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e'}\AgdaSymbol{)}\<%
\end{code}
%</bindersfreealphaelem>

\begin{code}%
\>\AgdaFunction{bindersFreeElem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{(}\AgdaFunction{accF} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaBound{e} \AgdaBound{e'} \<[17]%
\>[17]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{acce} \AgdaSymbol{:} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{acce'} \AgdaSymbol{:} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce} \AgdaDatatype{≡} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e'} \AgdaBound{acce'}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{)} \<[36]%
\>[36]\AgdaBound{xs} \AgdaBound{e} \<[46]%
\>[46]\AgdaSymbol{.}\AgdaBound{e} \<[54]%
\>[54]\AgdaInductiveConstructor{∼αV} \<[67]%
\>[67]\AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaInductiveConstructor{|1|} \<[36]%
\>[36]\AgdaBound{xs} \AgdaSymbol{.}\AgdaInductiveConstructor{tt} \<[46]%
\>[46]\AgdaSymbol{.}\AgdaInductiveConstructor{tt} \<[54]%
\>[54]\AgdaInductiveConstructor{∼α1} \<[67]%
\>[67]\AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[36]%
\>[36]\AgdaBound{xs} \AgdaBound{e} \<[46]%
\>[46]\AgdaSymbol{.}\AgdaBound{e} \<[54]%
\>[54]\AgdaInductiveConstructor{∼αE} \<[67]%
\>[67]\AgdaSymbol{\_} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[36]%
\>[36]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[47]%
\>[47]\AgdaInductiveConstructor{⟨} \AgdaBound{e'} \AgdaInductiveConstructor{⟩} \<[59]%
\>[59]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{e∼e'}\AgdaSymbol{)} \<[72]%
\>[72]\AgdaSymbol{(}\AgdaInductiveConstructor{accEf} \AgdaBound{acce}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accEf} \AgdaBound{acce'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Data.Product.map} \<[29]%
\>[29]\AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaFunction{lemma-bindsEf}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'} \AgdaBound{acce} \AgdaBound{acce'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[36]%
\>[36]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[46]%
\>[46]\AgdaInductiveConstructor{⟨} \AgdaBound{e'} \AgdaInductiveConstructor{⟩} \<[54]%
\>[54]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accR} \AgdaBound{acce}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accR} \AgdaBound{acce'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Data.Product.map} \<[29]%
\>[29]\AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaFunction{lemma-bindsR}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{F} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'} \AgdaBound{acce} \AgdaBound{acce'}\AgdaSymbol{)} \<[63]%
\>[63]\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₁} \AgdaBound{acce}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₁} \AgdaBound{acce'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Data.Product.map} \<[29]%
\>[29]\AgdaInductiveConstructor{inj₁} \AgdaFunction{lemma-binds+1}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'} \AgdaBound{acce} \AgdaBound{acce'}\AgdaSymbol{)} \<[65]%
\>[65]\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaBound{e∼e'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₂} \AgdaBound{acce}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{acc+₂} \AgdaBound{acce'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Data.Product.map} \<[29]%
\>[29]\AgdaInductiveConstructor{inj₂} \AgdaFunction{lemma-binds+2}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'} \AgdaBound{acce} \AgdaBound{acce'}\AgdaSymbol{)} \<[65]%
\>[65]\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{e₁′} \AgdaInductiveConstructor{,} \AgdaBound{e₂′}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e₁∼e₁′} \AgdaBound{e₂∼e₂′}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accx} \AgdaBound{acce₁} \AgdaBound{acce₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accx} \AgdaBound{acce₁′} \AgdaBound{acce₂′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e₁} \AgdaBound{acce₁} \AgdaSymbol{|} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e₂} \AgdaBound{acce₂} \AgdaSymbol{|}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e₁′} \AgdaBound{acce₁′} \AgdaSymbol{|} \AgdaFunction{bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e₂′} \AgdaBound{acce₂′} \AgdaSymbol{|}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e₁} \AgdaBound{e₁′} \AgdaBound{e₁∼e₁′} \AgdaBound{acce₁} \AgdaBound{acce₁′} \AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeαElemF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e₂} \AgdaBound{e₂′} \AgdaBound{e₂∼e₂′} \AgdaBound{acce₂} \AgdaBound{acce₂′}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{e₁″} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₁}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{e₂″} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₂}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaSymbol{.(}\AgdaBound{e₁″} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₁}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaSymbol{.(}\AgdaBound{e₂″} \AgdaInductiveConstructor{,} \AgdaBound{notOccur₂}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{|} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)} \AgdaBound{xe∼ye′} \AgdaSymbol{(}\AgdaInductiveConstructor{accB} \AgdaBound{facce}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accB} \AgdaBound{facce′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \<[8]%
\>[8]\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \<[8]%
\>[8]\AgdaFunction{inspect} \AgdaSymbol{(}\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \<[8]%
\>[8]\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \<[8]%
\>[8]\AgdaFunction{lemma∼fvF} \AgdaInductiveConstructor{[]} \AgdaBound{xe∼ye′}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{zs} \AgdaSymbol{|} \AgdaInductiveConstructor{[} \AgdaBound{fv≡zs} \AgdaInductiveConstructor{]ᵢ} \AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{zs} \AgdaSymbol{|} \AgdaInductiveConstructor{refl} \<[35]%
\>[35]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \<[8]%
\>[8]\AgdaFunction{χ'} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{z} \AgdaSymbol{|} \AgdaBound{z∉xs++fv}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Data.Product.map} \<[29]%
\>[29]\AgdaSymbol{(λ} \AgdaBound{e'} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{))} \<[47]%
\>[47]\<%
\\
\>[2]\AgdaIndent{29}{}\<[29]%
\>[29]\AgdaSymbol{(}\AgdaFunction{lemma-bindsB} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{z∉xs++fv}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαElemF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e′}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼B} \AgdaBound{xe∼ye′} \AgdaFunction{z\#xe}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facce} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facce′} \AgdaBound{z}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z∉fv} \AgdaSymbol{:} \AgdaBound{z} \AgdaFunction{∉} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z∉fv} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(}\AgdaFunction{\_∉\_} \AgdaBound{z}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{fv≡zs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{z∉xs++fv}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z\#xe} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{z\#xe} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaFunction{z∉fv}\<%
\end{code}

%<*bindersalpha>
\begin{code}%
\>\AgdaFunction{lemma-bindersFreeElem} \AgdaSymbol{:} \<[24]%
\>[24]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \<[43]%
\>[43]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'} \<[14]%
\>[14]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaFunction{bindersFreeElem} \AgdaBound{xs} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{bindersFreeElem} \AgdaBound{xs} \AgdaBound{e'}\<%
\end{code}
%</bindersalpha>

\begin{code}%
\>\AgdaFunction{lemma-bindersFreeElem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-bindersFreeαElemF} \AgdaInductiveConstructor{|R|} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'} \AgdaSymbol{(}\AgdaFunction{accF} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{accF} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{:} \<[27]%
\>[27]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \<[47]%
\>[47]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \<[62]%
\>[62]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{acce} \AgdaSymbol{:} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \AgdaSymbol{(}\AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{))} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaBound{e} \<[51]%
\>[51]\AgdaSymbol{\_} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αV}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaInductiveConstructor{|1|} \<[37]%
\>[37]\AgdaBound{xs} \AgdaBound{e} \<[51]%
\>[51]\AgdaSymbol{\_} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α1}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{B}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaBound{e} \<[51]%
\>[51]\AgdaSymbol{\_} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αE}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{accEf} \AgdaBound{acce}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αEf} \<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[37]%
\>[37]\AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{accR} \<[58]%
\>[58]\AgdaBound{acce}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αR} \<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{F} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{acc+₁} \AgdaBound{acce}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₁} \<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{acc+₂} \AgdaBound{acce}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼α+₂} \<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e} \AgdaBound{acce}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[51]%
\>[51]\AgdaSymbol{(}\AgdaInductiveConstructor{accx} \AgdaBound{acce₁} \AgdaBound{acce₂}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αx} \<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G₁} \AgdaBound{xs} \AgdaBound{e₁} \AgdaBound{acce₁}\AgdaSymbol{)} \<[123]%
\>[123]\<%
\\
\>[4]\AgdaIndent{81}{}\<[81]%
\>[81]\AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G₂} \AgdaBound{xs} \AgdaBound{e₂} \AgdaBound{acce₂}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{accB} \AgdaBound{facc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \<[8]%
\>[8]\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[27]%
\>[27]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \<[8]%
\>[8]\AgdaFunction{inspect} \AgdaSymbol{(}\AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{zs} \AgdaSymbol{|} \AgdaInductiveConstructor{[} \AgdaBound{fv≡zs} \AgdaInductiveConstructor{]ᵢ} \<[24]%
\>[24]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \<[8]%
\>[8]\AgdaFunction{χ'} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaFunction{lemmaχaux∉} \AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaBound{zs}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{z} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaBound{z∉xs++fv}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{∼αB} \AgdaBound{zs} \AgdaSymbol{(λ} \AgdaBound{y} \AgdaBound{y∉zs} \AgdaSymbol{→} \AgdaFunction{lemma∼} \AgdaBound{y∉zs}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{open} \AgdaModule{∼F-Reasoning}\AgdaSymbol{(}\AgdaBound{F}\AgdaSymbol{)(}\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{y} \AgdaFunction{∉} \AgdaBound{zs} \<[28]%
\>[28]\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{G} \<[18]%
\>[18]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facc} \AgdaBound{z}\AgdaSymbol{))))}\<%
\\
\>[9]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma∼} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{y∉zs}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeαElemF} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facc} \AgdaBound{z}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapEquivF} \AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaBound{G} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{facc} \AgdaBound{z}\AgdaSymbol{))} \AgdaBound{z} \AgdaBound{y} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{z} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaFunction{lemma∼swapCancelFƛ} \AgdaFunction{z\#xe} \AgdaFunction{y\#xe} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{z∉fv} \AgdaSymbol{:} \AgdaBound{z} \AgdaFunction{∉} \AgdaFunction{fvF} \<[20]%
\>[20]\AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[42]%
\>[42]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{z∉fv} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(}\AgdaFunction{\_∉\_} \AgdaBound{z}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{fv≡zs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{z∉xs++fv}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{z\#xe} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{z} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{z\#xe} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaFunction{z∉fv}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{y∉fv} \AgdaSymbol{:} \AgdaBound{y} \AgdaFunction{∉} \AgdaFunction{fvF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[41]%
\>[41]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{y∉fv} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(}\AgdaFunction{\_∉\_} \AgdaBound{y}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{fv≡zs}\AgdaSymbol{)} \AgdaBound{y∉zs}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{y\#xe} \AgdaSymbol{:} \AgdaDatatype{freshF} \AgdaBound{S} \AgdaBound{y} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{y\#xe} \AgdaSymbol{=} \AgdaFunction{lemmafvF\#} \AgdaFunction{y∉fv}\<%
\end{code}


\begin{code}%
\>\AgdaFunction{lemma-bindersFreeαFVα} \AgdaSymbol{:} \<[24]%
\>[24]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'} \<[14]%
\>[14]\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e'}\AgdaSymbol{)} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeαFVα} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{e∼e'} \AgdaKeyword{with} \AgdaFunction{fv} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{fv} \AgdaBound{e'} \AgdaSymbol{|} \AgdaFunction{lemma∼fv} \AgdaBound{e∼e'} \<[74]%
\>[74]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{fve} \AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{fve} \AgdaSymbol{|} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{bindersFreeElem} \AgdaBound{fve} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{bindersFreeElem} \AgdaBound{fve} \AgdaBound{e'} \AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeElem} \AgdaBound{fve} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{r} \AgdaInductiveConstructor{,} \AgdaBound{pr}\AgdaSymbol{)} \<[17]%
\>[17]\AgdaSymbol{|} \AgdaSymbol{(}\AgdaSymbol{.}\AgdaBound{r} \AgdaInductiveConstructor{,} \AgdaSymbol{.}\AgdaBound{pr}\AgdaSymbol{)} \<[31]%
\>[31]\AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}


%<*lemmabindersfreealpha>
\begin{code}%
\>\AgdaFunction{lemma-bindersFreeαAlpha} \AgdaSymbol{:} \<[26]%
\>[26]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \<[34]%
\>[34]\AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \<[41]%
\>[41]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{∼α} \AgdaBound{e}\<%
\end{code}
%</lemmabindersfreealpha>

\begin{code}%
\>\AgdaFunction{lemma-bindersFreeαAlpha} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{=} \AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlphaF} \AgdaInductiveConstructor{|R|} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{(}\AgdaFunction{accF} \AgdaBound{e}\AgdaSymbol{))}\<%
\end{code}

\begin{code}%
\>\AgdaFunction{bindersFreeα} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F}\<%
\\
\>\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{=} \AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeα-α} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-bindersFreeα-α} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{lemma-bindersFreeαAlpha} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeα-αCompatible} \AgdaSymbol{:} \<[33]%
\>[33]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'} \AgdaSymbol{→} \AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e'}\<%
\\
\>\AgdaFunction{lemma-bindersFreeα-αCompatible} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{e∼e'} \AgdaKeyword{with} \AgdaFunction{fv} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{fv} \AgdaBound{e'} \AgdaSymbol{|} \AgdaFunction{lemma∼fv} \AgdaBound{e∼e'} \<[88]%
\>[88]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{fve} \AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{fve} \AgdaSymbol{|} \AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaBound{fve} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaBound{fve} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e'} \AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeElem} \AgdaSymbol{(}\AgdaBound{fve} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼e'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{r} \AgdaInductiveConstructor{,} \AgdaBound{pr}\AgdaSymbol{)} \<[17]%
\>[17]\AgdaSymbol{|} \AgdaSymbol{(}\AgdaSymbol{.}\AgdaBound{r} \AgdaInductiveConstructor{,} \AgdaSymbol{.}\AgdaBound{pr}\AgdaSymbol{)} \<[31]%
\>[31]\AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeα-∉b} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{((}\AgdaFunction{fv} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{))} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeα-∉b} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{subst} \<[11]%
\>[11]\AgdaSymbol{(λ} \AgdaBound{ys} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{ys} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma∼fv} \AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeαAlpha} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)))}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaField{proj₂} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e} \AgdaFunction{++} \AgdaBound{xs}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaFunction{lemma-bindersFreeα-FV∉b} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-bindersFreeα-FV∉b} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{lemma-binds++l} \AgdaSymbol{(}\AgdaFunction{lemma-bindersFreeα-∉b} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}

\begin{code}%
\>\AgdaFunction{αCompatiblePred} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{αCompatiblePred} \AgdaSymbol{\{}\AgdaArgument{F} \AgdaSymbol{=} \AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{P} \AgdaSymbol{=} \AgdaSymbol{\{}\AgdaBound{e} \AgdaBound{e'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{e'} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e'}\<%
\end{code}

%<*strongalphacompatible>
\begin{code}%
\>\AgdaFunction{strong∼αCompatible} \<[20]%
\>[20]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \<[45]%
\>[45]\<%
\\
\>[2]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{strong∼αCompatible} \AgdaBound{f} \AgdaBound{M} \AgdaSymbol{=} \AgdaSymbol{∀} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{M} \AgdaDatatype{≡} \AgdaBound{f} \AgdaBound{N}\<%
\end{code}
%</strongalphacompatible>

%<*alphainductionhypotheses>
\begin{code}%
\>\AgdaFunction{fihalpha} \AgdaSymbol{:} \<[12]%
\>[12]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{List} \AgdaFunction{V} \AgdaSymbol{→} \<[66]%
\>[66]\AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\end{code}
%</alphainductionhypotheses>

%<*alphainductionhypothesescases>
\begin{code}%
\>\AgdaFunction{fihalpha} \AgdaInductiveConstructor{|R|} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaBound{P} \AgdaBound{e} \<[51]%
\>[51]\AgdaFunction{×} \AgdaSymbol{(∀} \AgdaBound{a} \AgdaSymbol{→} \AgdaBound{a} \AgdaFunction{∈} \AgdaBound{xs} \AgdaSymbol{→} \AgdaBound{a} \AgdaFunction{notOccurBind} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \<[18]%
\>[18]\AgdaBound{G}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaBound{x} \AgdaFunction{∉} \AgdaBound{xs} \<[51]%
\>[51]\AgdaFunction{×} \AgdaFunction{fihalpha} \AgdaBound{G} \<[65]%
\>[65]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e}\<%
\end{code}
%</alphainductionhypothesescases>

\begin{code}%
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[16]%
\>[16]\AgdaBound{S}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{n} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fihalpha} \AgdaInductiveConstructor{|1|} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaInductiveConstructor{tt} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[16]%
\>[16]\AgdaBound{B}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{b} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[16]%
\>[16]\AgdaBound{G}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[18]%
\>[18]\AgdaBound{G₂}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaFunction{fihalpha} \AgdaBound{G₁} \<[55]%
\>[55]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e} \<[62]%
\>[62]\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[18]%
\>[18]\AgdaBound{G₂}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaFunction{fihalpha} \AgdaBound{G₂} \<[55]%
\>[55]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e} \<[62]%
\>[62]\<%
\\
\>\AgdaFunction{fihalpha} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[18]%
\>[18]\AgdaBound{G₂}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaBound{P} \AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \<[42]%
\>[42]\AgdaFunction{fihalpha} \AgdaBound{G₁} \<[55]%
\>[55]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e₁} \<[64]%
\>[64]\AgdaFunction{×} \AgdaFunction{fihalpha} \AgdaBound{G₂} \AgdaBound{P} \AgdaBound{xs} \AgdaBound{e₂}\<%
\end{code}


\begin{code}%
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{:} \<[30]%
\>[30]\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)} \<[77]%
\>[77]\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaFunction{fih} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaSymbol{(λ} \AgdaBound{e'} \AgdaSymbol{→} \AgdaSymbol{(∀} \AgdaBound{c} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∈} \AgdaBound{xs} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{notOccurBind} \AgdaBound{e'}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e'}\AgdaSymbol{)} \AgdaBound{e} \<[70]%
\>[70]\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaSymbol{(∀} \AgdaBound{c} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∈} \AgdaBound{xs} \AgdaSymbol{→} \AgdaDatatype{notOccurBindF} \AgdaBound{c} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaFunction{fihalpha} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{G} \<[44]%
\>[44]\AgdaBound{P} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaBound{P} \AgdaBound{e} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccur} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaInductiveConstructor{|1|} \<[40]%
\>[40]\AgdaBound{P} \AgdaBound{e} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccur} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaBound{P} \AgdaBound{e} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccur} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaBound{P} \AgdaBound{e} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccur} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaInductiveConstructor{|R|} \<[40]%
\>[40]\AgdaBound{P} \AgdaBound{e} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccurR} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaBound{fih} \AgdaBound{notOccurR} \AgdaInductiveConstructor{,} \AgdaBound{notOccurR}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{P} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccurinj₁} \<[75]%
\>[75]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaBound{G₁} \<[38]%
\>[38]\AgdaBound{P} \AgdaBound{e} \AgdaBound{xs} \AgdaBound{fih} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBinj₁inv} \AgdaSymbol{(}\AgdaBound{notOccurinj₁} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{P} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccurinj₂} \<[75]%
\>[75]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaBound{G₂} \<[38]%
\>[38]\AgdaBound{P} \AgdaBound{e} \AgdaBound{xs} \AgdaBound{fih} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBinj₂inv} \AgdaSymbol{(}\AgdaBound{notOccurinj₂} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaBound{P} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[53]%
\>[53]\AgdaBound{xs} \AgdaSymbol{(}\AgdaBound{fih₁} \AgdaInductiveConstructor{,} \AgdaBound{fih₂}\AgdaSymbol{)} \AgdaBound{notOccur} \<[81]%
\>[81]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaBound{G₁} \<[36]%
\>[36]\AgdaBound{P} \AgdaBound{e₁} \AgdaBound{xs} \AgdaBound{fih₁} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBx₁inv} \AgdaSymbol{(}\AgdaBound{notOccur} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{))} \AgdaInductiveConstructor{,}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaBound{G₂} \<[36]%
\>[36]\AgdaBound{P} \AgdaBound{e₂} \AgdaBound{xs} \AgdaBound{fih₂} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBx₂inv} \AgdaSymbol{(}\AgdaBound{notOccur} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaBound{P} \AgdaSymbol{(}\AgdaBound{a} \<[46]%
\>[46]\AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[53]%
\>[53]\AgdaBound{xs} \AgdaBound{fih} \AgdaBound{notOccur} \<[71]%
\>[71]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{Any.any} \AgdaSymbol{(}\AgdaFunction{\_≟v\_} \AgdaBound{a}\AgdaSymbol{)} \AgdaBound{xs}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{a∈xs} \<[15]%
\>[15]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{((}\AgdaFunction{notOccurBBinv≢} \AgdaSymbol{(}\AgdaBound{notOccur} \AgdaBound{a} \AgdaBound{a∈xs}\AgdaSymbol{))} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[53]%
\>[53]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{a∉xs} \<[15]%
\>[15]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{a∉xs} \AgdaInductiveConstructor{,} \AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \AgdaBound{G} \AgdaBound{P} \AgdaBound{e} \AgdaBound{xs} \AgdaBound{fih} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBBinv} \AgdaSymbol{(}\AgdaBound{notOccur} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaComment{-- aux : \{F : Functor\}(P : μ F → Set)(xs : List V)}\<%
\\
\>\AgdaComment{--       → ((e : ⟦ F ⟧ (μ F)) → fihα F P xs e → P ⟨ e ⟩)      }\<%
\\
\>\AgdaComment{--       → (e : ⟦ F ⟧ (μ F)) }\<%
\\
\>\AgdaComment{--       → fih F (λ e' → (∀ c → c ∈ xs → c notOccurBind e') → P e') e}\<%
\\
\>\AgdaComment{--       → ((c : V) → c ∈ xs → \_notOccurBind\_ \{F\} c ⟨ e ⟩) }\<%
\\
\>\AgdaComment{--       → P ⟨ e ⟩}\<%
\\
\>\AgdaComment{-- aux \{F\} P xs hiα e hi notBind}\<%
\\
\>\AgdaComment{--   = hiα e (lemma-fih∧notOccurBind⇛fihα \{F\} F P e xs hi (λ c c∈xs → notOccurBRinv (notBind c c∈xs)))}\<%
\end{code}

%<*alphainductionprinciple>
\begin{code}%
\>\AgdaFunction{alphaPrimInd} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{αCompatiblePred} \AgdaBound{P} \<[77]%
\>[77]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{((}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fihalpha} \AgdaBound{F} \AgdaBound{P} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{P} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{∀} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e}\<%
\end{code}
%</alphainductionprinciple>

\begin{code}%
\>\AgdaFunction{alphaPrimInd} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{P} \AgdaBound{xs} \AgdaBound{αP} \AgdaBound{p} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{bindersFreeElem} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeαAlpha} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>\AgdaSymbol{...} \<[5]%
\>[5]\AgdaSymbol{|} \AgdaBound{e'} \AgdaInductiveConstructor{,} \AgdaBound{notBind} \AgdaSymbol{|} \AgdaBound{e'∼e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{αP} \<[8]%
\>[8]\AgdaBound{e'∼e}\<%
\\
\>[2]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{(}\AgdaFunction{foldInd} \<[18]%
\>[18]\AgdaBound{F} \<[20]%
\>[20]\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(λ} \AgdaBound{e} \AgdaSymbol{→} \AgdaSymbol{(∀} \AgdaBound{c} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∈} \AgdaBound{xs} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{notOccurBind} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(λ} \AgdaBound{e} \AgdaBound{hi} \AgdaBound{notBind}\<%
\\
\>[10]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{p} \<[18]%
\>[18]\AgdaBound{e}\<%
\\
\>[12]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{(}\AgdaFunction{lemma-fih∧notOccurBind⇛fihα} \<[48]%
\>[48]\AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{F} \AgdaBound{P} \AgdaBound{e} \AgdaBound{xs} \AgdaBound{hi}\<%
\\
\>[18]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∈xs} \AgdaSymbol{→} \AgdaFunction{notOccurBRinv} \AgdaSymbol{(}\AgdaBound{notBind} \AgdaBound{c} \AgdaBound{c∈xs}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaBound{e'} \<[13]%
\>[13]\<%
\\
\>[0]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{get} \AgdaBound{notBind}\AgdaSymbol{))}\<%
\end{code}
-- (aux {F} P xs p)
                         
-- αIteration : {F : Functor}{A : Set}(xs : List V)
--   → ((e : ⟦ F ⟧ (μ F)) → fihα F (const A) e xs → A)
--   → (e : μ F) → A
-- αIteration {A = A} xs f e = αPrimInd (const A) xs (const id) f e

-- lemma-αIteration-StrongαCompatible : 
--   {F : Functor}{A : Set}{xs : List V}{f : (e : ⟦ F ⟧ (μ F)) → fihα F (const A) e xs → A}
--   → {e : μ F} 
--   → strong∼αCompatible (αIteration xs f) e
-- lemma-αIteration-StrongαCompatible {xs = xs} {f} {e} e' e∼αe' 
--   with bindersFreeElem xs e | bindersFreeElem xs e' 
--   | lemma-bindersFreeElem xs e e' e∼αe' 
-- ... | (x , b) | (.x , .b) | refl = refl

{- Another way to obtain α Iteration -}
-- foldα : {A : Set}(F : Functor) → List V → (⟦ F ⟧ A → A) → μ F → A
-- foldα F xs f e with bindersFreeElem xs e
-- ... | e′ , _ = fold  F f e′
\end{code}





%<*foldCtxalpha>
\begin{code}%
\>\AgdaFunction{foldCtx-alpha} \AgdaSymbol{:} \<[17]%
\>[17]\AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \<[68]%
\>[68]\AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\<%
\\
\>\AgdaFunction{foldCtx-alpha} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaSymbol{(}\AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{))}\<%
\end{code}
%</foldCtxalpha>

%<*lemmafoldCtxalpha>
\begin{code}%
\>\AgdaFunction{lemma-foldCtxAlpha-foldCtx} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e′} \<[13]%
\>[13]\AgdaSymbol{:} \<[16]%
\>[16]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{S} \<[19]%
\>[19]\AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{foldCtx-alpha} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\<%
\end{code}
%</lemmafoldCtxalpha>

\begin{code}%
\>\AgdaFunction{lemma-foldCtxAlpha-foldCtx} \AgdaBound{F} \AgdaSymbol{\{}\AgdaArgument{c} \AgdaSymbol{=} \AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{cNotBinde} \AgdaKeyword{with} \AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeαAlpha} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{e′} \AgdaInductiveConstructor{,} \AgdaBound{nb} \AgdaSymbol{|} \AgdaBound{e′∼e} \AgdaSymbol{=} \AgdaFunction{lemma-foldCtx-alpha} \AgdaBound{prf} \AgdaBound{prf2} \AgdaBound{nb} \AgdaBound{cNotBinde} \AgdaFunction{ρ} \AgdaBound{e′∼e} \<[73]%
\>[73]\<%
\end{code}


%<*foldCtxalphastrongalphacompatible>
\begin{code}%
\>\AgdaFunction{lemma-foldCtxα-StrongαCompatible} \AgdaSymbol{:}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \<[43]%
\>[43]\AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{strong∼αCompatible} \AgdaSymbol{(}\AgdaFunction{foldCtx-alpha} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\<%
\end{code}
%</foldCtxalphastrongalphacompatible>

\begin{code}%
\>\AgdaFunction{lemma-foldCtxα-StrongαCompatible} \AgdaSymbol{\{}\AgdaArgument{f} \AgdaSymbol{=} \AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{e'} \AgdaBound{e∼αe'} \<[58]%
\>[58]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{|} \AgdaFunction{bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e'} \<[60]%
\>[60]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{|} \AgdaFunction{lemma-bindersFreeElem} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e} \AgdaBound{e'} \AgdaBound{e∼αe'} \<[44]%
\>[44]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{b}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaSymbol{(}\AgdaSymbol{.}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaSymbol{.}\AgdaBound{b}\AgdaSymbol{)} \AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}

%<*alphaproof>
\begin{code}%
\>\AgdaFunction{alphaProof} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{αCompatiblePred} \AgdaBound{P} \<[75]%
\>[75]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{((}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \<[16]%
\>[16]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e} \AgdaSymbol{)} \<[77]%
\>[77]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{∀} \AgdaBound{e} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e}\<%
\end{code}
%</alphaproof>

\begin{code}%
\>\AgdaFunction{alphaProof} \AgdaBound{P} \AgdaBound{xs} \AgdaBound{αC} \AgdaBound{proof} \AgdaBound{e}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaKeyword{with} \<[11]%
\>[11]\AgdaFunction{bindersFreeElem} \<[35]%
\>[35]\AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e}\AgdaSymbol{))} \AgdaBound{e}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{|} \<[11]%
\>[11]\AgdaFunction{lemma-bindersFreeαAlpha} \<[36]%
\>[36]\AgdaSymbol{(}\AgdaBound{xs} \AgdaFunction{++} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e}\AgdaSymbol{))} \AgdaBound{e}\<%
\\
\>\AgdaSymbol{...} \<[5]%
\>[5]\AgdaSymbol{|} \AgdaBound{e'} \AgdaInductiveConstructor{,} \AgdaBound{notBind} \AgdaSymbol{|} \AgdaBound{e'∼e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{αC} \AgdaBound{e'∼e} \AgdaSymbol{(}\AgdaBound{proof} \AgdaBound{e'} \AgdaFunction{nb1} \AgdaFunction{nb2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{nb1} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaBound{e'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{nb1} \AgdaSymbol{=} \AgdaFunction{lemma-binds++l} \AgdaBound{notBind}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{nb2} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{e'}\AgdaSymbol{)} \AgdaBound{e'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{nb2} \AgdaSymbol{=} \AgdaFunction{subst} \<[15]%
\>[15]\AgdaSymbol{(λ} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{e} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{(}\AgdaFunction{lemma∼fv} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaBound{e'∼e}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{notBind}\AgdaSymbol{)}\<%
\end{code}

%<*foldctxalpha-cxtalpha>
\begin{code}%
\>\AgdaFunction{lemma-foldCtxalpha-cxtalpha} \<[29]%
\>[29]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaBound{C} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}} \<[40]%
\>[40]\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′} \AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaBound{F} \AgdaBound{e} \AgdaBound{e′} \<[38]%
\>[38]\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e′}\AgdaSymbol{)} \<[49]%
\>[49]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{foldCtx-alpha} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{foldCtx-alpha} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c′} \AgdaBound{e}\<%
\end{code}
%</foldctxalpha-cxtalpha>

\begin{code}%
\>\AgdaFunction{lemma-foldCtxalpha-cxtalpha} \AgdaSymbol{\{}\AgdaArgument{c} \AgdaSymbol{=} \AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c′}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaBound{c∼c′} \AgdaBound{e} \<[52]%
\>[52]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{fv} \AgdaBound{c} \AgdaSymbol{|} \AgdaFunction{fv} \AgdaBound{c′} \AgdaSymbol{|} \AgdaFunction{lemma∼fv} \AgdaBound{c∼c′}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{fv} \AgdaSymbol{|} \AgdaSymbol{.}\AgdaBound{fv} \AgdaSymbol{|} \AgdaInductiveConstructor{refl} \AgdaSymbol{=} \AgdaFunction{lemma-foldCtx-alpha-Ctx} \AgdaBound{prf} \AgdaBound{c∼c′} \AgdaSymbol{(}\AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{bindersFreeElem} \AgdaBound{fv} \AgdaBound{e}\AgdaSymbol{))}\<%
\end{code}


--   lemma-binderFreeElemFold :
--     {F H C : Functor}{f : μ C → ⟦ F ⟧ (μ H) → μ H}{c c' : μ C}{e : μ F}{S : Sort}
--     → proj₁ (bindersFreeElem (fv S c) (foldS F f c' e))  ∼α
--       foldS F f (proj₁ (bindersFreeElem (fv S c) c')) (proj₁ (bindersFreeElem (fv S c) e))
-- binder (y,P) (M[x:=N]n) ∼ (binder (y,P) M) [ x := binder (y,P) N ] ????

{- Substitution Example - Can be done generically ? -}
-- substAux : {F : Functor}(G : Functor) 
--   → (x : V) → (e' : μ F) → (S : Sort) 
--   → (e : ⟦ G ⟧ (μ F)) 
--   → fihα G (const (⟦ F ⟧ (μ F))) e (x ∷ fv S e') 
--   →  ⟦ G ⟧ (μ F) ⊎ μ F
-- substAux (|v| S')    x e' S e         fihα    = {!!}
-- substAux |1|         x e' S e         fihα    = inj₁ tt
-- substAux (|E| B)     x e' S e         fihα    = inj₁ e
-- substAux (|Ef| G)    x e' S ⟨ e ⟩     fihα    = {! substAux {G} G x e' S e fihα)!}
-- substAux |R|         x e' S ⟨ e ⟩     (r , _) = inj₁ ⟨ r ⟩
-- substAux (G₁ |+| G₂) x e' S (inj₁ e)  fihα    = [ inj₁ ∘ inj₁ , inj₂ ]′ (substAux G₁ x e' S e fihα)
-- substAux (G₁ |+| G₂) x e' S (inj₂ e)  fihα    = [ inj₁ ∘ inj₂ , inj₂ ]′ (substAux G₂ x e' S e fihα)
-- substAux (G₁ |x| G₂) x e' S (e₁ , e₂) (fihα₁ , fihα₂) = {! !}
-- substAux (|B| S' G)  x e' S (y  , e)  fihα   = {!!}

-- substAux' : (F : Functor) 
--   → (x : V) → (e' : μ F) → (S : Sort) 
--   → (e : ⟦ F ⟧ (μ F)) 
--   → fihα F (const (⟦ F ⟧ (μ F))) e (x ∷ fv S e') 
--   → ⟦ F ⟧ (μ F)
-- substAux' F x e' S e fihα with substAux {F} F x e' S e fihα
-- ... | inj₁ r      = r
-- ... | inj₂ ⟨ r ⟩  = r

-- _[_≔_]_ : {F : Functor} → μ F → V → μ F → Sort → μ F
-- _[_≔_]_ {F} e x e' S = ⟨ αIteration (x ∷ fv S e') (substAux' F x e' S) e ⟩

Recursion

-- \begin{code}%
\>\AgdaComment{-- recCtxα :  \{C H : Functor\}(F : Functor)}\<%
\\
\>\AgdaComment{--             → (μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))  → μ H)}\<%
\\
\>\AgdaComment{--             → μ C → μ F → μ H}\<%
\\
\>\AgdaComment{-- recCtxα F f c e = recCtx F f c (proj₁ (bindersFreeElem (fv c) e))}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recCtxα-StrongαCompatible :}\<%
\\
\>\AgdaComment{--   \{C H F : Functor\}\{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c : μ C\}\{e : μ F\}}\<%
\\
\>\AgdaComment{--   → strong∼αCompatible (recCtxα F f c) e}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recCtxα-StrongαCompatible \{f = f\} \{c\} \{e\} e' e∼αe' }\<%
\\
\>\AgdaComment{--   with bindersFreeElem (fv c) e | bindersFreeElem (fv c) e' }\<%
\\
\>\AgdaComment{--   | lemma-bindersFreeElem (fv c) e e' e∼αe' }\<%
\\
\>\AgdaComment{-- ... | (x , b) | (.x , .b) | refl = refl}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx  : \{F H C : Functor\}(G : Functor)}\<%
\\
\>\AgdaComment{--               \{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c c′ : μ C\}}\<%
\\
\>\AgdaComment{--               → (\{e e′ :  ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)  }\<%
\\
\>\AgdaComment{--               → c ∼α c′}\<%
\\
\>\AgdaComment{--               → (e : ⟦ G ⟧ (μ F)) → ∼αF G (recmapCtx F G f c e) (recmapCtx F G f c′ e)}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (|v| S)      prf c∼c′  e          = ∼αV}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx |1|          prf c∼c′  e          = ∼α1}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx \{F\} |R|      prf c∼c′  ⟨ e ⟩      = ∼αR (∼αx (lemma-∼αR (prf c∼c′   (lemma-recmapSCtx F prf c∼c′ e))) ρF)    }\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (|E| x)      prf c∼c′  e          = ∼αE }\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (|Ef| G)     prf c∼c′  e          = ρF }\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (G₁ |+| G₂)  prf c∼c′  (inj₁ e)   = ∼α+₁  (lemma-recmapSCtx G₁ prf c∼c′  e)}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (G₁ |+| G₂)  prf c∼c′  (inj₂ e)   = ∼α+₂  (lemma-recmapSCtx G₂ prf c∼c′  e)}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (G₁ |x| G₂)  prf c∼c′  (e₁ , e₂)  = ∼αx   (lemma-recmapSCtx G₁ prf c∼c′  e₁) (lemma-recmapSCtx G₂ prf c∼c′  e₂)}\<%
\\
\>\AgdaComment{-- lemma-recmapSCtx (|B| S G)    prf c∼c′  (x , e)    = ∼αB   [] (λ y y∉[] → lemma∼swapEquivF (lemma-recmapSCtx G prf c∼c′  e) x y)}\<%
\\
%
\\
\>\AgdaComment{-- lemma-recCtx2  : \{F H C : Functor\}\{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c c′ : μ C\}}\<%
\\
\>\AgdaComment{--      → (\{e e′ :  ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)}\<%
\\
\>\AgdaComment{--      → c ∼α c′}\<%
\\
\>\AgdaComment{--      → (e : μ F) → recCtx F f c e ∼α recCtx F f c′ e}\<%
\\
\>\AgdaComment{-- lemma-recCtx2 \{F\} \{f = f\} \{c\} \{c′\} prf c∼c′ ⟨ e ⟩ = prf c∼c′ (lemma-recmapSCtx F prf c∼c′ e) }\<%
\\
\>\AgdaComment{-- }\<%
\end{code}


-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recmapα  : \{F H C : Functor\}(G : Functor)\{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c c' : μ C\}\{e e' : ⟦ G ⟧ (μ F)\}}\<%
\\
\>\AgdaComment{--                → (\{e e′ :  ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)}\<%
\\
\>\AgdaComment{--                → (\{c : μ C\}\{S : Sort\}\{x y : V\}\{e : ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\} }\<%
\\
\>\AgdaComment{--                      → f (swap S x y c) (swapF F S x y e) ≡ swap S x y (f c e))}\<%
\\
\>\AgdaComment{--                → c ∼α c'}\<%
\\
\>\AgdaComment{--                → ∼αF G e e'  }\<%
\\
\>\AgdaComment{--                → ∼αF G (recmapCtx F G f c e) (recmapCtx F G f c' e')}\<%
\\
\>\AgdaComment{-- lemma-recmapα (|v| S)        prf \_  \_    ∼αV         = ∼αV  }\<%
\\
\>\AgdaComment{-- lemma-recmapα |1|            prf \_  \_    ∼α1         = ∼α1 }\<%
\\
\>\AgdaComment{-- lemma-recmapα \{F\} |R|        prf prf2 c∼c' (∼αR e∼e')}\<%
\\
\>\AgdaComment{--   = ∼αR (∼αx (lemma-∼αR (prf c∼c'   (lemma-recmapα F prf prf2 c∼c' e∼e'))) (∼αEf e∼e'))     }\<%
\\
\>\AgdaComment{-- lemma-recmapα (|E| x)        prf \_  \_    ∼αE         = ρF }\<%
\\
\>\AgdaComment{-- lemma-recmapα (|Ef| G)       prf \_  \_    (∼αEf e∼e') = ∼αEf e∼e'}\<%
\\
\>\AgdaComment{-- lemma-recmapα (G₁ |+| G₂)    prf prf2  c∼c' (∼α+₁ e∼e')}\<%
\\
\>\AgdaComment{--   = ∼α+₁  (lemma-recmapα G₁ prf prf2  c∼c' e∼e')  }\<%
\\
\>\AgdaComment{-- lemma-recmapα (G₁ |+| G₂)    prf prf2 c∼c' (∼α+₂ e∼e')}\<%
\\
\>\AgdaComment{--   = ∼α+₂  (lemma-recmapα G₂ prf prf2 c∼c' e∼e') }\<%
\\
\>\AgdaComment{-- lemma-recmapα (G₁ |x| G₂)    prf prf2 c∼c' (∼αx α₁ α₂)}\<%
\\
\>\AgdaComment{--   = ∼αx   (lemma-recmapα G₁ prf prf2  c∼c' α₁)}\<%
\\
\>\AgdaComment{--           (lemma-recmapα G₂ prf prf2  c∼c' α₂)  }\<%
\\
\>\AgdaComment{-- lemma-recmapα \{F\} \{H\} \{C\} (|B| S G) \{f\} \{c\} \{c'\}  \{y , e\} \{z , e'\}}\<%
\\
\>\AgdaComment{--                prf prf2 c∼c' (∼αB xs fα)  }\<%
\\
\>\AgdaComment{--   = ∼αB  (fv c ++ fv c' ++ xs)}\<%
\\
\>\AgdaComment{--          (λ x x∉ → begin}\<%
\\
\>\AgdaComment{--                      swapF G S y x (recmapCtx F G f c e)}\<%
\\
\>\AgdaComment{--                    ≈⟨ \{!!\}  ⟩}\<%
\\
\>\AgdaComment{--                      recmapCtx F G f (swap S y x c) (swapF G S y x e)}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-recmapSCtx G prf}\<%
\\
\>\AgdaComment{--                                         \{!!\}}\<%
\\
\>\AgdaComment{--                                         (swapF G S y x e) ⟩}\<%
\\
\>\AgdaComment{--                      recmapCtx F G f c              (swapF G S y x e)}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-recmapα  G prf prf2}\<%
\\
\>\AgdaComment{--                                       c∼c'}\<%
\\
\>\AgdaComment{--                                       (fα x (c∉xs++ys→c∉ys \{xs = fv c'\} (c∉xs++ys→c∉ys \{xs = fv c\} x∉))) ⟩}\<%
\\
\>\AgdaComment{--                      recmapCtx F G f c'             (swapF G S z x e')}\<%
\\
\>\AgdaComment{--                    ∼⟨ lemma-recmapSCtx  G prf \{!!\}}\<%
\\
\>\AgdaComment{--                                          (swapF G S z x e') ⟩}\<%
\\
\>\AgdaComment{--                      recmapCtx F G f (swap S z x c') (swapF G S z x e')}\<%
\\
\>\AgdaComment{--                    ≈⟨ \{!!\} ⟩}\<%
\\
\>\AgdaComment{--                      swapF G S z x (recmapCtx F G f c' e')}\<%
\\
\>\AgdaComment{--                    ∎)}\<%
\\
\>\AgdaComment{--      where}\<%
\\
\>\AgdaComment{--      open ∼F-Reasoning(|Ef| H |x| |Ef| F)(G)}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}
  

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recCtx  : \{F H C : Functor\}\{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c c' : μ C\}\{e e' : μ F\}}\<%
\\
\>\AgdaComment{--                → (\{e e′ :  ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)}\<%
\\
\>\AgdaComment{--                → (\{c : μ C\}\{S : Sort\}\{x y : V\}\{e : ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\} }\<%
\\
\>\AgdaComment{--                      → f (swap S x y c) (swapF F S x y e) ≡ swap S x y (f c e))}\<%
\\
\>\AgdaComment{--                → c ∼α c'}\<%
\\
\>\AgdaComment{--                → e ∼α e'  }\<%
\\
\>\AgdaComment{--                → recCtx F f c e ∼α recCtx F f c' e'}\<%
\\
\>\AgdaComment{-- lemma-recCtx prf prf2  c∼c' e∼e' = \{!  (lemma-recmapα |R| prf prf2 c∼c' e∼e')!\} }\<%
\\
\>\AgdaComment{-- }\<%
\end{code}


-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recCtxα-recCtx  :}\<%
\\
\>\AgdaComment{--   \{C H : Functor\}(F : Functor)\{f : μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H\}\{c : μ C\}\{e : μ F\}}\<%
\\
\>\AgdaComment{--   → (\{e e′ :  ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\}\{c c′ : μ C\} → c ∼α c′ → ∼αF F e e′ → f c e ∼α f c′ e′)}\<%
\\
\>\AgdaComment{--   → (\{c : μ C\}\{S : Sort\}\{x y : V\}\{e : ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))\} }\<%
\\
\>\AgdaComment{--                      → f (swap S x y c) (swapF F S x y e) ≡ swap S x y (f c e))}\<%
\\
\>\AgdaComment{--   → recCtxα F f c e ∼α recCtx F f c e}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}


-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- lemma-recCtxα-recCtx F \{c = c\} \{e\} prf prf2 with bindersFreeElem (fv c) e | lemma-bindersFreeαAlpha (fv c) e}\<%
\\
\>\AgdaComment{-- ... | e′ , nb | e′∼e = lemma-recCtx prf prf2 ρ e′∼e  }\<%
\\
\>\AgdaComment{-- }\<%
\end{code}



==> GenericProgramming/Examples/LambdaCalculus.tex <==
Lambda Calculus

\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{Examples.LambdaCalculus} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Function} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{\_⟨\_⟩\_}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{fold}\AgdaSymbol{;}\AgdaPrimitive{\_*\_}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat.Properties}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{;}\AgdaFunction{,\_}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{Rel}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.Any} \AgdaSymbol{as} \AgdaModule{Any} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{tail}\AgdaSymbol{;}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{Any.}\AgdaModule{Membership-≡} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{\_⊆\_} \AgdaSymbol{to} \AgdaFunction{\_⊆l\_}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaSymbol{as} \AgdaModule{PropEq} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]} \AgdaSymbol{to} \AgdaInductiveConstructor{[\_]ᵢ}\AgdaSymbol{;}\AgdaFunction{trans} \AgdaSymbol{to} \AgdaFunction{trans≡}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{PropEq.}\AgdaModule{≡-Reasoning} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{begin\_} \AgdaSymbol{to} \AgdaFunction{begin≡\_}\AgdaSymbol{;}\AgdaFunction{\_∎} \AgdaSymbol{to} \AgdaFunction{\_□}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{GPBindings}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Atom}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Swap}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{FreeVariables}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Alpha}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{AlphaInduction}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{OccurBind}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{List.ListProperties}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{8} \AgdaFunction{\_·\_}\<%
\end{code}

\begin{code}%
\>\AgdaFunction{SortλTermVars} \AgdaSymbol{:} \AgdaFunction{Sort}\<%
\\
\>\AgdaFunction{SortλTermVars} \AgdaSymbol{=} \AgdaNumber{1}\<%
\end{code}

%<*lambdacalculus>
\begin{code}%
\>\AgdaFunction{λF} \AgdaSymbol{:} \AgdaDatatype{Functor} \<[41]%
\>[41]\AgdaComment{-- M,N  :-}\<%
\\
\>\AgdaFunction{λF} \AgdaSymbol{=} \<[10]%
\>[10]\AgdaInductiveConstructor{|v|} \AgdaFunction{SortλTermVars} \<[41]%
\>[41]\AgdaComment{--           x}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|R|} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|R|} \<[41]%
\>[41]\AgdaComment{--      |    M N}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|B|} \AgdaFunction{SortλTermVars} \AgdaInductiveConstructor{|R|} \<[41]%
\>[41]\AgdaComment{--      |    λ x M}\<%
\end{code}
%</lambdacalculus>

%<*lambdacalculusmu>
\begin{code}%
\>\AgdaFunction{λTerm} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{λTerm} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaFunction{λF}\<%
\end{code}
%</lambdacalculusmu>

%<*lambdaconstvar>
\begin{code}%
\>\AgdaFunction{v} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaFunction{v} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨\_⟩} \AgdaFunction{∘} \AgdaInductiveConstructor{inj₁}\<%
\end{code}
%</lambdaconstvar>

%<*lambdaconstapp>
\begin{code}%
\>\AgdaFunction{\_·\_} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\<%
\end{code}
%</lambdaconstapp>

%<*lambdaconstlam>
\begin{code}%
\>\AgdaFunction{ƛ} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaFunction{ƛ} \AgdaBound{n} \AgdaBound{M} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{n} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\<%
\end{code}
%</lambdaconstlam>

\begin{code}%
\>\AgdaFunction{testswap1} \AgdaSymbol{:} \AgdaFunction{swap} \AgdaFunction{SortλTermVars} \AgdaNumber{1} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaDatatype{≡} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{2} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{testswap1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}

Define function by primitive recursion directly

%<*vars>
\begin{code}%
\>\AgdaFunction{vars'} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λF} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{vars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{\_} \AgdaInductiveConstructor{⟩} \<[31]%
\>[31]\AgdaSymbol{=} \<[34]%
\>[34]\AgdaNumber{1}\<%
\\
\>\AgdaFunction{vars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{m} \AgdaInductiveConstructor{,} \AgdaBound{n}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[31]%
\>[31]\AgdaSymbol{=} \<[34]%
\>[34]\AgdaFunction{vars'} \AgdaBound{m}\<%
\\
\>[5]\AgdaIndent{31}{}\<[31]%
\>[31]\AgdaPrimitive{+} \<[34]%
\>[34]\AgdaFunction{vars'} \AgdaBound{n}\<%
\\
\>\AgdaFunction{vars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaBound{m}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[31]%
\>[31]\AgdaSymbol{=} \<[34]%
\>[34]\AgdaFunction{vars'} \AgdaBound{m}\<%
\end{code}
%</vars>

Now using fold.

%<*varsfold1>
\begin{code}%
\>\AgdaFunction{varsaux} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λF} \AgdaFunction{⟧} \AgdaDatatype{ℕ} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{\_)} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaNumber{1}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{m} \AgdaInductiveConstructor{,} \AgdaBound{n}\AgdaSymbol{)))} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaBound{m} \AgdaPrimitive{+} \AgdaBound{n}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaBound{m}\AgdaSymbol{)))} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaBound{m}\<%
\end{code}
%</varsfold1>

%<*varsfold2>
\begin{code}%
\>\AgdaFunction{vars} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λF} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{vars} \AgdaSymbol{=} \AgdaFunction{fold} \AgdaFunction{λF} \AgdaFunction{varsaux}\<%
\end{code}
%</varsfold2>

Prove trivial property of vars function by primitive induction.

%<*varsproof1>
\begin{code}%
\>\AgdaFunction{PVars} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λF} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{PVars} \AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{vars} \AgdaBound{M} \AgdaFunction{>} \AgdaNumber{0}\<%
\end{code}
%</varsproof1>

%<*varsproof2>
\begin{code}%
\>\AgdaFunction{plus>0} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{m} \AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{m} \AgdaFunction{>} \AgdaNumber{0} \AgdaSymbol{→} \AgdaBound{n} \AgdaFunction{>} \AgdaNumber{0} \AgdaSymbol{→} \AgdaBound{m} \AgdaPrimitive{+} \AgdaBound{n} \AgdaFunction{>} \AgdaNumber{0}\<%
\\
\>\AgdaFunction{plus>0} \AgdaSymbol{\{}\AgdaBound{m}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{n}\AgdaSymbol{\}} \AgdaBound{m>0} \AgdaBound{n>0} \AgdaSymbol{=} \AgdaFunction{≤-steps} \AgdaBound{m} \AgdaBound{n>0}\<%
\end{code}
%</varsproof2>

%<*proof'>
\begin{code}%
\>\AgdaFunction{provePVars'} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λF}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{PVars} \AgdaBound{M}\<%
\\
\>\AgdaFunction{provePVars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{x} \<[37]%
\>[37]\AgdaInductiveConstructor{⟩} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>\AgdaFunction{provePVars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(} \AgdaBound{M} \<[30]%
\>[30]\AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaFunction{plus>0} \AgdaSymbol{(}\AgdaFunction{provePVars'} \AgdaBound{M}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{provePVars'} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{provePVars'} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \<[31]%
\>[31]\AgdaBound{M}\AgdaSymbol{))} \<[37]%
\>[37]\AgdaInductiveConstructor{⟩} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaFunction{provePVars'} \AgdaBound{M}\<%
\end{code}
%</proof'>

%<*proofpvars>
\begin{code}%
\>\AgdaFunction{proof} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{λF}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaFunction{λF} \AgdaFunction{PVars} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{PVars} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{x}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaBound{tt} \<[43]%
\>[43]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \<[22]%
\>[22]\AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{)))} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaBound{ihM} \AgdaInductiveConstructor{,} \AgdaBound{ihN}\AgdaSymbol{)} \<[43]%
\>[43]\AgdaSymbol{=} \AgdaFunction{plus>0} \AgdaBound{ihM} \AgdaBound{ihN}\<%
\\
\>\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(\_} \<[22]%
\>[22]\AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))} \<[30]%
\>[30]\AgdaBound{ihM} \<[43]%
\>[43]\AgdaSymbol{=} \AgdaBound{ihM}\<%
\end{code}
%</proofpvars>

%<*proof>
\begin{code}%
\>\AgdaFunction{provePVars} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λF}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{PVars} \AgdaBound{M}\<%
\\
\>\AgdaFunction{provePVars} \AgdaSymbol{=} \AgdaFunction{foldInd} \AgdaFunction{λF} \AgdaFunction{PVars} \AgdaFunction{proof}\<%
\end{code}
%</proof>

Expression Problem (Data types a la carte, Reviewer 2)

\begin{code}%
\>\AgdaFunction{λExtF} \AgdaSymbol{:} \AgdaDatatype{Functor} \<[44]%
\>[44]\AgdaComment{-- M,N  :-}\<%
\\
\>\AgdaFunction{λExtF} \AgdaSymbol{=} \<[9]%
\>[9]\AgdaInductiveConstructor{|B|} \AgdaFunction{SortλTermVars} \AgdaSymbol{(}\AgdaInductiveConstructor{|R|} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|R|}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaComment{--      | let x = M in N }\<%
\\
%
\\
\>\AgdaFunction{varsauxExt} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λExtF} \AgdaFunction{⟧} \AgdaDatatype{ℕ} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{varsauxExt} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{m} \AgdaInductiveConstructor{,} \AgdaBound{n}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaBound{m} \AgdaPrimitive{+} \AgdaBound{n}\<%
\\
%
\\
\>\AgdaFunction{varsExt} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λExtF} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{varsExt} \AgdaSymbol{=} \AgdaFunction{fold} \AgdaFunction{λExtF} \AgdaFunction{varsauxExt}\<%
\\
%
\\
\>\AgdaFunction{PVarsExt} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λExtF} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{PVarsExt} \AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{varsExt} \AgdaBound{M} \AgdaFunction{>} \AgdaNumber{0}\<%
\\
%
\\
\>\AgdaFunction{proofExt} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λExtF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{λExtF}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaFunction{λExtF} \AgdaFunction{PVarsExt} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{PVarsExt} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>\AgdaFunction{proofExt} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{ihM} \AgdaInductiveConstructor{,} \AgdaBound{ihN}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaFunction{plus>0} \AgdaBound{ihM} \AgdaBound{ihN}\<%
\\
%
\\
\>\AgdaFunction{provePVarsExt} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λExtF}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{PVarsExt} \AgdaBound{M}\<%
\\
\>\AgdaFunction{provePVarsExt} \AgdaSymbol{=} \AgdaFunction{foldInd} \AgdaFunction{λExtF} \AgdaFunction{PVarsExt} \AgdaFunction{proofExt}\<%
\\
%
\\
\>\AgdaFunction{λLetF} \AgdaSymbol{:} \AgdaDatatype{Functor}\<%
\\
\>\AgdaFunction{λLetF} \AgdaSymbol{=} \AgdaFunction{λF} \AgdaInductiveConstructor{|+|} \AgdaFunction{λExtF}\<%
\\
%
\\
\>\AgdaFunction{varsLet} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{λLetF} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{varsLet} \AgdaSymbol{=} \AgdaFunction{fold} \AgdaFunction{λLetF} \AgdaFunction{[} \AgdaFunction{varsaux} \AgdaFunction{,} \AgdaFunction{varsauxExt} \AgdaFunction{]′}\<%
\end{code}

Substitiution

\begin{code}%
\>\AgdaKeyword{infix} \AgdaNumber{20} \AgdaFunction{\_[\_≔\_]ₙ}\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{20} \AgdaFunction{\_[\_≔\_]}\<%
\end{code}


Naive substitution, assuming binders in M not equal x !

In abstraction case we do not check if x ≡ y, we cannot alse because is a iteration principle

%<*substcontext>
\begin{code}%
\>\AgdaFunction{cF} \AgdaSymbol{=} \<[6]%
\>[6]\AgdaInductiveConstructor{|v|} \AgdaFunction{SortλTermVars} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{λF}\<%
\end{code}
%</substcontext>

%<*substaux>
\begin{code}%
\>\AgdaFunction{substaux} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{cF} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaFunction{λF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{λF}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaFunction{λF}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaInductiveConstructor{,} \AgdaBound{t₂}\AgdaSymbol{)))} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaBound{t₁} \AgdaFunction{·} \AgdaBound{t₂}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{)))} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{t} \<[56]%
\>[56]\<%
\\
\>\AgdaFunction{substaux} \AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \<[16]%
\>[16]\AgdaBound{N} \AgdaInductiveConstructor{⟩} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{y}\AgdaSymbol{)} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaBound{N}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{v} \AgdaBound{y} \<%
\end{code}
%</substaux>

%<*naivesubst>
\begin{code}%
\>\AgdaFunction{\_[\_≔\_]ₙ} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \<[14]%
\>[14]\AgdaSymbol{=} \AgdaFunction{foldCtx} \AgdaFunction{λF} \AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M}\<%
\end{code}
%</naivesubst>

%<*subst>
\begin{code}%
\>\AgdaFunction{\_[\_≔\_]} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \<[14]%
\>[14]\AgdaSymbol{=} \AgdaFunction{foldCtx-alpha} \AgdaFunction{λF} \AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M} \<%
\end{code}
%</subst>

Examples 

\begin{code}%
\>\AgdaFunction{exampleSubstn1} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{2} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]ₙ} \AgdaDatatype{≡} \AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{exampleSubstn1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{exampleSubst1} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{2} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaFunction{ƛ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{0} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{exampleSubst1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{exampleSubst2} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{2} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{3}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{3} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaFunction{ƛ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{0} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{exampleSubst2} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}

%<*substlemma1>
\begin{code}%
\>\AgdaFunction{lemma-substα} \<[14]%
\>[14]\AgdaSymbol{:} \<[17]%
\>[17]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M′} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \<[44]%
\>[44]\AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\<%
\\
\>\AgdaFunction{lemma-substα} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M′}\AgdaSymbol{\}} \AgdaBound{M∼M′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtxα-StrongαCompatible} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaBound{M′} \AgdaBound{M∼M′}\<%
\end{code}
%</substlemma1>

\begin{code}%
\>\AgdaKeyword{infix} \AgdaNumber{9} \AgdaFunction{（\_∙\_）\_} \<[15]%
\>[15]\<%
\\
\>\AgdaFunction{（\_∙\_）\_} \AgdaSymbol{=} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaFunction{SortλTermVars}\<%
\end{code}

%<*substauxswap>
\begin{code}%
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{cF}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λF} \AgdaFunction{⟧} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{substaux} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaFunction{λF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaDatatype{≡}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{(}\AgdaFunction{substaux} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}
%</substauxswap>

\begin{code}%
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{SortλTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[20]%
\>[20]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[29]%
\>[29]\AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[28]%
\>[28]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[37]%
\>[37]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[37]%
\>[37]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[43]%
\>[43]\AgdaBound{z≢z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{z≢z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢y} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{x≡w}\AgdaSymbol{)} \AgdaBound{x≡y}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[55]%
\>[55]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡w} \AgdaBound{w≡y}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[52]%
\>[52]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{y} \<[74]%
\>[74]\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≢y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{w≢z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢z} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{x≡w}\AgdaSymbol{)} \AgdaBound{x≡z}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[39]%
\>[39]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[55]%
\>[55]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡w} \AgdaBound{w≡y}\AgdaSymbol{))} \<[88]%
\>[88]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[49]%
\>[49]\AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[53]%
\>[53]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡w} \AgdaBound{w≡z}\AgdaSymbol{))} \<[98]%
\>[98]\<%
\\
\>\AgdaSymbol{...} \<[53]%
\>[53]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl} \<[80]%
\>[80]\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢w} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaBound{x≡w}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaKeyword{with} \AgdaFunction{SortλTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[28]%
\>[28]\AgdaBound{SortλTermVars≢S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{SortλTermVars≢S} \AgdaBound{SortλTermVars≡S}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[30]%
\>[30]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[40]%
\>[40]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡y} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡y}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[40]%
\>[40]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[46]%
\>[46]\AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{y} \<[73]%
\>[73]\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{z≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡y} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{z≡y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡z}\AgdaSymbol{))))}\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{z≢y} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \<[35]%
\>[35]\<%
\\
\>[3]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \<[61]%
\>[61]\AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{z≡w} \AgdaSymbol{=} \<[75]%
\>[75]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{z≡w}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \<[72]%
\>[72]\AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡y}\AgdaSymbol{))))}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢z} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡z}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[80]%
\>[80]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡w} \AgdaSymbol{=} \<[93]%
\>[93]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢y} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡w}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \<[80]%
\>[80]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢w} \AgdaSymbol{=} \<[92]%
\>[92]\AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[74]%
\>[74]\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{=} \<[84]%
\>[84]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z} \<[83]%
\>[83]\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{=} \<[94]%
\>[94]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaBound{x≡y}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \<[72]%
\>[72]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \AgdaSymbol{=} \<[94]%
\>[94]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaBound{x≡w}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[3]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{SortλTermVars≢S} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[14]%
\>[14]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[25]%
\>[25]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[14]%
\>[14]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[20]%
\>[20]\AgdaSymbol{\_} \<[25]%
\>[25]\AgdaKeyword{with} \AgdaFunction{SortλTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[26]%
\>[26]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortλTermVars≡S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{SortλTermVars≢S} \AgdaBound{SortλTermVars≡S}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[26]%
\>[26]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M'}\AgdaSymbol{))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}

%<*swapsubst>
\begin{code}%
\>\AgdaFunction{lemma-[]Swap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{y} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaFunction{（} \AgdaBound{y} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{x} \AgdaFunction{≔} \AgdaFunction{（} \AgdaBound{y} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaDatatype{≡} \AgdaFunction{（} \AgdaBound{y} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-[]Swap} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemmaSwapFoldCtxEquiv} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{SortλTermVars}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[97]%
\>[97]\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\end{code}
%</swapsubst>

\begin{code}%
\>\AgdaFunction{lemma-substaux} \<[16]%
\>[16]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{λF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{λF}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \<[49]%
\>[49]\AgdaDatatype{μ} \AgdaFunction{cF}\AgdaSymbol{\}}\<%
\\
\>[7]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′}\<%
\\
\>[7]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaFunction{λF} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>[7]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaFunction{substaux} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{substaux} \AgdaBound{c′} \AgdaBound{e′}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaInductiveConstructor{∼αV}\AgdaSymbol{)} \<[89]%
\>[89]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y} \<[14]%
\>[14]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[52]%
\>[52]\AgdaSymbol{=} \<[55]%
\>[55]\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[52]%
\>[52]\AgdaSymbol{=} \<[55]%
\>[55]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaInductiveConstructor{∼αV}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))} \<[52]%
\>[52]\AgdaSymbol{=} \<[55]%
\>[55]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁}\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)))} \<[52]%
\>[52]\AgdaSymbol{=} \<[55]%
\>[55]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)))}\<%
\\
%
\\
%
\\
\>\AgdaFunction{lemma-substnα′} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{N′} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{N′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-substnα′} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaFunction{lemma-foldCtx-alpha-Ctx} \AgdaFunction{lemma-substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaBound{M}\<%
\end{code}

%<*substlemma2>
\begin{code}%
\>\AgdaFunction{lemma-substα′} \<[15]%
\>[15]\AgdaSymbol{:} \<[18]%
\>[18]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{N′} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \<[45]%
\>[45]\AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{N′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \AgdaFunction{]}\<%
\\
\>\AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\AgdaSymbol{)} \<[33]%
\>[33]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtxalpha-cxtalpha} \AgdaFunction{lemma-substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaBound{M}\<%
\end{code}
%</substlemma2>

\begin{code}%
\>\AgdaFunction{fv2ctx} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{)} \AgdaBound{M} \<[63]%
\>[63]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>\AgdaFunction{fv2ctx} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{nb} \AgdaSymbol{=} \AgdaBound{nb}\<%
\end{code}

%<*lemmanaivesubst>
\begin{code}%
\>\AgdaFunction{lemmaSubsts} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaSymbol{\{}\AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{)} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaBound{nb}\<%
\\
\> \AgdaSymbol{=} \AgdaFunction{lemma-foldCtxAlpha-foldCtx} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaFunction{λF} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{lemma-substaux}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(}\AgdaFunction{fv2ctx} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaBound{nb}\AgdaSymbol{)}\<%
\end{code}
%</lemmanaivesubst>

Naive Substitution Composition

\begin{code}%
\>\AgdaFunction{lemma-substnfv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaFunction{fvS} \AgdaFunction{SortλTermVars} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{≡} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{y} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[54]%
\>[54]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fvy} \AgdaSymbol{\_} \<[70]%
\>[70]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{((}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{x∉fvy}\AgdaSymbol{)} \AgdaBound{x≡y}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{x≢y} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M′}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[54]%
\>[54]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv} \<[67]%
\>[67]\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaBound{xnbM} \AgdaBound{xnbM′}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{M} \AgdaFunction{·} \AgdaBound{M′}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaFunction{cong₂} \AgdaFunction{\_·\_} \<[19]%
\>[19]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{x∉fv}\AgdaSymbol{)} \AgdaBound{xnbM}\AgdaSymbol{)}\<%
\\
\>[5]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M′}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvS} \AgdaFunction{SortλTermVars} \<[80]%
\>[80]\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{x∉fv}\AgdaSymbol{)} \AgdaBound{xnbM′}\AgdaSymbol{)} \<[98]%
\>[98]\AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·} \AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{M′}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{□}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[55]%
\>[55]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv} \<[68]%
\>[68]\<%
\\
\>[5]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBB≢} \AgdaBound{x≢y} \AgdaBound{xnbM}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \<[37]%
\>[37]\AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}}\<%
\\
\>[5]\AgdaIndent{37}{}\<[37]%
\>[37]\AgdaSymbol{(}\AgdaFunction{lemma-∉} \AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≢y}\AgdaSymbol{)} \AgdaBound{x∉fv}\AgdaSymbol{)}\<%
\\
\>[5]\AgdaIndent{37}{}\<[37]%
\>[37]\AgdaBound{xnbM}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaFunction{⟩} \<[47]%
\>[47]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{ƛ} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩} \<[20]%
\>[20]\<%
\\
\>[5]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{□}\<%
\\
%
\\
\>\AgdaFunction{lemma-substCompositionV} \<[25]%
\>[25]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{N} \AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[5]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \<[39]%
\>[39]\AgdaBound{L}\<%
\\
\>[5]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[5]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{v} \AgdaBound{z}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaDatatype{≡} \AgdaSymbol{(}\AgdaFunction{v} \AgdaBound{z}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ} \<[96]%
\>[96]\<%
\\
\>\AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉yfvL} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z} \<[26]%
\>[26]\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{((}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{x∉yfvL}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{trans≡} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡z}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[18]%
\>[18]\AgdaBound{y≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{no} \<[29]%
\>[29]\AgdaBound{x≢z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z} \<[26]%
\>[26]\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-substnfv} \AgdaSymbol{(}\AgdaFunction{lemma∉fvfvS} \AgdaSymbol{\{}\AgdaFunction{λF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{SortλTermVars}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b∉xs} \AgdaBound{x∉yfvL}\AgdaSymbol{))} \AgdaBound{xnbL}\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[18]%
\>[18]\AgdaBound{y≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{no} \<[29]%
\>[29]\AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{lemma-substNComposition} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaDatatype{≡} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{z} \<[49]%
\>[49]\AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\<%
\\
\>\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M'}\AgdaSymbol{))} \<[49]%
\>[49]\AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaFunction{\_·\_} \AgdaSymbol{(}\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaBound{M'}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \<[49]%
\>[49]\AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-substNComposition} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{x∉y:fvL} \AgdaBound{x∉bL}\AgdaSymbol{)}\<%
\end{code}

Parallel Reduction

\begin{code}%
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Relation} \AgdaFunction{λTerm} \AgdaKeyword{renaming} \AgdaSymbol{(}\_∘\_ \AgdaSymbol{to} \_∘ᵣ\_\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{7} \AgdaDatatype{\_⇉n\_}\<%
\end{code}

\begin{code}%
\>\AgdaKeyword{data} \AgdaDatatype{\_⇉n\_} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nv} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{v} \AgdaBound{x} \AgdaDatatype{⇉n} \AgdaFunction{v} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nƛ} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉n·} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaFunction{·} \AgdaBound{N'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nβ} \AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \<[19]%
\>[19]\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N'} \AgdaFunction{]ₙ}\<%
\end{code}

All lemmas about ⇉n relation must have freshness premises so naive substitution behaves correctly

\begin{code}%
\>\AgdaFunction{lemma⇉nEquiv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）} \AgdaBound{N}\<%
\\
\>\AgdaFunction{lemma⇉nEquiv} \<[14]%
\>[14]\AgdaInductiveConstructor{⇉nv} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nv}\<%
\\
\>\AgdaFunction{lemma⇉nEquiv} \<[14]%
\>[14]\AgdaSymbol{(}\AgdaInductiveConstructor{⇉nƛ} \AgdaBound{M⇉N}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nƛ} \AgdaSymbol{(}\AgdaFunction{lemma⇉nEquiv} \AgdaBound{M⇉N}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma⇉nEquiv} \<[14]%
\>[14]\AgdaSymbol{(}\AgdaInductiveConstructor{⇉n·} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaInductiveConstructor{⇉n·} \AgdaSymbol{(}\AgdaFunction{lemma⇉nEquiv} \AgdaBound{M⇉M'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma⇉nEquiv} \AgdaBound{N⇉N'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma⇉nEquiv} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \<[22]%
\>[22]\<%
\\
\>[9]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{(}\AgdaInductiveConstructor{⇉nβ} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'}\AgdaSymbol{)} \<[51]%
\>[51]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{subst} \<[11]%
\>[11]\AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaFunction{（} \AgdaBound{x} \AgdaFunction{∙} \AgdaBound{y} \AgdaFunction{）} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaDatatype{⇉n} \AgdaBound{X}\AgdaSymbol{)} \<[46]%
\>[46]\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaFunction{lemma-[]Swap} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N'}\AgdaSymbol{\})} \<[48]%
\>[48]\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{⇉nβ} \AgdaSymbol{(}\AgdaFunction{lemma⇉nEquiv} \AgdaBound{M⇉M'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma⇉nEquiv} \AgdaBound{N⇉N'}\AgdaSymbol{))}\<%
\\
\>\AgdaComment{-- }\<%
\\
\>\AgdaFunction{FourλTermF} \AgdaSymbol{=} \<[14]%
\>[14]\AgdaInductiveConstructor{|Ef|} \AgdaFunction{λF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{λF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{λF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{λF} \<[58]%
\>[58]\<%
\\
\>\AgdaFunction{FourλTerm} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaFunction{FourλTermF}\<%
\\
%
\\
\>\AgdaFunction{BVC} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{BVC} \AgdaBound{M} \AgdaSymbol{=} \<[9]%
\>[9]\AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\<%
\\
\>\AgdaFunction{BVCC} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{BVCC} \AgdaBound{M} \AgdaSymbol{=} \AgdaSymbol{(\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}(}\AgdaBound{y∈bM} \AgdaSymbol{:} \AgdaBound{y} \AgdaFunction{∈b} \AgdaBound{M}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{notOccurBindExcept} \AgdaBound{y} \AgdaBound{M} \AgdaBound{y∈bM}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{BVCN} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{BVCN} \AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{BVC} \AgdaBound{M} \AgdaFunction{×} \AgdaFunction{BVCC} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaComment{-- Future Church-Rosser development}\<%
\\
%
\\
\>\AgdaKeyword{postulate}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma⇉nBinders} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∈b} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∈b} \AgdaBound{M}\<%
\\
\>\AgdaComment{-- lemma⇉nBinders = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma⇉nNotBinders} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{N}\<%
\\
\>\AgdaComment{-- lemma⇉nNotBinders = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma⇉nListNotBinders} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaBound{N}\<%
\\
\>\AgdaComment{-- lemma⇉nListNotBinders = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemmaSubstsBVCN} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaSymbol{((}\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \<[65]%
\>[65]\<%
\\
\>\AgdaComment{-- lemmaSubstsBVCN \{z\} \{M\} \{N\} (bvcƛxMN , f) = lemmaSubsts \{z\} \{M\} \{N\} \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma⇉nNotBindersExcept} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaBound{M} \AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaBound{N}\<%
\\
\>\AgdaComment{-- lemma⇉nNotBindersExcept M⇉nN f y∈bN = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma⇉nBVCN} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{N}\<%
\\
\>\AgdaComment{-- lemma⇉nBVCN BVCNM M⇉nN = \{! !\}}\<%
\\
%
\\
\>\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{:} \<[17]%
\>[17]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{N'}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}(}\AgdaBound{y∈bM} \AgdaSymbol{:} \AgdaBound{y} \AgdaFunction{∈b} \AgdaBound{M}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{y} \AgdaFunction{notOccurBind} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N'} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{y} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaBound{nb} \AgdaInductiveConstructor{⇉nv} \<[66]%
\>[66]\AgdaBound{N⇉N'} \AgdaSymbol{\_}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \<[15]%
\>[15]\AgdaBound{N⇉N'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \AgdaSymbol{=} \<[15]%
\>[15]\AgdaInductiveConstructor{⇉nv}\<%
\\
\>\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{P}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaBound{nb} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉n·} \AgdaBound{M⇉M'} \AgdaBound{P⇉P'}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaBound{N⇉N'} \AgdaBound{f}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉n·} \<[9]%
\>[9]\AgdaSymbol{(}\AgdaFunction{lemma-⇉SubstN} \<[25]%
\>[25]\AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'} \AgdaSymbol{(}\AgdaBound{f} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₁} \AgdaFunction{∘} \<[182]%
\>[182]\AgdaInductiveConstructor{∈bFx₁}\AgdaSymbol{))}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))} \AgdaBound{P⇉P'} \AgdaBound{N⇉N'} \AgdaSymbol{(}\AgdaBound{f} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₁} \AgdaFunction{∘} \<[181]%
\>[181]\AgdaInductiveConstructor{∈bFx₂}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaBound{P}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{.\{}\AgdaBound{M'} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{P'} \AgdaFunction{]ₙ}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N'}\AgdaSymbol{\}}\<%
\\
\>[9]\AgdaIndent{46}{}\<[46]%
\>[46]\AgdaBound{nb} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉nβ} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{P}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{P'}\AgdaSymbol{\}} \AgdaBound{M⇉M'} \AgdaBound{P⇉P'}\AgdaSymbol{)} \<[86]%
\>[86]\AgdaBound{N⇉N'} \AgdaBound{f}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{subst} \<[11]%
\>[11]\AgdaSymbol{(λ} \AgdaBound{X} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{))} \AgdaFunction{·} \AgdaSymbol{(}\AgdaBound{P} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaDatatype{⇉n} \AgdaBound{X}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemma-substNComposition} \<[42]%
\>[42]\AgdaSymbol{\{}\AgdaBound{M'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{P'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \<[65]%
\>[65]\<%
\\
\>[11]\AgdaIndent{42}{}\<[42]%
\>[42]\AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv∉fv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))))))} \<[269]%
\>[269]\<%
\\
\>[11]\AgdaIndent{42}{}\<[42]%
\>[42]\AgdaSymbol{(}\AgdaPostulate{lemma⇉nNotBinders} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFx₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaInductiveConstructor{∈bFB≡}\AgdaSymbol{))))))))} \AgdaBound{N⇉N'}\AgdaSymbol{)))} \<[141]%
\>[141]\<%
\\
\>[0]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{⇉nβ} \<[17]%
\>[17]\AgdaSymbol{(}\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))))))} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'} \AgdaSymbol{(}\AgdaBound{f} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₁} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFx₁} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFB}\AgdaSymbol{))}\<%
\\
\>[11]\AgdaIndent{17}{}\<[17]%
\>[17]\AgdaSymbol{(}\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))} \AgdaBound{P⇉P'} \AgdaBound{N⇉N'} \AgdaSymbol{(}\AgdaBound{f} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₁} \AgdaFunction{∘} \<[189]%
\>[189]\AgdaInductiveConstructor{∈bFx₂}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaBound{nb} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉nƛ} \AgdaBound{M⇉M'}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaBound{N⇉N'} \AgdaBound{f}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nƛ} \AgdaSymbol{(}\AgdaFunction{lemma-⇉SubstN} \AgdaSymbol{(}\AgdaFunction{listNotOccurBBinv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBinj₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nb}\AgdaSymbol{))))} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'} \AgdaSymbol{(}\AgdaBound{f} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFR} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFinj₂} \AgdaFunction{∘} \AgdaInductiveConstructor{∈bFB}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaFunction{\_*} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{x} \<[46]%
\>[46]\AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[51]%
\>[51]\AgdaSymbol{=} \AgdaFunction{v} \AgdaBound{x}\<%
\\
\>\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{x} \<[37]%
\>[37]\AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \<[46]%
\>[46]\AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[51]%
\>[51]\AgdaSymbol{=} \AgdaFunction{v} \AgdaBound{x} \<[81]%
\>[81]\AgdaFunction{·} \AgdaBound{N} \AgdaFunction{*}\<%
\\
\>\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M′}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \<[46]%
\>[46]\AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[51]%
\>[51]\AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M′}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[81]%
\>[81]\AgdaFunction{·} \AgdaBound{N} \AgdaFunction{*}\<%
\\
\>\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{M} \AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \<[46]%
\>[46]\AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[51]%
\>[51]\AgdaSymbol{=} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{*}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{*} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \<[46]%
\>[46]\AgdaInductiveConstructor{⟩} \AgdaFunction{*} \<[51]%
\>[51]\AgdaSymbol{=} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{*}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemmaBindersβbinder} \<[21]%
\>[21]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{y} \AgdaFunction{notOccurBind} \AgdaBound{M}\<%
\\
\>\AgdaFunction{lemmaBindersβbinder} \AgdaBound{f} \AgdaKeyword{with} \AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFx₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaInductiveConstructor{∈bFB≡}\AgdaSymbol{)))))))}\<%
\\
\>\AgdaFunction{lemmaBindersβbinder} \AgdaBound{f} \AgdaSymbol{|} \AgdaInductiveConstructor{notOccurBExceptR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptx₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptB≡} \AgdaBound{y∉bM}\AgdaSymbol{))))} \AgdaSymbol{\_)))} \AgdaSymbol{=} \AgdaBound{y∉bM}\<%
\\
%
\\
\>\AgdaFunction{lemmaBindersβ} \<[15]%
\>[15]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∈b} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{N}\<%
\\
\>\AgdaFunction{lemmaBindersβ} \AgdaBound{f} \AgdaBound{x∈} \AgdaKeyword{with} \AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFx₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFR} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∈bFB} \AgdaBound{x∈}\AgdaSymbol{))))))))}\<%
\\
\>\AgdaFunction{lemmaBindersβ} \AgdaBound{f} \AgdaBound{x∈} \AgdaSymbol{|} \AgdaInductiveConstructor{notOccurBExceptR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBExceptx₁} \AgdaBound{nbe} \AgdaBound{xnotOccurBindM}\AgdaSymbol{)))} \AgdaSymbol{=} \AgdaBound{xnotOccurBindM} \<[138]%
\>[138]\<%
\\
%
\\
\>\AgdaFunction{lemmaBinders⇉β} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{M'} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∈b} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{N'}\<%
\\
\>\AgdaFunction{lemmaBinders⇉β} \AgdaBound{f} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'} \AgdaBound{x∈bM'} \AgdaSymbol{=} \<[36]%
\>[36]\AgdaPostulate{lemma⇉nNotBinders} \AgdaSymbol{(}\AgdaFunction{lemmaBindersβ} \AgdaBound{f} \AgdaSymbol{(}\AgdaPostulate{lemma⇉nBinders} \AgdaBound{x∈bM'} \AgdaBound{M⇉M'}\AgdaSymbol{))} \AgdaBound{N⇉N'}\<%
\\
%
\\
\>\AgdaKeyword{postulate} \<[10]%
\>[10]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-⇉nFree} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{fv} \AgdaBound{N} \AgdaFunction{⊆l} \AgdaFunction{fv} \AgdaBound{M}\<%
\\
\>\AgdaComment{-- lemma-⇉nFree = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-⇉nFree*} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{fv} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{*}\AgdaSymbol{)} \AgdaFunction{⊆l} \AgdaFunction{fv} \AgdaBound{M}\<%
\\
\>\AgdaComment{-- lemma-⇉nFree* = \{!!\}}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma*} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{M} \AgdaFunction{*}\<%
\\
\>\AgdaComment{-- lemma*  \_          ⇉nv                      = ⇉nv}\<%
\\
\>\AgdaComment{-- lemma*  (nb , b≢)  (⇉nƛ M⇉N)                = ⇉nƛ  (lemma* (\{!listNotOccurBBinv (listNotOccurBinj₂inv (listNotOccurBinj₂inv (lemmalistNotOccurBindFR→ListNotOccurBindF nb)))!\}  , \{!!\}) M⇉N)}\<%
\\
\>\AgdaComment{-- lemma*  \{⟨ inj₂ (inj₁ (⟨ inj₁ x ⟩ , N)) ⟩\}}\<%
\\
\>\AgdaComment{--         (nb , b≢)  (⇉n· M⇉M' N⇉N')          = ⇉n·  (lemma* (\{!!\} , (λ \{(∈bFR (∈bFinj₁ ()))\})) M⇉M')}\<%
\\
\>\AgdaComment{--                                                    (lemma* (\{!!\} , \{!!\}) N⇉N')}\<%
\\
\>\AgdaComment{-- lemma*  \{⟨ inj₂ (inj₁ (⟨ inj₂ (inj₁ (M , P)) ⟩ , N)) ⟩\}}\<%
\\
\>\AgdaComment{--         (nb , b≢)  (⇉n· M⇉M' N⇉N')          = ⇉n·  (lemma* (\{!!\} , \{!!\}) M⇉M') }\<%
\\
\>\AgdaComment{--                                                    (lemma* (\{!!\} , \{!!\}) N⇉N')}\<%
\\
\>\AgdaComment{-- lemma*  \{⟨ inj₂ (inj₁ (⟨ inj₂ (inj₂ (x , M)) ⟩ , N)) ⟩\}}\<%
\\
\>\AgdaComment{--         (nb , b≢)  (⇉n· (⇉nƛ M⇉M') N⇉N')    = ⇉nβ  (lemma* (\{!!\} , \{!!\}) M⇉M') }\<%
\\
\>\AgdaComment{--                                                    (lemma* (\{!!\} , \{!!\}) N⇉N')   }\<%
\\
\>\AgdaComment{-- lemma*  (nb , b≢)  (⇉nβ \{M = M\} \{N = N\}\{x = y\} M⇉M' N⇉N')  }\<%
\\
\>\AgdaComment{--   = lemma-⇉SubstN  (lemma-binds:cons (lemma⇉nNotBinders (lemmaBindersβbinder b≢) M⇉M') (lemma-binds⊆ (lemma-⇉nFree* \{N\}) (lemma⇉nListNotBinders (listNotOccurBBinv (listNotOccurBinj₂inv (listNotOccurBinj₂inv  (lemmalistNotOccurBindFR→ListNotOccurBindF  (listNotOccurBx₁inv (listNotOccurBinj₁inv (listNotOccurBinj₂inv (lemmalistNotOccurBindFR→ListNotOccurBindF (lemma-binds++r \{xs = fv (ƛ y M)\} nb))))))))) M⇉M')))}\<%
\\
\>\AgdaComment{--                    (lemma* (\{!!\} , \{!!\}) M⇉M')}\<%
\\
\>\AgdaComment{--                    (lemma* (\{!!\} , \{!!\}) N⇉N')}\<%
\\
\>\AgdaComment{--                    (lemmaBinders⇉β b≢ M⇉M' N⇉N') }\<%
\\
%
\\
\>\AgdaFunction{diamBVC⇉n} \AgdaSymbol{:} \<[13]%
\>[13]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{P} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M} \<[38]%
\>[38]\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{P} \AgdaSymbol{→} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{R} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{R} \AgdaFunction{×} \AgdaBound{P} \AgdaDatatype{⇉n} \AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{diamBVC⇉n} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{bvc} \AgdaBound{M⇉N} \AgdaBound{M⇉P} \AgdaSymbol{=} \AgdaBound{M} \AgdaFunction{*} \AgdaInductiveConstructor{,} \AgdaPostulate{lemma*} \AgdaBound{bvc} \AgdaBound{M⇉N} \AgdaInductiveConstructor{,} \AgdaPostulate{lemma*} \AgdaBound{bvc} \AgdaBound{M⇉P}\<%
\end{code}

Next postulate could be done as started in AlphaInduction3 file, all binders distinct, and is used only for Church-Rosser future development.

\begin{code}%
\>\AgdaKeyword{postulate}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-bindersFreeα-BindersAll≢} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \<[71]%
\>[71]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}(}\AgdaBound{x∈be'} \AgdaSymbol{:} \AgdaBound{x} \AgdaFunction{∈b} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{notOccurBindExcept} \AgdaBound{x} \AgdaSymbol{(}\AgdaFunction{bindersFreeα} \AgdaBound{xs} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x∈be'}\AgdaSymbol{))} \<%
\end{code}

\begin{code}%
\>\AgdaFunction{bvcTerm} \AgdaSymbol{:} \AgdaFunction{λTerm} \AgdaSymbol{→} \AgdaFunction{λTerm}\<%
\\
\>\AgdaFunction{bvcTerm} \AgdaSymbol{=} \AgdaFunction{bindersFreeα} \AgdaInductiveConstructor{[]}\<%
\\
%
\\
\>\AgdaFunction{lemma-bvcTermα} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{bvcTerm} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M}\<%
\\
\>\AgdaFunction{lemma-bvcTermα} \AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{lemma-bindersFreeα-α} \AgdaInductiveConstructor{[]} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaFunction{lemmaBVC-bvcTerm} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{BVC} \AgdaSymbol{(}\AgdaFunction{bvcTerm} \AgdaBound{M}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaBVC-bvcTerm} \<[18]%
\>[18]\AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{lemma-bindersFreeα-FV∉b} \AgdaInductiveConstructor{[]} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaFunction{lemmaBVCC-bvcTerm} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{BVCC} \AgdaSymbol{(}\AgdaFunction{bvcTerm} \AgdaBound{M}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaBVCC-bvcTerm} \AgdaBound{M} \AgdaSymbol{=} \AgdaPostulate{lemma-bindersFreeα-BindersAll≢} \AgdaInductiveConstructor{[]} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaFunction{lemmasBVCN} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaSymbol{(}\AgdaFunction{bvcTerm} \AgdaBound{M}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmasBVCN} \AgdaBound{M} \AgdaSymbol{=} \AgdaSymbol{(}\AgdaFunction{lemmaBVC-bvcTerm} \AgdaBound{M}\AgdaSymbol{)} \AgdaInductiveConstructor{,} \AgdaSymbol{(}\AgdaFunction{lemmaBVCC-bvcTerm} \AgdaBound{M}\AgdaSymbol{)} \<[60]%
\>[60]\<%
\\
%
\\
\>\AgdaKeyword{postulate} \<[10]%
\>[10]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-⇉nleftα} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M'} \<[23]%
\>[23]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaBound{M'} \AgdaFunction{∼α} \AgdaBound{M}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{N'} \AgdaSymbol{→} \AgdaBound{M'} \AgdaDatatype{⇉n} \AgdaBound{N'} \AgdaFunction{×} \AgdaBound{N'} \AgdaFunction{∼α} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>\AgdaComment{-- lemma-⇉nleftα  BVCNM BVCM' }\<%
\\
\>\AgdaComment{--                (∼αR (∼α+₁ (∼αV \{x\})))                            }\<%
\\
\>\AgdaComment{--                ⇉nv }\<%
\\
\>\AgdaComment{--   = v x , ⇉nv , ∼αR (∼α+₁ ∼αV)}\<%
\\
\>\AgdaComment{-- lemma-⇉nleftα  BVCNM BVCM' }\<%
\\
\>\AgdaComment{--                (∼αR (∼α+₂ (∼α+₂ \{e = y , N\} \{x , M\} (∼αB xs f))))  }\<%
\\
\>\AgdaComment{--                (⇉nƛ M⇉nM') }\<%
\\
\>\AgdaComment{--   with lemma∼Bswap \{S = SortλTermVars\} \{y\} \{x\} \{N\} \{M\} (∼αB xs f)}\<%
\\
\>\AgdaComment{-- ... | （yx）N∼M}\<%
\\
\>\AgdaComment{--   with lemma-⇉nleftα \{!!\} \{!!\} （yx）N∼M  M⇉nM'}\<%
\\
\>\AgdaComment{-- ... | N' , （yx）N⇉nN' , N'∼N }\<%
\\
\>\AgdaComment{--   = \{! （yx）M'∼M!\}}\<%
\\
\>\AgdaComment{-- lemma-⇉nleftα BVCNM BVCM' M'∼M (⇉n· M⇉nN M⇉nN₁) = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma-⇉nleftα BVCNM BVCM' M'∼M (⇉nβ M⇉nN M⇉nN₁) = \{!!\}}\<%
\end{code}


-- Another approach

\begin{code}%
\>\AgdaKeyword{infix} \AgdaNumber{7} \AgdaFunction{\_⇉\_}\<%
\\
%
\\
\>\AgdaFunction{\_⇉\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaBound{M} \AgdaFunction{⇉} \AgdaBound{N} \AgdaSymbol{=} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M'} \AgdaFunction{×} \AgdaFunction{BVCN} \AgdaBound{M'} \AgdaFunction{×} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{N'} \AgdaSymbol{→} \AgdaBound{N'} \AgdaFunction{∼α} \AgdaBound{N} \AgdaFunction{×} \AgdaBound{M'} \AgdaDatatype{⇉n} \AgdaBound{N'}\AgdaSymbol{))}\<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemma-⇉rightα} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{P} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{⇉} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{P} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{⇉} \AgdaBound{P}\<%
\\
\>\AgdaFunction{lemma-⇉rightα} \<[15]%
\>[15]\AgdaSymbol{(}\AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉N'}\AgdaSymbol{)} \AgdaBound{N∼P} \<[59]%
\>[59]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaFunction{τ} \AgdaBound{N'∼N} \AgdaBound{N∼P} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉N'}\<%
\\
%
\\
\>\AgdaFunction{lemma-⇉leftα} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{P} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{P} \AgdaFunction{∼α} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{⇉} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{P} \AgdaFunction{⇉} \AgdaBound{N}\<%
\\
\>\AgdaFunction{lemma-⇉leftα} \AgdaBound{P∼M} \AgdaSymbol{(}\AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉N'}\AgdaSymbol{)} \<[57]%
\>[57]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaFunction{τ} \AgdaBound{P∼M} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉N'} \<[48]%
\>[48]\<%
\\
%
\\
\>\AgdaFunction{ρ⇉n} \AgdaSymbol{:} \AgdaFunction{Reflexive} \AgdaSymbol{(}\AgdaDatatype{\_⇉n\_}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{ρ⇉n} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{x} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nv}\<%
\\
\>\AgdaFunction{ρ⇉n} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉n·} \AgdaFunction{ρ⇉n} \AgdaFunction{ρ⇉n}\<%
\\
\>\AgdaFunction{ρ⇉n} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nƛ} \AgdaFunction{ρ⇉n}\<%
\\
%
\\
\>\AgdaFunction{ρ⇉} \AgdaSymbol{:} \AgdaFunction{Reflexive} \AgdaSymbol{(}\AgdaFunction{\_⇉\_}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{ρ⇉} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{M'} \AgdaInductiveConstructor{,} \AgdaFunction{σ} \AgdaFunction{M'∼M} \AgdaInductiveConstructor{,} \AgdaFunction{BVCNM'} \AgdaInductiveConstructor{,} \AgdaFunction{M'} \AgdaInductiveConstructor{,} \AgdaFunction{M'∼M} \AgdaInductiveConstructor{,} \AgdaFunction{ρ⇉n} \<[48]%
\>[48]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{M'} \AgdaSymbol{=} \AgdaFunction{bvcTerm} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{M'∼M} \AgdaSymbol{=} \AgdaFunction{lemma-bvcTermα} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{BVCNM'} \AgdaSymbol{=} \AgdaFunction{lemmasBVCN} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaFunction{diam⇉} \AgdaSymbol{:} \AgdaFunction{diamond} \AgdaSymbol{(}\AgdaFunction{\_⇉\_}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{diam⇉} \<[7]%
\>[7]\AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{P}\AgdaSymbol{\}} \<[19]%
\>[19]\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M'} \AgdaInductiveConstructor{,} \<[14]%
\>[14]\AgdaBound{M∼M'} \<[21]%
\>[21]\AgdaInductiveConstructor{,} \AgdaBound{BVCM'} \<[31]%
\>[31]\AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉nN'}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M''} \AgdaInductiveConstructor{,} \AgdaBound{M∼M''} \<[21]%
\>[21]\AgdaInductiveConstructor{,} \AgdaBound{BVCM''} \<[31]%
\>[31]\AgdaInductiveConstructor{,} \AgdaBound{P'} \AgdaInductiveConstructor{,} \AgdaBound{P'∼P} \AgdaInductiveConstructor{,} \AgdaBound{M''⇉nP'}\AgdaSymbol{)} \<[54]%
\>[54]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaPostulate{lemma-⇉nleftα} \AgdaBound{BVCM''} \AgdaBound{BVCM'} \AgdaSymbol{(}\AgdaFunction{τ} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaBound{M∼M'}\AgdaSymbol{)} \AgdaBound{M∼M''}\AgdaSymbol{)} \AgdaBound{M''⇉nP'} \<[62]%
\>[62]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{P''} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉nP''} \AgdaInductiveConstructor{,} \AgdaBound{P''∼P'} \<[33]%
\>[33]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{diamBVC⇉n} \AgdaBound{BVCM'} \AgdaBound{M'⇉nN'} \AgdaBound{M'⇉nP''}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaBound{R} \AgdaInductiveConstructor{,} \AgdaBound{N'⇉nR} \AgdaInductiveConstructor{,} \AgdaBound{P''⇉nR}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaBound{R} \<[80]%
\>[80]\AgdaInductiveConstructor{,} \<[82]%
\>[82]\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{(}\AgdaBound{N'} \<[11]%
\>[11]\AgdaInductiveConstructor{,} \AgdaFunction{σ} \AgdaBound{N'∼N} \<[32]%
\>[32]\AgdaInductiveConstructor{,} \AgdaPostulate{lemma⇉nBVCN} \AgdaBound{BVCM'} \AgdaBound{M'⇉nN'} \<[61]%
\>[61]\AgdaInductiveConstructor{,} \AgdaBound{R} \AgdaInductiveConstructor{,} \AgdaFunction{ρ} \AgdaInductiveConstructor{,} \AgdaBound{N'⇉nR} \AgdaSymbol{)} \<[80]%
\>[80]\AgdaInductiveConstructor{,} \<[83]%
\>[83]\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{(}\AgdaBound{P''} \<[11]%
\>[11]\AgdaInductiveConstructor{,} \AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{τ} \AgdaBound{P''∼P'} \AgdaBound{P'∼P}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaInductiveConstructor{,} \AgdaPostulate{lemma⇉nBVCN} \AgdaBound{BVCM'} \AgdaBound{M'⇉nP''} \<[61]%
\>[61]\AgdaInductiveConstructor{,} \AgdaBound{R} \AgdaInductiveConstructor{,} \AgdaFunction{ρ} \AgdaInductiveConstructor{,} \AgdaBound{P''⇉nR}\AgdaSymbol{)}\<%
\end{code}


Ctx can be done generically

\begin{code}%
\>\AgdaKeyword{data} \AgdaDatatype{ctx} \AgdaSymbol{(}\AgdaBound{r} \AgdaSymbol{:} \AgdaFunction{Rel}\AgdaSymbol{)} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{ctxinj} \AgdaSymbol{:} \AgdaSymbol{∀} \AgdaSymbol{\{}\AgdaBound{t} \AgdaBound{t'}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{→} \AgdaBound{r} \AgdaBound{t} \AgdaBound{t'} \<[42]%
\>[42]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaBound{t} \AgdaBound{t'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{ctx·l} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaSymbol{∀} \AgdaSymbol{\{}\AgdaBound{t₁} \AgdaBound{t₁'} \AgdaBound{t₂}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaBound{t₁} \AgdaBound{t₁'} \<[42]%
\>[42]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaFunction{·} \AgdaBound{t₂}\AgdaSymbol{)} \<[62]%
\>[62]\AgdaSymbol{(}\AgdaBound{t₁'} \AgdaFunction{·} \AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{ctx·r} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaSymbol{∀} \AgdaSymbol{\{}\AgdaBound{t₁} \AgdaBound{t₂} \AgdaBound{t₂'}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaBound{t₂} \AgdaBound{t₂'} \<[42]%
\>[42]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaFunction{·} \AgdaBound{t₂}\AgdaSymbol{)} \<[62]%
\>[62]\AgdaSymbol{(}\AgdaBound{t₁} \AgdaFunction{·} \AgdaBound{t₂'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{ctxƛ} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaSymbol{∀} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{t₁} \AgdaBound{t₁'}\AgdaSymbol{\}} \<[26]%
\>[26]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaBound{t₁} \AgdaBound{t₁'} \<[42]%
\>[42]\AgdaSymbol{→} \AgdaDatatype{ctx} \AgdaBound{r} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{t₁}\AgdaSymbol{)} \<[62]%
\>[62]\AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{t₁'}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{1} \AgdaDatatype{\_▹n\_} \<[13]%
\>[13]\<%
\\
\>\AgdaKeyword{data} \AgdaDatatype{\_▹n\_} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{▹βn} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{→} \<[9]%
\>[9]\AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{▹n} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{1} \AgdaDatatype{\_▹\_} \<[12]%
\>[12]\<%
\\
\>\AgdaKeyword{data} \AgdaDatatype{\_▹\_} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{▹β} \<[6]%
\>[6]\AgdaSymbol{:} \<[9]%
\>[9]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{→} \<[9]%
\>[9]\AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{▹} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→βn\_}\<%
\\
\>\AgdaFunction{\_→βn\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{\_→βn\_} \AgdaSymbol{=} \AgdaDatatype{ctx} \AgdaDatatype{\_▹n\_}\<%
\\
%
\\
\>\AgdaFunction{BVCNRel} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaSymbol{→} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{BVCNRel} \AgdaBound{R} \AgdaBound{M} \AgdaBound{N} \AgdaSymbol{=} \AgdaFunction{BVCN} \AgdaBound{M} \AgdaFunction{×} \AgdaBound{R} \AgdaBound{M} \AgdaBound{N}\<%
\\
%
\\
\>\AgdaComment{-- lemma▹n⊆▹ : BVCNRel \_▹n\_ ⊆ (\_▹\_ ∘ᵣ \_∼α\_)}\<%
\\
\>\AgdaComment{-- lemma▹n⊆▹ (BVCN , M▹nN) = \{!!\} }\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→βn*\_}\<%
\\
\>\AgdaFunction{\_→βn*\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{\_→βn*\_} \AgdaSymbol{=} \AgdaDatatype{star} \AgdaFunction{\_→βn\_}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→β\_}\<%
\\
\>\AgdaFunction{\_→β\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaBound{M} \AgdaFunction{→β} \AgdaBound{N} \AgdaSymbol{=} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M'} \AgdaFunction{×} \AgdaFunction{BVCN} \AgdaBound{M'} \AgdaFunction{×} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{N'} \AgdaSymbol{→} \AgdaBound{N'} \AgdaFunction{∼α} \AgdaBound{N} \AgdaFunction{×} \AgdaBound{M'} \AgdaFunction{→βn} \AgdaBound{N'}\AgdaSymbol{))} \<[71]%
\>[71]\<%
\\
%
\\
\>\AgdaComment{-- Real one}\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→βR\_}\<%
\\
\>\AgdaFunction{\_→βR\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaBound{M} \AgdaFunction{→βR} \AgdaBound{N} \AgdaSymbol{=} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M'} \AgdaFunction{×} \AgdaFunction{∃} \AgdaSymbol{(λ} \AgdaBound{N'} \AgdaSymbol{→} \AgdaBound{N'} \AgdaFunction{∼α} \AgdaBound{N} \AgdaFunction{×} \AgdaSymbol{(}\AgdaDatatype{ctx} \AgdaDatatype{\_▹\_}\AgdaSymbol{)} \AgdaBound{M'} \AgdaBound{N'}\AgdaSymbol{))} \<[68]%
\>[68]\<%
\\
%
\\
\>\AgdaKeyword{postulate}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma→β⊆→βR} \AgdaSymbol{:} \AgdaFunction{\_→β\_} \AgdaFunction{⊆} \AgdaFunction{\_→βR\_}\<%
\\
\>\AgdaComment{-- lemma→β⊆→βR (M' , M∼M' , BVCM' , N' , N'∼N , M'→βnN') = M' , M∼M' , N' , N'∼N , \{!!\} }\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma→βR⊆→β} \AgdaSymbol{:} \AgdaFunction{\_→βR\_} \AgdaFunction{⊆} \AgdaFunction{\_→β\_}\<%
\\
\>\AgdaComment{-- lemma→βR⊆→β (M' , M∼M' , N' , N'∼N , M'→βRN') = \{!!\}}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→α\_} \<[13]%
\>[13]\<%
\\
\>\AgdaFunction{\_→α\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{\_→α\_} \AgdaSymbol{=} \AgdaFunction{\_→β\_} \AgdaFunction{∪} \AgdaFunction{\_∼α\_}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→α*\_}\<%
\\
\>\AgdaFunction{\_→α*\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{\_→α*\_} \AgdaSymbol{=} \AgdaDatatype{star} \AgdaFunction{\_→α\_}\<%
\\
%
\\
\>\AgdaFunction{lemmaBVCN→βn⊆→β} \AgdaSymbol{:} \AgdaFunction{BVCNRel} \AgdaFunction{\_→βn\_} \AgdaFunction{⊆} \AgdaFunction{\_→β\_}\<%
\\
\>\AgdaFunction{lemmaBVCN→βn⊆→β} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{BVCNM} \AgdaInductiveConstructor{,} \AgdaBound{M→βnN}\AgdaSymbol{)} \AgdaSymbol{=} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaFunction{ρ} \AgdaInductiveConstructor{,} \AgdaBound{BVCNM} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaFunction{ρ} \AgdaInductiveConstructor{,} \AgdaBound{M→βnN} \<[72]%
\>[72]\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{4} \AgdaFunction{\_→β*\_}\<%
\\
\>\AgdaFunction{\_→β*\_} \AgdaSymbol{:} \AgdaFunction{Rel}\<%
\\
\>\AgdaFunction{\_→β*\_} \AgdaSymbol{=} \AgdaDatatype{star} \AgdaFunction{\_→β\_}\<%
\\
%
\\
\>\AgdaFunction{lemma→α*α} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M'} \AgdaFunction{∼α} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{N'} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→α*} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{M'} \AgdaFunction{→α*} \AgdaBound{N'}\<%
\\
\>\AgdaFunction{lemma→α*α} \AgdaBound{M'∼M} \AgdaBound{N∼N'} \AgdaInductiveConstructor{refl} \<[41]%
\>[41]\AgdaSymbol{=} \AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{τ} \AgdaBound{M'∼M} \AgdaBound{N∼N'}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma→α*α} \AgdaBound{M'∼M} \AgdaBound{N∼N'} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→αN}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{M'∼M}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→αN}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{N∼N'}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma→α*α} \AgdaBound{M'∼M} \AgdaBound{N∼N'} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaBound{M→α*N} \AgdaBound{N→α*P}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→α*α} \AgdaBound{M'∼M} \AgdaFunction{ρ} \AgdaBound{M→α*N}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma→α*α} \AgdaFunction{ρ} \AgdaBound{N∼N'} \AgdaBound{N→α*P}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{postulate}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-BVCN→βn*} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{N}\<%
\\
\>\AgdaComment{-- lemma-BVCN→βn* = \{!!\}}\<%
\\
%
\\
\>\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{BVCN} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{N} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→β*} \AgdaBound{N}\<%
\\
\>\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaBound{BVCM} \AgdaInductiveConstructor{refl} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaBound{BVCM} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaFunction{lemmaBVCN→βn⊆→β} \AgdaSymbol{(}\AgdaBound{BVCM} \AgdaInductiveConstructor{,} \AgdaBound{M→βnN}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaBound{BVCM} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaBound{M→βn*N} \AgdaBound{N→βn*P}\AgdaSymbol{)} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaBound{BVCM} \AgdaBound{M→βn*N}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaSymbol{(}\AgdaPostulate{lemma-BVCN→βn*} \AgdaBound{BVCM} \AgdaBound{M→βn*N}\AgdaSymbol{)} \AgdaBound{N→βn*P}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn*ƛ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{N} \AgdaSymbol{→} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{N}\<%
\\
\>\AgdaFunction{lemma→βn*ƛ} \AgdaInductiveConstructor{refl} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma→βn*ƛ} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{ctxƛ} \AgdaBound{M→βnN}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma→βn*ƛ} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaBound{M→βnN} \AgdaBound{N→βnP}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→βn*ƛ} \AgdaBound{M→βnN}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma→βn*ƛ} \AgdaBound{N→βnP}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn*·l} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{M'} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaFunction{→βn*} \AgdaSymbol{(}\AgdaBound{M'} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma→βn*·l} \AgdaInductiveConstructor{refl} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma→βn*·l} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{ctx·l} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[54]%
\>[54]\<%
\\
\>\AgdaFunction{lemma→βn*·l} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaBound{M→βnN} \AgdaBound{N→βnP}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·l} \AgdaBound{M→βnN}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·l} \AgdaBound{N→βnP}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn*·r} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{→βn*} \AgdaBound{N'} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaFunction{→βn*} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma→βn*·r} \AgdaInductiveConstructor{refl} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma→βn*·r} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{ctx·r} \AgdaBound{M→βnN}\AgdaSymbol{)} \<[54]%
\>[54]\<%
\\
\>\AgdaFunction{lemma→βn*·r} \AgdaSymbol{(}\AgdaInductiveConstructor{trans} \AgdaBound{M→βnN} \AgdaBound{N→βnP}\AgdaSymbol{)} \<[33]%
\>[33]\AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·r} \AgdaBound{M→βnN}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·r} \AgdaBound{N→βnP}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn*·} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{→βn*} \AgdaBound{N'} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaFunction{→βn*} \AgdaSymbol{(}\AgdaBound{M'} \AgdaFunction{·} \AgdaBound{N'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma→βn*·} \AgdaBound{M→βn*M'} \AgdaBound{N→βn*N'} \AgdaSymbol{=} \AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·l} \AgdaBound{M→βn*M'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·r} \AgdaBound{N→βn*N'}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn*β} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{λTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{→βn*} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{→βn*} \AgdaBound{N'} \AgdaSymbol{→} \AgdaSymbol{((}\AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{·} \AgdaBound{N}\AgdaSymbol{)} \AgdaFunction{→βn*} \AgdaSymbol{(}\AgdaBound{M'} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N'} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma→βn*β} \AgdaBound{M→βn*M'} \AgdaBound{N→βn*N'} \AgdaSymbol{=} \<[30]%
\>[30]\AgdaInductiveConstructor{trans} \AgdaSymbol{(}\AgdaFunction{lemma→βn*·} \AgdaSymbol{(}\AgdaFunction{lemma→βn*ƛ} \AgdaBound{M→βn*M'}\AgdaSymbol{)} \AgdaBound{N→βn*N'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{just} \AgdaSymbol{(}\AgdaInductiveConstructor{ctxinj} \AgdaInductiveConstructor{▹βn}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaFunction{lemma→βn⊆⇉n} \AgdaSymbol{:} \AgdaFunction{\_→βn\_} \AgdaFunction{⊆} \AgdaDatatype{\_⇉n\_}\<%
\\
\>\AgdaFunction{lemma→βn⊆⇉n} \AgdaSymbol{(}\AgdaInductiveConstructor{ctxinj} \AgdaInductiveConstructor{▹βn}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nβ} \<[33]%
\>[33]\AgdaFunction{ρ⇉n} \AgdaFunction{ρ⇉n}\<%
\\
\>\AgdaFunction{lemma→βn⊆⇉n} \AgdaSymbol{(}\AgdaInductiveConstructor{ctx·l} \AgdaBound{r}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉n·} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaFunction{lemma→βn⊆⇉n} \AgdaBound{r}\AgdaSymbol{)} \AgdaFunction{ρ⇉n}\<%
\\
\>\AgdaFunction{lemma→βn⊆⇉n} \AgdaSymbol{(}\AgdaInductiveConstructor{ctx·r} \AgdaBound{r}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉n·} \<[33]%
\>[33]\AgdaFunction{ρ⇉n} \AgdaSymbol{(}\AgdaFunction{lemma→βn⊆⇉n} \AgdaBound{r}\AgdaSymbol{)} \<[53]%
\>[53]\<%
\\
\>\AgdaFunction{lemma→βn⊆⇉n} \AgdaSymbol{(}\AgdaInductiveConstructor{ctxƛ} \AgdaBound{r}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaSymbol{=} \AgdaInductiveConstructor{⇉nƛ} \<[33]%
\>[33]\AgdaSymbol{(}\AgdaFunction{lemma→βn⊆⇉n} \AgdaBound{r}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaComment{-- open ∼-Reasoning(λF)}\<%
\\
%
\\
\>\AgdaComment{-- lemma-λxMN⇉M[x:=N] : (M N : λTerm)(x : V) → ƛ x M · N ⇉ M [ x ≔ N ] }\<%
\\
\>\AgdaComment{-- lemma-λxMN⇉M[x:=N] M N x }\<%
\\
\>\AgdaComment{--   with bvcTerm (ƛ x M · N) | lemma-bvcTermα (ƛ x M · N) | lemmaBVC-bvcTerm (ƛ x M · N) | lemmaBVCC-bvcTerm (ƛ x M · N)}\<%
\\
\>\AgdaComment{-- ...  | ⟨ (inj₂ (inj₁ (  ⟨ inj₂ (inj₂ (y , M')) ⟩  , N'))) ⟩  }\<%
\\
\>\AgdaComment{--      | (∼αR (∼α+₂ (∼α+₁ (∼αx (∼αR (∼α+₂ (∼α+₂ (∼αB xs f))))  N'∼N)))) }\<%
\\
\>\AgdaComment{--      | bvc | bvcc}\<%
\\
\>\AgdaComment{--   =  M' [ y ≔ N' ]ₙ          , }\<%
\\
\>\AgdaComment{--      ⇉nβ ρ⇉n ρ⇉n             ,}\<%
\\
\>\AgdaComment{--      (begin}\<%
\\
\>\AgdaComment{--           M'  [ y ≔ N'  ]ₙ}\<%
\\
\>\AgdaComment{--         ∼⟨ σ (lemmaSubsts \{y\} \{M'\} \{N'\} \{!!\}) ⟩}\<%
\\
\>\AgdaComment{--           M'  [ y ≔ N'  ]}\<%
\\
\>\AgdaComment{--         ∼⟨  \{!!\}  ⟩}\<%
\\
\>\AgdaComment{--           (swap SortλTermVars y x M') [ x ≔ N' ]}\<%
\\
\>\AgdaComment{--         ∼⟨ lemma-substα′ \{x\} \{swap SortλTermVars y x M'\} \{N'\} \{N\} N'∼N ⟩}\<%
\\
\>\AgdaComment{--           (swap SortλTermVars y x M') [ x ≔ N  ]}\<%
\\
\>\AgdaComment{--         ≈⟨ lemma-substα \{swap SortλTermVars y x M'\} \{M\} \{N\} \{x\} (lemma∼Bswap \{x = y\} \{x\} \{M'\} \{M\} (∼αB xs f)) ⟩}\<%
\\
\>\AgdaComment{--           M   [ x ≔ N   ]}\<%
\\
\>\AgdaComment{--      ∎)                     }\<%
\\
%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctxinj (▹β \{M\} \{N\} \{x\})))  = lemma-λxMN⇉M[x:=N] M N x}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctx·l M→αM'))              = lemma-⇉· (lemma→α⊆⇉  (inj₁ M→αM')) ρ⇉}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctx·r N→αN'))              = lemma-⇉· ρ⇉ (lemma→α⊆⇉  (inj₁ N→αN')) }\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctxƛ M→αM'))               = lemma-⇉λ (lemma→α⊆⇉  (inj₁ M→αM'))}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₂ (∼αR f))                    = lemma-⇉rightα ρ⇉ (∼αR f) }\<%
\\
%
\\
\>\AgdaFunction{lemma⇉n⊆→βn*} \AgdaSymbol{:} \AgdaDatatype{\_⇉n\_} \AgdaFunction{⊆} \AgdaFunction{\_→βn*\_}\<%
\\
\>\AgdaFunction{lemma⇉n⊆→βn*} \AgdaInductiveConstructor{⇉nv} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma⇉n⊆→βn*} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉nƛ} \AgdaBound{M⇉M'}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaFunction{lemma→βn*ƛ} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{M⇉M'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma⇉n⊆→βn*} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉n·} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaFunction{lemma→βn*·} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{M⇉M'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{N⇉N'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma⇉n⊆→βn*} \AgdaSymbol{(}\AgdaInductiveConstructor{⇉nβ} \AgdaBound{M⇉M'} \AgdaBound{N⇉N'}\AgdaSymbol{)} \<[30]%
\>[30]\AgdaSymbol{=} \AgdaFunction{lemma→βn*β} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{M⇉M'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{N⇉N'}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{postulate}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaPostulate{lemma-CR⇉n} \AgdaSymbol{:} \AgdaFunction{cr} \AgdaSymbol{(}\AgdaDatatype{\_⇉n\_}\AgdaSymbol{)}\<%
\\
\>\AgdaComment{-- lemma-CR⇉n = diamond-cr \{!diamBVC⇉n!\} --}\<%
\\
%
\\
\>\AgdaFunction{lemma-CR→βn} \AgdaSymbol{:} \AgdaFunction{cr} \AgdaFunction{\_→βn\_}\<%
\\
\>\AgdaFunction{lemma-CR→βn} \AgdaSymbol{=} \AgdaFunction{cr-⊆} \AgdaFunction{lemma→βn⊆⇉n} \AgdaFunction{lemma⇉n⊆→βn*} \AgdaPostulate{lemma-CR⇉n}\<%
\\
%
\\
\>\AgdaFunction{lemma→β⊆⇉} \AgdaSymbol{:} \AgdaFunction{\_→β\_} \AgdaFunction{⊆} \AgdaFunction{\_⇉\_}\<%
\\
\>\AgdaFunction{lemma→β⊆⇉} \AgdaSymbol{(}\AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCNM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'→βN'}\AgdaSymbol{)} \<[52]%
\>[52]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCNM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaFunction{lemma→βn⊆⇉n} \AgdaBound{M'→βN'}\<%
\\
%
\\
\>\AgdaFunction{lemma∼α⊆⇉} \AgdaSymbol{:} \AgdaFunction{\_∼α\_} \AgdaFunction{⊆} \AgdaFunction{\_⇉\_}\<%
\\
\>\AgdaFunction{lemma∼α⊆⇉} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaBound{M∼N} \AgdaSymbol{=} \<[25]%
\>[25]\AgdaFunction{M'} \AgdaInductiveConstructor{,} \AgdaFunction{σ} \AgdaFunction{M'∼M} \AgdaInductiveConstructor{,} \AgdaFunction{BVCNM'} \AgdaInductiveConstructor{,} \<[49]%
\>[49]\AgdaFunction{M'} \AgdaInductiveConstructor{,} \AgdaFunction{τ} \AgdaFunction{M'∼M} \AgdaBound{M∼N} \AgdaInductiveConstructor{,} \AgdaFunction{ρ⇉n}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{M'} \AgdaSymbol{=} \AgdaFunction{bvcTerm} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{M'∼M} \AgdaSymbol{=} \AgdaFunction{lemma-bvcTermα} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{BVCNM'} \AgdaSymbol{=} \AgdaFunction{lemmasBVCN} \AgdaBound{M}\<%
\\
%
\\
\>\AgdaFunction{lemma→α⊆⇉} \AgdaSymbol{:} \AgdaFunction{\_→α\_} \AgdaFunction{⊆} \AgdaFunction{\_⇉\_}\<%
\\
\>\AgdaFunction{lemma→α⊆⇉} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{M→βN}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaSymbol{=} \AgdaFunction{lemma→β⊆⇉} \AgdaBound{M→βN}\<%
\\
\>\AgdaFunction{lemma→α⊆⇉} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{M∼N}\AgdaSymbol{)} \<[23]%
\>[23]\AgdaSymbol{=} \AgdaFunction{lemma∼α⊆⇉} \AgdaBound{M∼N}\<%
\\
%
\\
\>\AgdaFunction{lemma→β⊆→α} \AgdaSymbol{:} \<[14]%
\>[14]\AgdaFunction{\_→β\_} \AgdaFunction{⊆} \AgdaFunction{\_→α\_}\<%
\\
\>\AgdaFunction{lemma→β⊆→α} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₁}\<%
\\
%
\\
\>\AgdaFunction{lemma⇉⊆→α*} \AgdaSymbol{:} \AgdaFunction{\_⇉\_} \AgdaFunction{⊆} \AgdaFunction{\_→α*\_}\<%
\\
\>\AgdaFunction{lemma⇉⊆→α*} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{M'} \AgdaInductiveConstructor{,} \AgdaBound{M∼M'} \AgdaInductiveConstructor{,} \AgdaBound{BVCNM'} \AgdaInductiveConstructor{,} \AgdaBound{N'} \AgdaInductiveConstructor{,} \AgdaBound{N'∼N} \AgdaInductiveConstructor{,} \AgdaBound{M'⇉nN'}\AgdaSymbol{)} \<[61]%
\>[61]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma→α*α} \AgdaBound{M∼M'} \AgdaBound{N'∼N} \AgdaSymbol{(}\AgdaFunction{mon-star} \AgdaFunction{lemma→β⊆→α} \AgdaSymbol{(}\AgdaFunction{lemmaBVCN→βn*⊆→β*} \AgdaBound{BVCNM'} \AgdaSymbol{(}\AgdaFunction{lemma⇉n⊆→βn*} \AgdaBound{M'⇉nN'}\AgdaSymbol{)))} \<[95]%
\>[95]\<%
\\
%
\\
\>\AgdaFunction{lemma-CR⇉} \AgdaSymbol{:} \AgdaFunction{cr} \AgdaFunction{\_⇉\_}\<%
\\
\>\AgdaFunction{lemma-CR⇉} \AgdaSymbol{=} \AgdaFunction{diamond-cr} \AgdaFunction{diam⇉}\<%
\\
%
\\
\>\AgdaFunction{lemma-CR→β} \AgdaSymbol{:} \AgdaFunction{cr} \AgdaFunction{\_→α\_}\<%
\\
\>\AgdaFunction{lemma-CR→β} \AgdaSymbol{=} \AgdaFunction{cr-⊆} \AgdaFunction{lemma→α⊆⇉} \AgdaFunction{lemma⇉⊆→α*} \AgdaFunction{lemma-CR⇉}\<%
\end{code}





==> GenericProgramming/Examples/SystemF.tex <==
System F, Nominal syntax

\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{Examples.SystemF} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{Rel}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Function}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{fold}\AgdaSymbol{;}\AgdaPrimitive{\_*\_}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat.Properties}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{unfold}\AgdaSymbol{;}\AgdaFunction{[\_]}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.All}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaSymbol{as} \AgdaModule{PropEq} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]} \AgdaSymbol{to} \AgdaInductiveConstructor{[\_]ᵢ}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{PropEq.}\AgdaModule{≡-Reasoning} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{begin\_} \AgdaSymbol{to} \AgdaFunction{begin≡\_}\AgdaSymbol{;}\AgdaFunction{\_∎} \AgdaSymbol{to} \AgdaFunction{\_□}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.Any} \AgdaSymbol{as} \AgdaModule{Any} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{tail}\AgdaSymbol{;}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{Any.}\AgdaModule{Membership-≡} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{\_⊆\_}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{GPBindings}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Atom}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Swap}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Fresh}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{FreeVariables}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Alpha}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{AlphaInduction}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{OccurBind}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{List.ListProperties}\<%
\\
%
\\
\>\AgdaFunction{SortFTypeVars} \AgdaSymbol{:} \AgdaFunction{Sort}\<%
\\
\>\AgdaFunction{SortFTypeVars} \AgdaSymbol{=} \AgdaNumber{1}\<%
\\
%
\\
\>\AgdaFunction{SortFTermVars} \AgdaSymbol{:} \AgdaFunction{Sort}\<%
\\
\>\AgdaFunction{SortFTermVars} \AgdaSymbol{=} \AgdaNumber{2}\<%
\end{code}

%<*systemF>
\begin{code}%
\>\AgdaFunction{tyF} \AgdaSymbol{:} \AgdaDatatype{Functor} \<[51]%
\>[51]\AgdaComment{-- t,r :-}\<%
\\
\>\AgdaFunction{tyF} \AgdaSymbol{=} \<[11]%
\>[11]\AgdaInductiveConstructor{|v|} \AgdaFunction{SortFTypeVars} \<[51]%
\>[51]\AgdaComment{--   α}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaInductiveConstructor{|+|} \<[11]%
\>[11]\AgdaInductiveConstructor{|R|} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|R|} \<[51]%
\>[51]\AgdaComment{-- | t → r}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaInductiveConstructor{|+|} \<[11]%
\>[11]\AgdaInductiveConstructor{|B|} \AgdaFunction{SortFTypeVars} \AgdaInductiveConstructor{|R|} \<[51]%
\>[51]\AgdaComment{-- | ∀ α . t}\<%
\\
%
\\
\>\AgdaFunction{tF} \AgdaSymbol{:} \AgdaDatatype{Functor} \<[51]%
\>[51]\AgdaComment{-- M,N :-}\<%
\\
\>\AgdaFunction{tF} \AgdaSymbol{=} \<[10]%
\>[10]\AgdaInductiveConstructor{|v|} \AgdaFunction{SortFTermVars} \<[51]%
\>[51]\AgdaComment{--   x}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|R|} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|R|} \<[51]%
\>[51]\AgdaComment{-- | M N}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|Ef|} \AgdaFunction{tyF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|B|} \AgdaFunction{SortFTermVars} \AgdaInductiveConstructor{|R|} \<[51]%
\>[51]\AgdaComment{-- | λ x : t . M}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|R|} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{tyF} \<[51]%
\>[51]\AgdaComment{-- | M t}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaInductiveConstructor{|+|} \<[10]%
\>[10]\AgdaInductiveConstructor{|B|} \AgdaFunction{SortFTypeVars} \AgdaInductiveConstructor{|R|} \<[51]%
\>[51]\AgdaComment{-- | Λ α . M}\<%
\end{code}
%</systemF>

%<*systemFmuty>
\begin{code}%
\>\AgdaFunction{FType} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{FType} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaFunction{tyF}\<%
\end{code}
%</systemFmuty>

%<*systemFmutrm>
\begin{code}%
\>\AgdaFunction{FTerm} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{FTerm} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaFunction{tF}\<%
\end{code}
%</systemFmutrm>


\begin{code}%
\>\AgdaFunction{vₜ} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FType}\<%
\\
\>\AgdaFunction{vₜ} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨\_⟩} \AgdaFunction{∘} \AgdaInductiveConstructor{inj₁}\<%
\\
%
\\
\>\AgdaFunction{\_⟶\_} \AgdaSymbol{:} \AgdaFunction{FType} \AgdaSymbol{→} \AgdaFunction{FType} \AgdaSymbol{→} \AgdaFunction{FType}\<%
\\
\>\AgdaBound{α} \AgdaFunction{⟶} \AgdaBound{β} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{β}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[33]%
\>[33]\<%
\\
%
\\
\>\AgdaFunction{∀ₜ} \<[4]%
\>[4]\AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FType} \AgdaSymbol{→} \AgdaFunction{FType}\<%
\\
\>\AgdaFunction{∀ₜ} \AgdaBound{x} \AgdaBound{α} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{α}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[33]%
\>[33]\<%
\\
%
\\
\>\AgdaFunction{v} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaFunction{v} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨\_⟩} \AgdaFunction{∘} \AgdaInductiveConstructor{inj₁}\<%
\\
%
\\
\>\AgdaFunction{\_·\_} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩} \<[32]%
\>[32]\<%
\\
%
\\
\>\AgdaFunction{ƛ} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FType} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaFunction{ƛ} \AgdaBound{n} \AgdaBound{α} \AgdaBound{M} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{n} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))} \AgdaInductiveConstructor{⟩}\<%
\\
%
\\
\>\AgdaFunction{\_·ₜ\_} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FType} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{α} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{α}\AgdaSymbol{))))} \AgdaInductiveConstructor{⟩}\<%
\\
%
\\
\>\AgdaFunction{Λ} \AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{M} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))))} \AgdaInductiveConstructor{⟩}\<%
\\
%
\\
\>\AgdaFunction{testswap1} \AgdaSymbol{:} \AgdaFunction{swap} \AgdaFunction{SortFTermVars} \AgdaNumber{1} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{)))} \AgdaDatatype{≡} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{2} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{testswap1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{testswap2} \AgdaSymbol{:} \AgdaFunction{swap} \AgdaFunction{SortFTypeVars} \AgdaNumber{1} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{)))} \AgdaDatatype{≡} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{2}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{testswap2} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaComment{-- Define function with fold}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaDatatype{ℕ} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{n}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaNumber{1}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{m} \AgdaInductiveConstructor{,} \AgdaBound{n}\AgdaSymbol{)))} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaBound{m} \AgdaPrimitive{+} \AgdaBound{n}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaSymbol{\_} \AgdaInductiveConstructor{,} \AgdaBound{m}\AgdaSymbol{))))} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaBound{m}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{n} \AgdaInductiveConstructor{,} \AgdaSymbol{\_)))))} \AgdaSymbol{=} \AgdaBound{n}\<%
\\
\>\AgdaFunction{varsaux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaBound{m}\AgdaSymbol{)))))} \AgdaSymbol{=} \AgdaBound{m}\<%
\\
%
\\
\>\AgdaFunction{vars} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{vars} \AgdaSymbol{=} \AgdaFunction{fold} \AgdaFunction{tF} \AgdaFunction{varsaux}\<%
\\
%
\\
\>\AgdaComment{-- Prove trivial property of vars function by primitive induction.}\<%
\\
\>\AgdaFunction{PVars} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{PVars} \AgdaBound{M} \AgdaSymbol{=} \AgdaFunction{vars} \AgdaBound{M} \AgdaFunction{>} \AgdaNumber{0}\<%
\\
%
\\
\>\AgdaFunction{ProvePVars} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{M} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{PVars} \AgdaBound{M}\<%
\\
\>\AgdaFunction{ProvePVars} \AgdaSymbol{=} \AgdaFunction{foldInd} \AgdaFunction{tF} \AgdaFunction{PVars} \AgdaFunction{proof}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{plus>0} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{m} \AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{m} \AgdaFunction{>} \AgdaNumber{0} \AgdaSymbol{→} \AgdaBound{n} \AgdaFunction{>} \AgdaNumber{0} \AgdaSymbol{→} \AgdaBound{m} \AgdaPrimitive{+} \AgdaBound{n} \AgdaFunction{>} \AgdaNumber{0}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{plus>0} \AgdaSymbol{\{}\AgdaBound{m}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{n}\AgdaSymbol{\}} \AgdaBound{m>0} \AgdaBound{n>0} \AgdaSymbol{=} \AgdaFunction{≤-steps} \AgdaBound{m} \AgdaBound{n>0}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaFunction{tF} \AgdaFunction{PVars} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{PVars} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{x}\AgdaSymbol{)} \<[50]%
\>[50]\AgdaBound{tt} \<[61]%
\>[61]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)))} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaBound{PM} \AgdaInductiveConstructor{,} \AgdaBound{PN}\AgdaSymbol{)} \<[61]%
\>[61]\AgdaSymbol{=} \AgdaFunction{plus>0} \AgdaBound{PM} \AgdaBound{PN}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{⟩}\AgdaSymbol{))))} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaBound{tt} \AgdaInductiveConstructor{,} \AgdaBound{PM}\AgdaSymbol{)} \<[61]%
\>[61]\AgdaSymbol{=} \AgdaBound{PM}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{,} \AgdaBound{α}\AgdaSymbol{)))))} \<[50]%
\>[50]\AgdaSymbol{(}\AgdaBound{PM} \AgdaInductiveConstructor{,} \AgdaBound{tt}\AgdaSymbol{)} \<[61]%
\>[61]\AgdaSymbol{=} \AgdaBound{PM}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{proof} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)))))} \<[50]%
\>[50]\AgdaBound{PM} \<[61]%
\>[61]\AgdaSymbol{=} \AgdaBound{PM}\<%
\\
%
\\
\>\AgdaFunction{examplefresh} \AgdaSymbol{:} \AgdaFunction{fresh} \AgdaFunction{SortFTermVars} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{examplefresh} \AgdaSymbol{=} \AgdaInductiveConstructor{freshR} \AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{freshx} \AgdaSymbol{(}\AgdaInductiveConstructor{freshEf} \AgdaSymbol{(}\AgdaInductiveConstructor{freshinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{freshV≢S} \AgdaFunction{1≢2}\AgdaSymbol{)))} \AgdaInductiveConstructor{freshb≡}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{1≢2} \AgdaSymbol{:} \AgdaNumber{1} \AgdaFunction{≢} \AgdaNumber{2}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{1≢2} \AgdaSymbol{=} \AgdaSymbol{λ} \AgdaSymbol{()}\<%
\\
%
\\
\>\AgdaFunction{examplefv} \AgdaSymbol{:} \AgdaFunction{fvS} \AgdaFunction{SortFTermVars} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{)))} \AgdaDatatype{≡} \AgdaNumber{2} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\<%
\\
\>\AgdaFunction{examplefv} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{examplefv2} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaFunction{fvS} \AgdaFunction{SortFTypeVars} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))))} \AgdaDatatype{≡} \AgdaInductiveConstructor{[]}\<%
\\
\>\AgdaFunction{examplefv2} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{examplefv3} \AgdaSymbol{:} \AgdaFunction{fvS} \AgdaFunction{SortFTypeVars} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaDatatype{≡} \AgdaNumber{1} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\<%
\\
\>\AgdaFunction{examplefv3} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\end{code}

-- substaux :  (x : V)(t : μ tF)
--             → (e : ⟦ tF ⟧ (μ tF)) 
--             → fihα tF (const (μ tF)) e (x ∷ fv SortFTermVars t) 
--             → μ tF
-- substaux x t' (inj₁ y)                              tt     with x ≟v y
-- ... | yes _                                                      = t'
-- ... | no _                                                       = v y 
-- substaux x t' (inj₂ (inj₁ (t₁ , t₂)))               (hi₁ , hi₂)  = proj₁ hi₁ · proj₁ hi₂
-- substaux x t' (inj₂ (inj₂ (inj₁ (ty , y , t))))     ih           = ƛ y ty (proj₁ (proj₂ (proj₂ ih)))
-- substaux x t' (inj₂ (inj₂ (inj₂ (inj₁ (t , ty)))))  ih           = (proj₁ (proj₁  ih)) ·ₜ  ty
-- substaux x t' (inj₂ (inj₂ (inj₂ (inj₂ (α , t)))))   ih           = Λ α (proj₁ (proj₂ ih))

-- _[_≔_] : FTerm → V → FTerm → FTerm
-- t [ x ≔ t' ] = αIteration (x ∷ fv SortFTermVars t') (substaux x t') t

-- substaux : (x : V)(t : μ tF) → ⟦ tF ⟧ (μ tF) → μ tF
-- substaux x t' (inj₁ y) with x ≟v y
-- ... | yes _                                         = t'
-- ... | no _                                          = v y 
-- substaux x t' (inj₂ (inj₁ (t₁ , t₂)))               = t₁ · t₂
-- substaux x t' (inj₂ (inj₂ (inj₁ (ty , y , t))))     = ƛ y ty t
-- substaux x t' (inj₂ (inj₂ (inj₂ (inj₁ (t , ty)))))  = t ·ₜ  ty
-- substaux x t' (inj₂ (inj₂ (inj₂ (inj₂ (α , t)))))   = Λ α t

-- _[_≔_]ₙ : FTerm → V → FTerm → FTerm
-- t [ x ≔ t' ]ₙ  = fold tF (substaux x t') t

-- _[_≔_] : FTerm → V → FTerm → FTerm
-- t [ x ≔ t' ]   = foldα tF (x ∷ fv SortFTermVars t') (substaux x t') t

\begin{code}%
\>\AgdaKeyword{infix} \AgdaNumber{11} \AgdaFunction{\_[\_≔\_]ₙ}\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{11} \AgdaFunction{\_[\_≔\_]}\<%
\end{code}

%<*substaux>
\begin{code}%
\>\AgdaFunction{cF} \AgdaSymbol{=} \<[6]%
\>[6]\AgdaInductiveConstructor{|v|} \AgdaFunction{SortFTermVars} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{tF}\<%
\\
%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{cF} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaFunction{tF}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaInductiveConstructor{,} \AgdaBound{t₂}\AgdaSymbol{)))} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaBound{t₁} \AgdaFunction{·} \AgdaBound{t₂}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{ty} \AgdaInductiveConstructor{,} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{))))} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{ty} \AgdaBound{t}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{ty}\AgdaSymbol{)))))} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaBound{t} \AgdaFunction{·ₜ} \<[67]%
\>[67]\AgdaBound{ty}\<%
\\
\>\AgdaFunction{substaux} \AgdaSymbol{\_} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{)))))} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{t}\<%
\\
\>\AgdaFunction{substaux} \AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \<[16]%
\>[16]\AgdaBound{N} \AgdaInductiveConstructor{⟩} \<[21]%
\>[21]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{y}\AgdaSymbol{)} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaBound{N}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[59]%
\>[59]\AgdaSymbol{=} \AgdaFunction{v} \AgdaBound{y} \<%
\end{code}
%</substaux>

%<*naivesubst>
\begin{code}%
\>\AgdaFunction{\_[\_≔\_]ₙ} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \<[14]%
\>[14]\AgdaSymbol{=} \AgdaFunction{foldCtx} \AgdaFunction{tF} \AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M}\<%
\end{code}
%</naivesubst>

%<*subst>
\begin{code}%
\>\AgdaFunction{\_[\_≔\_]} \AgdaSymbol{:} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm}\<%
\\
\>\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \<[14]%
\>[14]\AgdaSymbol{=} \AgdaFunction{foldCtx-alpha} \<[31]%
\>[31]\AgdaFunction{tF} \AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M} \<%
\end{code}
%</subst>

\begin{code}%
\>\AgdaComment{-- Examples }\<%
\\
\>\AgdaFunction{exampleSubstn1} \AgdaSymbol{:} \AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{2} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]ₙ} \AgdaDatatype{≡} \AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{exampleSubstn1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{exampleSubst1} \AgdaSymbol{:} \AgdaFunction{Λ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{1} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{2}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{2} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaFunction{Λ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{0}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{0} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{exampleSubst1} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{exampleSubst2} \AgdaSymbol{:} \AgdaFunction{Λ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{2} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{2} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{3}\AgdaSymbol{))} \AgdaFunction{[} \AgdaNumber{3} \AgdaFunction{≔} \AgdaFunction{v} \AgdaNumber{1} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaFunction{Λ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaNumber{0} \AgdaSymbol{(}\AgdaFunction{vₜ} \AgdaNumber{1}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{v} \AgdaNumber{0} \AgdaFunction{·} \AgdaFunction{v} \AgdaNumber{1}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{exampleSubst2} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaKeyword{infix} \AgdaNumber{9} \AgdaFunction{（\_∙\_）\_} \<[15]%
\>[15]\<%
\\
\>\AgdaFunction{（\_∙\_）\_} \AgdaSymbol{=} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaFunction{SortFTermVars}\<%
\end{code}

\begin{code}%
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List.Any} \AgdaSymbol{as} \AgdaModule{any}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{any.}\AgdaModule{Membership-≡}\<%
\\
%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{)\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}} \AgdaSymbol{→}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{⊆} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaFunction{++} \AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{x}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemma-⊆∷} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaInductiveConstructor{[]} \AgdaBound{L}\AgdaSymbol{\}} \<[72]%
\>[72]\AgdaSymbol{\{}\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaFunction{SortFTermVars}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma∈fvSfv} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\})}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaInductiveConstructor{,} \AgdaBound{t₂}\AgdaSymbol{))\}} \<[69]%
\>[69]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{ty} \AgdaInductiveConstructor{,} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{)))\}} \<[69]%
\>[69]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{ty}\AgdaSymbol{))))\}} \<[69]%
\>[69]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[31]%
\>[31]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{))))\}} \<[69]%
\>[69]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{)\}\{}\AgdaBound{ys} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{Sort}\AgdaSymbol{\}} \AgdaSymbol{→}\<%
\\
\>\AgdaComment{--  fvSF≢ \{tF\} \{|R|\} ys (substaux (⟨ y , L ⟩) e) ⊆ fvSF≢ \{cF\} \{|R|\} ys ⟨ y , L ⟩ ++ fvSF≢ \{tF\} \{tF\} ys e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \AgdaBound{ys} \AgdaSymbol{(}\AgdaFunction{substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{⊆} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \<[68]%
\>[68]\AgdaFunction{++} \AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaBound{ys} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{x}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemma-⊆∷} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaBound{ys} \AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaInductiveConstructor{[]} \AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF≢} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaFunction{SortFTermVars}\AgdaSymbol{\}} \AgdaBound{ys} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{fvSF≢⊆} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{[]}\AgdaSymbol{\}} \AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{\_}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaSymbol{λ} \AgdaSymbol{()))} \<[159]%
\>[159]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t₁} \AgdaInductiveConstructor{,} \AgdaBound{t₂}\AgdaSymbol{))\}} \<[67]%
\>[67]\AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{ty} \AgdaInductiveConstructor{,} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{)))\}} \<[67]%
\>[67]\AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{ty}\AgdaSymbol{))))\}} \AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>\AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{))))\}} \<[67]%
\>[67]\AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{c∈ys→c∈xs++ys} \AgdaSymbol{\{}\AgdaArgument{xs} \AgdaSymbol{=} \AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\end{code}

%<*substauxBinds>
\begin{code}%
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{cF}\AgdaSymbol{\}\{}\AgdaBound{xs} \AgdaSymbol{:} \AgdaDatatype{List} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaBound{c}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBindF} \AgdaFunction{tF} \AgdaBound{xs} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaSymbol{(}\AgdaFunction{substaux} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{xs∉xN} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{y}\AgdaSymbol{\}} \<[81]%
\>[81]\AgdaBound{xs∉e} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \<[77]%
\>[77]\AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{xs∉xN}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaBound{xs∉e}\<%
\\
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{xs∉xN} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{P}\AgdaSymbol{))\}} \<[81]%
\>[81]\AgdaBound{xs∉e} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaBound{xs∉e}\<%
\\
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{xs∉xN} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{ty} \AgdaInductiveConstructor{,} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))\}} \<[81]%
\>[81]\AgdaBound{xs∉e} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaBound{xs∉e}\<%
\\
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{xs∉xN} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{ty}\AgdaSymbol{))))\}} \<[81]%
\>[81]\AgdaBound{xs∉e} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaBound{xs∉e}\<%
\\
\>\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{xs}\AgdaSymbol{\}} \AgdaBound{xs∉xN} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))))\}} \<[81]%
\>[81]\AgdaBound{xs∉e} \AgdaSymbol{=} \AgdaFunction{lemma-bindsR} \AgdaBound{xs∉e}\<%
\end{code}
%</substauxBinds>


%<*substauxSwap>
\begin{code}%
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{cF}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaFunction{substaux} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaFunction{tF} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaDatatype{≡}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{(}\AgdaFunction{substaux} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}
%</substauxSwap>

\begin{code}%
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaFunction{SortFTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[20]%
\>[20]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[29]%
\>[29]\AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[28]%
\>[28]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[37]%
\>[37]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[37]%
\>[37]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[43]%
\>[43]\AgdaBound{z≢z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{z≢z} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢y} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{x≡w}\AgdaSymbol{)} \AgdaBound{x≡y}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[55]%
\>[55]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡w} \AgdaBound{w≡y}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[52]%
\>[52]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{y} \<[74]%
\>[74]\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{y≢y} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{w≢z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢z} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{x≡w}\AgdaSymbol{)} \AgdaBound{x≡z}\AgdaSymbol{))}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[23]%
\>[23]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \<[33]%
\>[33]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[39]%
\>[39]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[55]%
\>[55]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡w} \AgdaBound{w≡y}\AgdaSymbol{))} \<[87]%
\>[87]\<%
\\
\>\AgdaSymbol{...} \<[43]%
\>[43]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[49]%
\>[49]\AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[53]%
\>[53]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡w} \AgdaBound{w≡z}\AgdaSymbol{))} \<[97]%
\>[97]\<%
\\
\>\AgdaSymbol{...} \<[53]%
\>[53]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl} \<[80]%
\>[80]\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢w} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaBound{x≡w}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaKeyword{with} \AgdaFunction{SortFTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[28]%
\>[28]\AgdaBound{SortFTermVars≢S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{SortFTermVars≢S} \AgdaBound{SortFTermVars≡S}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[30]%
\>[30]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[40]%
\>[40]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡y} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡y}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[40]%
\>[40]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[46]%
\>[46]\AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{y} \<[73]%
\>[73]\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{z≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡y} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{z≡y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡z}\AgdaSymbol{))))}\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{z≢y} \<[71]%
\>[71]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \<[35]%
\>[35]\<%
\\
\>[3]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \<[61]%
\>[61]\AgdaKeyword{with} \AgdaBound{z} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{z≡w} \AgdaSymbol{=} \<[75]%
\>[75]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{z≡w}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \<[62]%
\>[62]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \<[72]%
\>[72]\AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[51]%
\>[51]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡z}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡y}\AgdaSymbol{))))}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢z} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{w≡z}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[80]%
\>[80]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡w} \AgdaSymbol{=} \<[93]%
\>[93]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{w≢y} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡w}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \<[80]%
\>[80]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{y≢w} \AgdaSymbol{=} \<[92]%
\>[92]\AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{y} \<[74]%
\>[74]\<%
\\
\>\AgdaSymbol{...} \<[61]%
\>[61]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡y} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaSymbol{=} \<[84]%
\>[84]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \AgdaKeyword{with} \AgdaBound{w} \AgdaFunction{≟v} \AgdaBound{z} \<[83]%
\>[83]\<%
\\
\>\AgdaSymbol{...} \<[71]%
\>[71]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{w≡z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{=} \<[94]%
\>[94]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢y} \AgdaBound{x≡y}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[31]%
\>[31]\AgdaBound{x≢w} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{x≢y} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[58]%
\>[58]\AgdaBound{x≢z} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢y} \<[72]%
\>[72]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaBound{w≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \AgdaSymbol{=} \<[94]%
\>[94]\AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢w} \AgdaBound{x≡w}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[81]%
\>[81]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{w}\AgdaSymbol{\}} \<[84]%
\>[84]\<%
\\
\>[3]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{SortFTermVars≢S} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{w}\<%
\\
\>\AgdaSymbol{...} \<[14]%
\>[14]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡w} \<[25]%
\>[25]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaSymbol{...} \<[14]%
\>[14]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[20]%
\>[20]\AgdaSymbol{\_} \<[25]%
\>[25]\AgdaKeyword{with} \AgdaFunction{SortFTermVars} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[26]%
\>[26]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{SortFTermVars≡S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{SortFTermVars≢S} \AgdaBound{SortFTermVars≡S}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[26]%
\>[26]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M'}\AgdaSymbol{))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{w} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{))))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))))\}} \<[80]%
\>[80]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{lemma-[]Swap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaFunction{SortFTermVars} \AgdaBound{y} \AgdaBound{z} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaFunction{（} \AgdaBound{y} \AgdaFunction{∙} \AgdaBound{z} \AgdaFunction{）ₐ} \AgdaBound{x} \AgdaFunction{≔} \AgdaFunction{swap} \AgdaFunction{SortFTermVars} \AgdaBound{y} \AgdaBound{z} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaDatatype{≡}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{swap} \AgdaFunction{SortFTermVars} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-[]Swap} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemmaSwapFoldCtxEquiv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{SortFTermVars}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\<%
\end{code}

%<*substlemma1>
\begin{code}%
\>\AgdaFunction{lemma-subst-alpha} \AgdaSymbol{:} \<[21]%
\>[21]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M′} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{∼α} \AgdaBound{M′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaDatatype{≡} \AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\<%
\\
\>\AgdaFunction{lemma-subst-alpha} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M′}\AgdaSymbol{\}} \AgdaBound{M∼M′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtxα-StrongαCompatible} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaBound{M′} \AgdaBound{M∼M′}\<%
\end{code}
%</substlemma1>

\begin{code}%
\>\<%
\end{code}

%<*lemmasubstaux>
\begin{code}%
\>\AgdaFunction{lemma-substaux} \<[16]%
\>[16]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{e} \AgdaBound{e′} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{)\}\{}\AgdaBound{c} \AgdaBound{c′} \AgdaSymbol{:} \<[49]%
\>[49]\AgdaDatatype{μ} \AgdaFunction{cF}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaBound{c} \AgdaFunction{∼α} \AgdaBound{c′}\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaDatatype{∼αF} \AgdaFunction{tF} \AgdaBound{e} \AgdaBound{e′}\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{→} \AgdaFunction{substaux} \AgdaBound{c} \AgdaBound{e} \AgdaFunction{∼α} \AgdaFunction{substaux} \AgdaBound{c′} \AgdaBound{e′}\<%
\end{code}
%</lemmasubstaux>

\begin{code}%
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaSymbol{.}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{N′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaInductiveConstructor{∼αV}\AgdaSymbol{)} \<[89]%
\>[89]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y} \<[14]%
\>[14]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaInductiveConstructor{∼αV}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \<[83]%
\>[83]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{))))} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{))))}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))))} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{e∼e′} \AgdaBound{e∼e′₁}\AgdaSymbol{)))))}\<%
\\
\>\AgdaFunction{lemma-substaux} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \<[42]%
\>[42]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{x₁}\AgdaSymbol{)))))} \<[63]%
\>[63]\AgdaSymbol{=} \<[66]%
\>[66]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \<[95]%
\>[95]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaBound{xs} \AgdaBound{x₁}\AgdaSymbol{)))))}\<%
\\
%
\\
\>\AgdaFunction{lemma-substn-alpha} \AgdaSymbol{:} \<[22]%
\>[22]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{N′} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{18}{}\<[18]%
\>[18]\AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{N′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-substn-alpha} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtx-alpha-Ctx} \AgdaFunction{lemma-substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaBound{M}\<%
\end{code}

%<*substlemma2>
\begin{code}%
\>\AgdaFunction{lemma-substα′} \AgdaSymbol{:} \<[17]%
\>[17]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{N′} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{17}{}\<[17]%
\>[17]\AgdaSymbol{→} \AgdaBound{N} \AgdaFunction{∼α} \AgdaBound{N′} \AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \AgdaFunction{]}\<%
\\
\>\AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaBound{N∼N′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtxalpha-cxtalpha} \AgdaFunction{lemma-substaux} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaInductiveConstructor{∼αV} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αEf} \AgdaBound{N∼N′}\AgdaSymbol{)))} \AgdaBound{M}\<%
\end{code}
%</substlemma2>

\begin{code}%
\>\AgdaFunction{fv2ctx} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{)} \AgdaBound{M} \<[63]%
\>[63]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>\AgdaFunction{fv2ctx} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{nb} \AgdaSymbol{=} \AgdaBound{nb}\<%
\end{code}

%<*lemmasubsts>
\begin{code}%
\>\AgdaFunction{lemmaSubsts} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaSymbol{\{}\AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[2]\AgdaIndent{15}{}\<[15]%
\>[15]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{z} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaBound{nb}\<%
\\
\> \AgdaSymbol{=} \AgdaFunction{lemma-foldCtxAlpha-foldCtx}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaFunction{tF} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{lemma-substaux}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxSwap} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(}\AgdaFunction{fv2ctx} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaBound{nb}\AgdaSymbol{)}\<%
\end{code}
%</lemmasubsts>

\begin{code}%
\>\AgdaComment{-- \{- Previous lemma could also be proved by simple induction on terms -\}}\<%
\\
\>\AgdaComment{-- substα′2 : (x : V)(t t′ t″ : FTerm) → t′ ∼α t″ → t [ x ≔ t′ ] ∼α t [ x ≔ t″ ]}\<%
\\
\>\AgdaComment{-- substα′2 x t t′ t″ t′∼t″ }\<%
\\
\>\AgdaComment{--   with x ∷ fv SortFTermVars t′ | x ∷ fv SortFTermVars t″ | cong (\_∷\_ x) (lemma∼fv' SortFTermVars t′∼t″)}\<%
\\
\>\AgdaComment{-- ... | fvt′ | .fvt′ | refl }\<%
\\
\>\AgdaComment{--   with proj₁ (bindersFreeαElem fvt′ t)}\<%
\\
\>\AgdaComment{-- ... | e }\<%
\\
\>\AgdaComment{--   = foldInd tF (λ t → t′ ∼α t″ → fold tF (substaux x t′) t ∼α fold tF (substaux x t″) t) substα′aux e t′∼t″}\<%
\\
\>\AgdaComment{--   where}\<%
\\
\>\AgdaComment{--   substα′aux  : (e : ⟦ tF ⟧ (μ tF))}\<%
\\
\>\AgdaComment{--               → fih tF (λ t₁ → t′ ∼α t″ → fold tF (substaux x t′) t₁ ∼α fold tF (substaux x t″) t₁) e}\<%
\\
\>\AgdaComment{--               → t′ ∼α t″ → fold tF (substaux x t′) ⟨ e ⟩ ∼α fold tF (substaux x t″) ⟨ e ⟩}\<%
\\
\>\AgdaComment{--   substα′aux (inj₁ y)                                  \_            t′∼t″}\<%
\\
\>\AgdaComment{--       with x ≟v y }\<%
\\
\>\AgdaComment{--   ... | yes \_ = t′∼t″}\<%
\\
\>\AgdaComment{--   ... | no  \_ = ∼αR (∼α+₁ ∼αV)}\<%
\\
\>\AgdaComment{--   substα′aux (inj₂ (inj₁ (⟨ t₁ ⟩ , ⟨ t₂ ⟩)))           (hi₁ , hi₂)  t′∼t″}\<%
\\
\>\AgdaComment{--     = ∼αR (∼α+₂ (∼α+₁ (∼αx (hi₁ t′∼t″) (hi₂ t′∼t″))))}\<%
\\
\>\AgdaComment{--   substα′aux (inj₂ (inj₂ (inj₁ (ty , x , ⟨ t ⟩))))     (\_ , hi)     t′∼t″}\<%
\\
\>\AgdaComment{--     = ∼αR (∼α+₂ (∼α+₂ (∼α+₁ (∼αx ρF (∼αB [] ( λ c c∉[] → lemma∼swapEquiv2 (hi  t′∼t″) x c)))))) --}\<%
\\
\>\AgdaComment{--   substα′aux (inj₂ (inj₂ (inj₂ (inj₁ (⟨ t ⟩ , ty)))))  (hi , \_)     t′∼t″}\<%
\\
\>\AgdaComment{--     = ∼αR (∼α+₂ (∼α+₂ (∼α+₂ (∼α+₁ (∼αx (hi t′∼t″) ρF))))) --}\<%
\\
\>\AgdaComment{--   substα′aux (inj₂ (inj₂ (inj₂ (inj₂ (α , ⟨ t ⟩)))))   hi           t′∼t″}\<%
\\
\>\AgdaComment{--     = ∼αR (∼α+₂ (∼α+₂ (∼α+₂ (∼α+₂ (∼αB [] (λ c c∉[] → lemma∼swapEquiv2 (hi  t′∼t″) α c)))))) --}\<%
\\
%
\\
\>\AgdaComment{-- -- substauxty : (x : V)(ty : FType)}\<%
\\
\>\AgdaComment{-- --       (e : ⟦ tF ⟧ (μ tF))}\<%
\\
\>\AgdaComment{-- --       → fihα tF (const (μ tF)) e (x ∷ fv SortFTypeVars ty)}\<%
\\
\>\AgdaComment{-- --       → μ tF}\<%
\\
\>\AgdaComment{-- -- substauxty x ty e fihα = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- -- \_[\_≔\_]ₜ : FTerm → V → FType → FTerm}\<%
\\
\>\AgdaComment{-- -- t [ x ≔ ty ]ₜ = αIteration (x ∷ fv SortFTypeVars ty) (substauxty x ty) t}\<%
\\
%
\\
\>\AgdaFunction{lemma-substnfv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaFunction{fvS} \AgdaFunction{SortFTermVars} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{M} \AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{≡} \AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₁} \AgdaBound{y} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[54]%
\>[54]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fvy} \AgdaSymbol{\_} \<[70]%
\>[70]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{y}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡y} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{((}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{x∉fvy}\AgdaSymbol{)} \AgdaBound{x≡y}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{x≢y} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{M′}\AgdaSymbol{))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[54]%
\>[54]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv} \<[67]%
\>[67]\<%
\\
\>[2]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaBound{xnbM} \AgdaBound{xnbM′}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaBound{M} \AgdaFunction{·} \AgdaBound{M′}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaFunction{cong₂} \AgdaFunction{\_·\_} \<[19]%
\>[19]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{x∉fv}\AgdaSymbol{)} \AgdaBound{xnbM}\AgdaSymbol{)}\<%
\\
\>[5]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M′}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvS} \AgdaFunction{SortFTermVars} \<[80]%
\>[80]\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{x∉fv}\AgdaSymbol{)} \AgdaBound{xnbM′}\AgdaSymbol{)} \<[98]%
\>[98]\AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·} \AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·} \AgdaBound{M′}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{□}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[54]%
\>[54]\AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv} \<[67]%
\>[67]\<%
\\
\>[5]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \<[59]%
\>[59]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaSymbol{\_} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBB≢} \AgdaBound{x≢y} \AgdaBound{xnbM}\AgdaSymbol{))))))} \<[116]%
\>[116]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{t} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{t}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \<[38]%
\>[38]\AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}}\<%
\\
\>[5]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaSymbol{(}\AgdaFunction{lemma-∉} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaFunction{sym≢} \AgdaBound{x≢y}\AgdaSymbol{)}\<%
\\
\>[38]\AgdaIndent{48}{}\<[48]%
\>[48]\AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉ys} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fvSF} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaFunction{tyF}\AgdaSymbol{\}} \AgdaFunction{SortFTermVars} \AgdaBound{t}\AgdaSymbol{\}} \AgdaBound{x∉fv}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{38}{}\<[38]%
\>[38]\AgdaBound{xnbM}\AgdaSymbol{)} \<[45]%
\>[45]\AgdaFunction{⟩} \<[48]%
\>[48]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{t} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩} \<[20]%
\>[20]\<%
\\
\>[5]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{y} \AgdaBound{t} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{□}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{))))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv}\<%
\\
\>[5]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \<[59]%
\>[59]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₁} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaBound{xnbM} \AgdaSymbol{\_))))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{t}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≡⟨} \<[10]%
\>[10]\AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{P} \AgdaSymbol{→} \<[23]%
\>[23]\AgdaBound{P} \AgdaFunction{·ₜ} \AgdaBound{t}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{c∉xs++ys→c∉xs} \AgdaBound{x∉fv}\AgdaSymbol{)} \AgdaBound{xnbM}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·ₜ} \AgdaBound{t}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{t}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{□}\<%
\\
\>\AgdaFunction{lemma-substnfv} \<[16]%
\>[16]\AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{α} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))))} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{x∉fv}\<%
\\
\>[6]\AgdaIndent{16}{}\<[16]%
\>[16]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \<[59]%
\>[59]\AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBinj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBB≢} \AgdaBound{x≢α} \AgdaBound{xnbM}\AgdaSymbol{))))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin≡}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaFunction{Λ} \AgdaBound{α}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaBound{x∉fv} \AgdaBound{xnbM}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{Λ} \AgdaBound{α} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{□}\<%
\end{code}

%<*substnaivecompositionpredicate>
\begin{code}%
\>\AgdaFunction{PSCn} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaFunction{FTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{PSCn} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{N} \AgdaBound{M} \AgdaSymbol{=} \<[24]%
\>[24]\AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L} \AgdaSymbol{→} \<[40]%
\>[40]\AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{∼α} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\<%
\end{code}
%</substnaivecompositionpredicate>

\begin{code}%
\>\AgdaFunction{lemma-substCompositionV} \<[25]%
\>[25]\AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaBound{z} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{N} \AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \<[39]%
\>[39]\AgdaBound{L}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[2]\AgdaIndent{25}{}\<[25]%
\>[25]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{v} \AgdaBound{z}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{∼α} \AgdaSymbol{(}\AgdaFunction{v} \AgdaBound{z}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ} \<[97]%
\>[97]\<%
\\
\>\AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉yfvL} \AgdaSymbol{\_} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z} \<[26]%
\>[26]\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{((}\AgdaFunction{b∉a∷xs→b≢a} \AgdaBound{x∉yfvL}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaBound{x≡z} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{y≡z}\AgdaSymbol{)))}\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[18]%
\>[18]\AgdaBound{y≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{ρ}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{no} \<[29]%
\>[29]\AgdaBound{x≢z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{x≢z} \AgdaKeyword{with} \AgdaBound{y} \AgdaFunction{≟v} \AgdaBound{z} \<[26]%
\>[26]\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{y≡z}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{subst} \<[11]%
\>[11]\AgdaSymbol{(λ} \AgdaBound{M} \AgdaSymbol{→} \<[19]%
\>[19]\AgdaBound{L} \AgdaFunction{∼α} \AgdaBound{M}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaFunction{lemma-substnfv} \AgdaSymbol{(}\AgdaFunction{lemma∉fvfvS} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{SortFTermVars}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{b∉a∷xs→b∉xs} \AgdaBound{x∉yfvL}\AgdaSymbol{))} \AgdaBound{xnbL}\AgdaSymbol{)} \AgdaFunction{ρ} \<[95]%
\>[95]\<%
\\
\>\AgdaSymbol{...} \<[12]%
\>[12]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[18]%
\>[18]\AgdaBound{y≢z} \AgdaKeyword{with} \AgdaBound{x} \AgdaFunction{≟v} \AgdaBound{z}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{yes} \AgdaBound{x≡z} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{x≢z} \AgdaBound{x≡z}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \<[22]%
\>[22]\AgdaSymbol{|} \<[25]%
\>[25]\AgdaInductiveConstructor{no} \<[29]%
\>[29]\AgdaSymbol{\_} \<[34]%
\>[34]\AgdaSymbol{=} \AgdaFunction{ρ}\<%
\\
%
\\
\>\AgdaComment{-- Esto puede demostrarse genericamente usando fold fusion !}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{∼-Reasoning}\AgdaSymbol{(}\AgdaFunction{tF}\AgdaSymbol{)}\<%
\\
\>\<%
\end{code}

%<*substcompositionNdef>
\begin{code}%
\>\AgdaFunction{lemma-substCompositionN} \AgdaSymbol{:} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{M} \AgdaBound{N} \AgdaBound{L} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{PSCn} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{N} \AgdaBound{M}\<%
\\
\>\AgdaFunction{lemma-substCompositionN} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{foldInd} \AgdaFunction{tF} \AgdaSymbol{(}\AgdaFunction{PSCn} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{N}\AgdaSymbol{)} \AgdaFunction{lemma-substCompositionNAux} \AgdaBound{M}\<%
\end{code}
%</substcompositionNdef>

\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaFunction{tF} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaFunction{tF} \AgdaSymbol{(}\AgdaFunction{PSCn} \AgdaBound{N}\AgdaSymbol{)} \AgdaBound{e} \AgdaSymbol{→} \AgdaFunction{PSCn} \AgdaBound{N} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[87]%
\>[87]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{z}\AgdaSymbol{)} \AgdaSymbol{\_} \AgdaBound{x∉yfvL} \AgdaBound{xnbL} \AgdaSymbol{=} \AgdaFunction{lemma-substCompositionV} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{z}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M′} \<[46]%
\>[46]\AgdaInductiveConstructor{,} \AgdaBound{M″} \AgdaSymbol{)))} \AgdaSymbol{(}\AgdaBound{hiM′} \AgdaInductiveConstructor{,} \AgdaBound{hiM″}\AgdaSymbol{)} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[8]%
\>[8]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{·} \<[17]%
\>[17]\AgdaBound{M″} \AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{((}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaBound{M″} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{))} \<[48]%
\>[48]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaBound{M″} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{∼⟨} \<[12]%
\>[12]\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaSymbol{(}\AgdaBound{hiM′} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{hiM″} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\AgdaSymbol{))))} \AgdaFunction{⟩}\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ} \AgdaSymbol{)} \AgdaFunction{·} \<[52]%
\>[52]\AgdaSymbol{(}\AgdaBound{M″} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[8]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{·} \<[17]%
\>[17]\AgdaBound{M″}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ} \<[54]%
\>[54]\<%
\\
\>[0]\AgdaIndent{8}{}\<[8]%
\>[8]\AgdaFunction{∎}\<%
\end{code}

%<*substncompositionabstractioncase>
\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{))))} \<[64]%
\>[64]\AgdaSymbol{(\_} \AgdaInductiveConstructor{,} \AgdaBound{hiM}\AgdaSymbol{)} \AgdaBound{xnotInyfvL} \AgdaBound{xnotBL} \AgdaSymbol{=} \<[95]%
\>[95]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{t} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \<[52]%
\>[52]\AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{t} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{∼⟨} \AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \<[18]%
\>[18]\AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁}\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \<[15]%
\>[15]\AgdaFunction{ρF} \AgdaSymbol{(}\AgdaFunction{lemma∼+B} \AgdaSymbol{(}\AgdaBound{hiM} \AgdaBound{xnotInyfvL} \AgdaBound{xnotBL}\AgdaSymbol{))))))} \<[58]%
\>[58]\AgdaFunction{⟩} \<[60]%
\>[60]\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{t} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \<[52]%
\>[52]\AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{(}\AgdaFunction{ƛ} \AgdaBound{z} \AgdaBound{t} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{∎}\<%
\end{code}
%</substncompositionabstractioncase>

\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{t}\AgdaSymbol{)))))} \AgdaSymbol{(}\AgdaBound{hi} \AgdaInductiveConstructor{,} \AgdaSymbol{\_)} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{t}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·ₜ} \AgdaBound{t} \<[40]%
\>[40]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₁} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaSymbol{(}\AgdaBound{hi} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\AgdaSymbol{)} \AgdaFunction{ρF}\AgdaSymbol{)))))} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\AgdaSymbol{)} \AgdaFunction{·ₜ} \AgdaBound{t} \<[51]%
\>[51]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{t}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{lemma-substCompositionNAux} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaBound{t} \AgdaInductiveConstructor{,} \AgdaBound{M}\AgdaSymbol{)))))} \AgdaBound{hi} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \<[7]%
\>[7]\AgdaFunction{begin}\<%
\\
\>[4]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Λ} \AgdaBound{t} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{Λ} \AgdaBound{t} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∼⟨} \AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼α+₂} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αB} \AgdaInductiveConstructor{[]} \AgdaSymbol{(λ} \AgdaBound{c} \AgdaBound{c∉[]} \AgdaSymbol{→} \AgdaFunction{lemma∼swapEquiv} \AgdaSymbol{(}\AgdaBound{hi} \AgdaBound{x∉yfvL} \AgdaBound{xnbL}\AgdaSymbol{)} \AgdaBound{t} \AgdaBound{c}\AgdaSymbol{))))))} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaFunction{Λ} \AgdaBound{t} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{≈⟨} \AgdaInductiveConstructor{refl} \AgdaFunction{⟩}\<%
\\
\>[7]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{Λ} \AgdaBound{t} \AgdaBound{M}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\end{code}




Composition Lemma (exemplifies alpha induction principle usage)



--lemma-substComposition' :  {x y : V}{M N L : FTerm} → PSC {x} {y} {L} N M 
--lemma-substComposition' {x} {y} {M} {N} {L} p∉ = {!!}
\end{code}

%<*substcompositionpredicate>
\begin{code}%
\>\AgdaFunction{TreeFTermF} \AgdaSymbol{=} \<[14]%
\>[14]\AgdaInductiveConstructor{|Ef|} \AgdaFunction{tF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{tF} \AgdaInductiveConstructor{|x|} \AgdaInductiveConstructor{|Ef|} \AgdaFunction{tF} \<[46]%
\>[46]\<%
\\
\>\AgdaFunction{TreeFTerm} \AgdaSymbol{=} \AgdaDatatype{μ} \AgdaFunction{TreeFTermF}\<%
\\
%
\\
\>\AgdaFunction{PSComp} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{TreeFTerm} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{PSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaSymbol{=} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\AgdaSymbol{)} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \AgdaFunction{∼α} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{)}\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \AgdaFunction{]}\<%
\end{code}
%</substcompositionpredicate>


%<*substcompositionpredicatealpha>
\begin{code}%
\>\AgdaFunction{αCompatiblePSComp} \AgdaSymbol{:} \AgdaSymbol{∀} \AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{αCompatiblePred} \AgdaSymbol{\{}\AgdaFunction{TreeFTermF}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{PSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{αCompatiblePSComp} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{M′} \AgdaInductiveConstructor{,} \AgdaBound{N′} \AgdaInductiveConstructor{,} \AgdaBound{L′} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[62]%
\>[62]\<%
\\
\>[4]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{(}\AgdaInductiveConstructor{∼αR} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{M∼M′} \AgdaSymbol{(}\AgdaInductiveConstructor{∼αx} \AgdaBound{N∼N′} \AgdaBound{L∼L′}\AgdaSymbol{)))} \AgdaBound{PMs} \AgdaBound{x∉y:fvL′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \<[5]%
\>[5]\AgdaFunction{begin}\<%
\\
\>[2]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M′} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[36]%
\>[36]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Strong α compability of inner substitution operation       }\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong} \AgdaSymbol{(λ} \AgdaBound{z} \AgdaSymbol{→} \AgdaBound{z} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \AgdaFunction{]}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-subst-alpha} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaFunction{M∼M'}\AgdaSymbol{))} \<[90]%
\>[90]\AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[36]%
\>[36]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Strong α compability of outter substitution operation       }\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{lemma-subst-alpha} \<[27]%
\>[27]\AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaFunction{N∼N'}\AgdaSymbol{))} \<[90]%
\>[90]\AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[36]%
\>[36]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Outter substitution is alpha-compatible in its substituted argument}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[39]%
\>[39]\AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaFunction{L∼L'}\AgdaSymbol{)} \<[90]%
\>[90]\AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[36]%
\>[36]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Application of the inductive hypothesis}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaBound{PMs} \AgdaFunction{x∉y∶fvL} \<[90]%
\>[90]\AgdaFunction{⟩} \<[92]%
\>[92]\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[36]%
\>[36]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[46]%
\>[46]\AgdaFunction{]} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Strong α compability of inner substitution operation       }\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong} \<[14]%
\>[14]\AgdaSymbol{(λ} \AgdaBound{P} \AgdaSymbol{→} \AgdaBound{P} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \AgdaFunction{]}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-subst-alpha} \AgdaFunction{M∼M'}\AgdaSymbol{)} \<[90]%
\>[90]\AgdaFunction{⟩} \<[92]%
\>[92]\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M′} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[36]%
\>[36]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[46]%
\>[46]\AgdaFunction{]} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Inner substitution is alpha-compatible in its substituted argument}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{lemma-subst-alpha} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\<%
\\
\>[5]\AgdaIndent{23}{}\<[23]%
\>[23]\AgdaSymbol{(}\AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M′}\AgdaSymbol{\}} \AgdaFunction{L∼L'}\AgdaSymbol{)} \<[90]%
\>[90]\AgdaFunction{⟩} \<[99]%
\>[99]\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M′} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[36]%
\>[36]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[46]%
\>[46]\AgdaFunction{]} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Strong α compability of substitution operation in subsituted term       }\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{≈⟨} \AgdaFunction{cong} \<[14]%
\>[14]\AgdaSymbol{(λ} \AgdaBound{P} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{M′} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \AgdaFunction{]}\AgdaSymbol{)} \<[38]%
\>[38]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{P} \AgdaFunction{]}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-subst-alpha} \AgdaFunction{N∼N'}\AgdaSymbol{)} \<[90]%
\>[90]\AgdaFunction{⟩}\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M′} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \<[36]%
\>[36]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[46]%
\>[46]\AgdaFunction{]} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaComment{-- Outter substitution is alpha-compatible in its substituted argument}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∼⟨} \AgdaFunction{lemma-substα′} \<[23]%
\>[23]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M′} \<[32]%
\>[32]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N′} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-substα′} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N′}\AgdaSymbol{\}} \AgdaFunction{L∼L'}\AgdaSymbol{)} \<[90]%
\>[90]\AgdaFunction{⟩} \<[92]%
\>[92]\<%
\\
\>[5]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{(}\AgdaBound{M′} \<[12]%
\>[12]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N′} \<[36]%
\>[36]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L′} \<[46]%
\>[46]\AgdaFunction{]} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaFunction{∎} \<[11]%
\>[11]\<%
\end{code}
%</substcompositionpredicatealpha>

\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x∉y∶fvL} \AgdaSymbol{:} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x∉y∶fvL} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{xs} \AgdaSymbol{→} \AgdaBound{x} \AgdaFunction{∉} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∼fv} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemma-∼αEf} \AgdaBound{L∼L′}\AgdaSymbol{)))} \AgdaBound{x∉y:fvL′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{M∼M'} \AgdaSymbol{=} \AgdaFunction{lemma-∼αEf} \AgdaBound{M∼M′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{N∼N'} \AgdaSymbol{=} \AgdaFunction{lemma-∼αEf} \AgdaBound{N∼N′}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{L∼L'} \AgdaSymbol{=} \AgdaFunction{lemma-∼αEf} \AgdaBound{L∼L′}\<%
\end{code}


%<*substitutioncompositionproof>
\begin{code}%
\>\AgdaFunction{alpha-proof} \AgdaSymbol{:} \<[15]%
\>[15]\AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}(}\AgdaBound{Ms} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{TreeFTermF}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaBound{Ms} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{Ms}\AgdaSymbol{)} \AgdaBound{Ms} \AgdaSymbol{→} \AgdaFunction{PSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{Ms}\<%
\\
\>\AgdaFunction{alpha-proof} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaBound{nOcc} \AgdaBound{nOcc2} \AgdaBound{xnIny∶fvL}\<%
\\
\>[2]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{=} \<[6]%
\>[6]\AgdaFunction{begin}\<%
\\
\>[3]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≈⟨} \AgdaFunction{lemma-subst-alpha} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaFunction{x:fvN-NB-M}\AgdaSymbol{)} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∼⟨} \AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaFunction{y:fvL-NB-M[x≔N]ₙ} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∼⟨} \AgdaFunction{lemma-substCompositionN} \<[34]%
\>[34]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaBound{xnIny∶fvL} \AgdaFunction{x-NB-L} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \<[46]%
\>[46]\AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∼⟨} \AgdaFunction{lemma-substn-alpha} \<[29]%
\>[29]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaFunction{y:fvL-NB-N}\AgdaSymbol{))} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \<[46]%
\>[46]\AgdaFunction{]ₙ}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{∼⟨} \AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemmaSubsts} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{\}} \AgdaFunction{x:fvN[y≔L]-NB-M[y≔L]ₙ}\AgdaSymbol{)} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \<[46]%
\>[46]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{≈⟨} \AgdaFunction{lemma-subst-alpha} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemmaSubsts} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaFunction{y:fvL-NB-M}\AgdaSymbol{))} \<[86]%
\>[86]\AgdaFunction{⟩}\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaBound{M} \<[13]%
\>[13]\AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \<[22]%
\>[22]\AgdaFunction{]}\AgdaSymbol{)} \<[26]%
\>[26]\AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]} \<[46]%
\>[46]\AgdaFunction{]}\<%
\\
\>[0]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaFunction{∎}\<%
\end{code}
%</substitutioncompositionproof>

\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bM,N,L} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{\{}\AgdaFunction{TreeFTermF}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{M} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{N} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bM,N,L} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{xs} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaBound{xs} \AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmafvtern} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\})} \AgdaBound{nOcc2}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bM} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{M} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{N} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bM}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaFunction{fvM++fvN++fvL∉bM,N,L}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bN} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{M} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{N} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bN}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaFunction{fvM++fvN++fvL∉bM,N,L}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bL} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{M} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{N} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvM++fvN++fvL∉bL}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaFunction{fvM++fvN++fvL∉bM,N,L}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bM} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bM} \AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nOcc}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bN} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bN} \AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₁inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nOcc}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bL} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:y∉bL} \AgdaSymbol{=} \AgdaFunction{lemmalistNotOccurBindEf→ListNotOccurBindR} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{listNotOccurBx₂inv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindF} \AgdaBound{nOcc}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN-NB-M} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \<[41]%
\>[41]\AgdaBound{N}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN-NB-M} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaFunction{x:y∉bM}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-binds++l} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bM}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x-NB-L} \AgdaSymbol{:} \AgdaBound{x} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x-NB-L} \AgdaSymbol{=} \AgdaFunction{lemma-binds:head} \AgdaFunction{x:y∉bL}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-M} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-M} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaSymbol{(}\AgdaFunction{lemma-binds:tail} \AgdaFunction{x:y∉bM}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bM}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-N} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-N} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaSymbol{(}\AgdaFunction{lemma-binds:tail} \AgdaFunction{x:y∉bN}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bN}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-M[x≔N]ₙ} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y:fvL-NB-M[x≔N]ₙ}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemma-foldCtxBinds} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{(}\AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaInductiveConstructor{notOccurBv} \AgdaSymbol{(}\AgdaFunction{notOccurBindR→notOccurBindEf} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaFunction{y:fvL-NB-N}\AgdaSymbol{))))} \AgdaSymbol{(}\AgdaFunction{lemma-bindsR} \AgdaSymbol{(}\AgdaFunction{lemma-binds×} \AgdaFunction{lemma-bindsv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindEf} \AgdaSymbol{(}\AgdaFunction{lemma-binds:tail} \AgdaFunction{y:fvL-NB-N}\AgdaSymbol{))))))} \AgdaFunction{y:fvL-NB-M} \<[319]%
\>[319]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{[x]∉bM[y≔L]ₙ} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{[x]∉bM[y≔L]ₙ} \AgdaSymbol{=} \AgdaFunction{lemma-foldCtxBinds} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{(}\AgdaFunction{lemma-bindsR} \AgdaSymbol{(} \AgdaFunction{lemma-binds×} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBv} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \AgdaSymbol{(} \AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindEf} \AgdaSymbol{(} \AgdaFunction{lemma-binds:cons} \<[195]%
\>[195]\AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaFunction{x:y∉bL}\AgdaSymbol{)} \AgdaInductiveConstructor{[]}\AgdaSymbol{)))))} \AgdaSymbol{(}\AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaFunction{x:y∉bM} \AgdaSymbol{)} \AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fv⟨y,L⟩∉bM} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{L} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{M} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaBound{M}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fv⟨y,L⟩∉bM} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{y:fvL∉bM} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaBound{y:fvL∉bM}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma-binds:tail} \AgdaBound{y:fvL∉bM}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y∉bL} \AgdaSymbol{:} \AgdaBound{y} \AgdaFunction{notOccurBind} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{y∉bL} \AgdaSymbol{=} \AgdaFunction{lemma-binds:head} \AgdaSymbol{(}\AgdaFunction{lemma-binds:tail} \AgdaFunction{x:y∉bL}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvL∉bL} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{L}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvL∉bL} \AgdaSymbol{=} \AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bL}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fv⟨y,L⟩∉b⟨y,L⟩} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{L} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaBound{y} \AgdaFunction{notOccurBind} \AgdaBound{L} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaBound{L}\AgdaSymbol{)} \AgdaBound{L} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}}\AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fv⟨y,L⟩∉b⟨y,L⟩} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{y∉bL} \AgdaBound{fvL∉bL} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBR} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBx} \AgdaInductiveConstructor{notOccurBv} \AgdaSymbol{(}\AgdaInductiveConstructor{notOccurBEf} \AgdaSymbol{(}\AgdaFunction{notOccurBRinv} \AgdaBound{y∉bL}\AgdaSymbol{))))} \AgdaSymbol{((}\AgdaFunction{lemma-bindsR} \AgdaSymbol{(}\AgdaFunction{lemma-binds×} \AgdaFunction{lemma-bindsv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindEf} \AgdaBound{fvL∉bL}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvN[y≔L]ₙ∉bM[y≔L]ₙ} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaFunction{fv} \AgdaSymbol{(}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{fvN[y≔L]ₙ∉bM[y≔L]ₙ}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{=} \AgdaFunction{lemma-binds⊆} \<[20]%
\>[20]\AgdaSymbol{\{}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩} \AgdaFunction{++} \AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaSymbol{(}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{(}\AgdaFunction{foldCtxFV} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{N}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxFv} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{ys}\AgdaSymbol{\})} \AgdaSymbol{(λ} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{lemma-substauxFvS} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}))}\<%
\\
\>[4]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{(}\AgdaFunction{lemma-binds++} \<[36]%
\>[36]\AgdaSymbol{\{}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{N}\AgdaSymbol{\}}\<%
\\
\>[20]\AgdaIndent{36}{}\<[36]%
\>[36]\AgdaSymbol{(}\AgdaFunction{lemma-foldCtxBinds} \<[57]%
\>[57]\AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{M}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{y} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{(}\AgdaFunction{fv⟨y,L⟩∉b⟨y,L⟩} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaFunction{y∉bL} \AgdaFunction{fvL∉bL}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{fv⟨y,L⟩∉bM} \AgdaSymbol{\{}\AgdaBound{L}\AgdaSymbol{\}} \AgdaFunction{y:fvL-NB-M}\AgdaSymbol{))}\<%
\\
\>[20]\AgdaIndent{36}{}\<[36]%
\>[36]\AgdaSymbol{(}\AgdaFunction{lemma-foldCtxBinds} \<[57]%
\>[57]\AgdaSymbol{\{}\AgdaFunction{cF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{tF}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaFunction{substaux}\AgdaSymbol{\}}\<%
\\
\>[36]\AgdaIndent{57}{}\<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma-substauxBinds} \AgdaSymbol{(}\AgdaFunction{lemma-bindsR} \AgdaSymbol{(} \AgdaFunction{lemma-binds×} \AgdaFunction{lemma-bindsv} \AgdaSymbol{(}\AgdaFunction{lemmalistNotOccurBindFR→ListNotOccurBindEf} \AgdaSymbol{(}\AgdaFunction{lemma-binds++l} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bL}\AgdaSymbol{))))))}\<%
\\
\>[36]\AgdaIndent{57}{}\<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{lemma-binds++l} \AgdaSymbol{(}\AgdaFunction{lemma-binds++r} \AgdaSymbol{\{}\AgdaFunction{fv} \AgdaBound{M}\AgdaSymbol{\}} \AgdaFunction{fvM++fvN++fvL∉bM}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN[y≔L]ₙ∉bM[y≔L]ₙ} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaSymbol{(}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN[y≔L]ₙ∉bM[y≔L]ₙ} \AgdaSymbol{=} \AgdaFunction{lemma-binds:cons} \AgdaSymbol{(}\AgdaFunction{lemma-binds:head} \AgdaFunction{[x]∉bM[y≔L]ₙ}\AgdaSymbol{)} \AgdaFunction{fvN[y≔L]ₙ∉bM[y≔L]ₙ}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN[y≔L]-NB-M[y≔L]ₙ} \AgdaSymbol{:} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaFunction{fv} \AgdaSymbol{(}\AgdaBound{N} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{x:fvN[y≔L]-NB-M[y≔L]ₙ} \AgdaSymbol{=} \AgdaFunction{subst} \AgdaSymbol{(λ} \AgdaBound{xs} \AgdaSymbol{→} \AgdaFunction{ListNotOccurBind} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{xs}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{M} \AgdaFunction{[} \AgdaBound{y} \AgdaFunction{≔} \AgdaBound{L} \AgdaFunction{]ₙ}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{lemma∼fv} \AgdaSymbol{(}\AgdaFunction{σ} \AgdaSymbol{(}\AgdaFunction{lemmaSubsts} \AgdaFunction{y:fvL-NB-N}\AgdaSymbol{)))} \AgdaFunction{x:fvN[y≔L]ₙ∉bM[y≔L]ₙ}\<%
\end{code}

%<*substcompalphaproof>
\begin{code}%
\>\AgdaFunction{lemma-substComposition2} \<[25]%
\>[25]\AgdaSymbol{:} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{Ms} \AgdaSymbol{:} \AgdaFunction{TreeFTerm}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{PSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaBound{Ms}\<%
\\
\>\AgdaFunction{lemma-substComposition2} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}}\<%
\\
\> \AgdaSymbol{=} \AgdaFunction{alphaProof} \<[15]%
\>[15]\AgdaSymbol{(}\AgdaFunction{PSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{∷} \AgdaBound{y} \AgdaInductiveConstructor{∷} \AgdaInductiveConstructor{[]}\AgdaSymbol{)} \<[45]%
\>[45]\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{(}\AgdaFunction{αCompatiblePSComp} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\})}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaFunction{alpha-proof}\<%
\\
\>[2]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaInductiveConstructor{⟨} \AgdaBound{M} \AgdaInductiveConstructor{,} \AgdaBound{N} \AgdaInductiveConstructor{,} \AgdaBound{L} \AgdaInductiveConstructor{⟩}\<%
\end{code}
%</substcompalphaproof>



Parallel Reduction

\begin{code}%
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Relation} \AgdaFunction{FTerm} \<[36]%
\>[36]\<%
\\
\>\AgdaKeyword{infix} \AgdaNumber{7} \AgdaDatatype{\_⇉n\_}\<%
\end{code}

\begin{code}%
\>\AgdaKeyword{data} \AgdaDatatype{\_⇉n\_} \AgdaSymbol{:} \AgdaFunction{Rel} \AgdaKeyword{where}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nv} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{v} \AgdaBound{x} \AgdaDatatype{⇉n} \AgdaFunction{v} \AgdaBound{x}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nƛ} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{t} \AgdaSymbol{:} \AgdaFunction{FType}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{t} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{t} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉n·} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaFunction{·} \AgdaBound{N'}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉n·ₜ} \AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{t} \AgdaSymbol{:} \AgdaFunction{FType}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaFunction{·ₜ} \AgdaBound{t} \AgdaDatatype{⇉n} \AgdaBound{N} \AgdaFunction{·ₜ} \AgdaBound{t}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nΛ} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{N} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{α} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{N}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaFunction{Λ} \AgdaBound{α} \AgdaBound{N}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{⇉nβ} \AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{M} \AgdaBound{M'} \AgdaBound{N} \AgdaBound{N'} \AgdaBound{P} \AgdaSymbol{:} \AgdaFunction{FTerm}\AgdaSymbol{\}\{}\AgdaBound{t} \AgdaSymbol{:} \AgdaFunction{FType}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{M} \AgdaDatatype{⇉n} \AgdaBound{M'} \<[19]%
\>[19]\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{N'}\<%
\\
\>[2]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{→} \AgdaFunction{ƛ} \AgdaBound{x} \AgdaBound{t} \AgdaBound{M} \AgdaFunction{·} \AgdaBound{N} \AgdaDatatype{⇉n} \AgdaBound{M'} \AgdaFunction{[} \AgdaBound{x} \AgdaFunction{≔} \AgdaBound{N'} \AgdaFunction{]ₙ}\<%
\end{code}

All lemmas about ⇉n relation must have freshness premises so naive substitution behaves correctly

-- \begin{code}%
\>\AgdaComment{-- FourFTermF =  |Ef| tF |x| |Ef| tF |x| |Ef| tF |x| |Ef| tF }\<%
\\
\>\AgdaComment{-- FourFTerm = μ FourFTermF}\<%
\\
%
\\
\>\AgdaComment{-- lemma-⇉SubstN :  \{x : V\}\{M M' N N' : FTerm \}}\<%
\\
\>\AgdaComment{--                  → ListNotOccurBind \{FourFTermF\}}\<%
\\
\>\AgdaComment{--                       (x ∷ fv \{FourFTermF\} ⟨ M , M' , N , N' ⟩)}\<%
\\
\>\AgdaComment{--                       ⟨ M , M' , N , N' ⟩}\<%
\\
\>\AgdaComment{--                  → M ⇉n M' → N ⇉n N'}\<%
\\
\>\AgdaComment{--                  → M [ x ≔ N ]ₙ ⇉n M' [ x ≔ N' ]ₙ}\<%
\\
\>\AgdaComment{-- lemma-⇉SubstN = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- diam⇉n :  \{M N P : FTerm\} → ListNotOccurBind (fv M) M}\<%
\\
\>\AgdaComment{--           → M ⇉n N → M ⇉n P → ∃ (λ R → N ⇉n R × P ⇉n R)}\<%
\\
\>\AgdaComment{-- diam⇉n = \{!!\}}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- infix 7 \_⇉\_}\<%
\\
%
\\
\>\AgdaComment{-- bvcFTerm : FTerm → FTerm}\<%
\\
\>\AgdaComment{-- bvcFTerm M = proj₁ (bindersFreeαElem (fv M) M)}\<%
\\
%
\\
\>\AgdaComment{-- \_⇉\_ : Rel}\<%
\\
\>\AgdaComment{-- M ⇉ N = ∃ (λ N' → M' ⇉n N' × N' ∼α N)}\<%
\\
\>\AgdaComment{--   where}\<%
\\
\>\AgdaComment{--   M' = bvcFTerm M}\<%
\\
%
\\
\>\AgdaComment{-- lemma-⇉rightα : \{M N P : FTerm\} → M ⇉ N → N ∼α P → M ⇉ P}\<%
\\
\>\AgdaComment{-- lemma-⇉rightα \{P = P\} (N' , M'⇉N' , N'∼N) N∼P =  N' , M'⇉N' , τ N'∼N N∼P}\<%
\\
%
\\
\>\AgdaComment{-- lemma-⇉leftα : \{M N P : FTerm\} → P ∼α M → M ⇉ N → P ⇉ N}\<%
\\
\>\AgdaComment{-- lemma-⇉leftα \{M\} \{N\} \{P\} P∼M M⇉N}\<%
\\
\>\AgdaComment{--   with bvcFTerm P | bvcFTerm M | lemma-bindersFreeαFV P∼M}\<%
\\
\>\AgdaComment{-- ... | M' | .M' | refl  = M⇉N}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}


-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- ρ⇉ : Reflexive (\_⇉\_)}\<%
\\
\>\AgdaComment{-- ρ⇉ = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- τ⇉ : Transitive (\_⇉\_)}\<%
\\
\>\AgdaComment{-- τ⇉ = \{!!\} }\<%
\\
%
\\
\>\AgdaComment{-- module ⇉-Reasoning where}\<%
\\
\>\AgdaComment{--   ⇉-preorder : Preorder \_ \_ \_}\<%
\\
\>\AgdaComment{--   ⇉-preorder =  }\<%
\\
\>\AgdaComment{--              record \{ }\<%
\\
\>\AgdaComment{--              Carrier = FTerm;}\<%
\\
\>\AgdaComment{--              \_≈\_ = \_≡\_;}\<%
\\
\>\AgdaComment{--              \_∼\_ = \_⇉\_;}\<%
\\
\>\AgdaComment{--              isPreorder =  record \{}\<%
\\
\>\AgdaComment{--              isEquivalence = Relation.Binary.Setoid.isEquivalence (setoid FTerm) ;}\<%
\\
\>\AgdaComment{--              reflexive = λ \{ \{M\} \{.M\} refl → ρ⇉\};}\<%
\\
\>\AgdaComment{--              trans = τ⇉ \} \}}\<%
\\
%
\\
\>\AgdaComment{--   import Relation.Binary.PreorderReasoning as PreR⇉}\<%
\\
\>\AgdaComment{--   open PreR⇉ ⇉-preorder renaming (begin\_ to begin⇉\_;\_∼⟨\_⟩\_ to \_⇉⟨\_⟩\_;\_≈⟨\_⟩\_ to \_⇉≈⟨\_⟩\_;\_∎ to \_∎⇉) public}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- Ctx can be done generically

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- data ctx (r : Rel) : Rel where}\<%
\\
\>\AgdaComment{--   ctxinj : ∀ \{t t'\}       → r t t'        → ctx r t t'}\<%
\\
\>\AgdaComment{--   ctx·l  : ∀ \{t₁ t₁' t₂\}  → ctx r t₁ t₁'  → ctx r (t₁ · t₂)   (t₁' · t₂)}\<%
\\
\>\AgdaComment{--   ctx·r  : ∀ \{t₁ t₂ t₂'\}  → ctx r t₂ t₂'  → ctx r (t₁ · t₂)   (t₁ · t₂')}\<%
\\
\>\AgdaComment{--   ctx·ₜ  : ∀ \{t₁ t₁' t₂\}  → ctx r t₁ t₁'  → ctx r (t₁ ·ₜ t₂)  (t₁' ·ₜ t₂)}\<%
\\
\>\AgdaComment{--   ctxƛ   : ∀ \{x t t₁ t₁'\} → ctx r t₁ t₁'  → ctx r (ƛ x t t₁)  (ƛ x t t₁')}\<%
\\
\>\AgdaComment{--   ctxΛ   : ∀ \{t t₁ t₁'\}   → ctx r t₁ t₁'  → ctx r (Λ t t₁)    (Λ t t₁')}\<%
\\
%
\\
\>\AgdaComment{-- infix 1 \_▹\_ }\<%
\\
\>\AgdaComment{-- data \_▹\_ : Rel where}\<%
\\
\>\AgdaComment{--   ▹β  :  \{M N : FTerm\}\{x : V\}\{t : FType\} }\<%
\\
\>\AgdaComment{--       →  ƛ x t M · N ▹ M [ x ≔ N ]}\<%
\\
%
\\
\>\AgdaComment{-- infix 4 \_→β\_}\<%
\\
\>\AgdaComment{-- \_→β\_ : Rel}\<%
\\
\>\AgdaComment{-- \_→β\_ = ctx \_▹\_}\<%
\\
%
\\
\>\AgdaComment{-- infix 4 \_→α\_ }\<%
\\
\>\AgdaComment{-- \_→α\_ : Rel}\<%
\\
\>\AgdaComment{-- \_→α\_ = \_→β\_ ∪ \_∼α\_}\<%
\\
%
\\
\>\AgdaComment{-- infix 4 \_→α*\_}\<%
\\
\>\AgdaComment{-- \_→α*\_ : Rel}\<%
\\
\>\AgdaComment{-- \_→α*\_ = star \_→α\_}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
%
\\
\>\AgdaComment{-- -- This 3 results are what I need !}\<%
\\
%
\\
\>\AgdaComment{-- lemma→α⊆⇉ : \_→α\_ ⊆ \_⇉\_}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctxinj (▹β \{M\}))) = \{! ⇉β ρ⇉ ρ⇉!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctx·l x))   = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctx·r x))   = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctx·ₜ x))   = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctxƛ x₁))   = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₁ (ctxΛ x))    = \{!!\}}\<%
\\
\>\AgdaComment{-- lemma→α⊆⇉ (inj₂ (∼αR y))     = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- lemma⇉⊆→α* : \_⇉\_ ⊆ \_→α*\_}\<%
\\
\>\AgdaComment{-- lemma⇉⊆→α* = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- diam⇉ : diamond \_⇉\_}\<%
\\
\>\AgdaComment{-- diam⇉ = \{!!\}}\<%
\\
%
\\
\>\AgdaComment{-- lemma-CR⇉ : cr \_⇉\_}\<%
\\
\>\AgdaComment{-- lemma-CR⇉ = diamond-cr diam⇉}\<%
\\
\>\AgdaComment{-- --}\<%
\\
\>\AgdaComment{-- lemma-CR→α : cr \_→α\_}\<%
\\
\>\AgdaComment{-- lemma-CR→α = cr-⊆ lemma→α⊆⇉ lemma⇉⊆→α* lemma-CR⇉}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}




-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- open ⇉-Reasoning}\<%
\\
%
\\
\>\AgdaComment{-- Psubst⇉ : \{N N' : FTerm\}(x : V) → FTerm → Set}\<%
\\
\>\AgdaComment{-- Psubst⇉ \{N\} \{N'\} x M = \{M' : FTerm\} → M ⇉ M' → N ⇉ N' → M [ x ≔ N ] ⇉ M' [ x ≔ N' ]}\<%
\\
%
\\
\>\AgdaComment{-- αCompP⇉[] : \{N N' : FTerm\}(x : V) → αCompatiblePred (Psubst⇉ \{N\} \{N'\} x)}\<%
\\
\>\AgdaComment{-- αCompP⇉[] \{N\} \{N'\} x \{M\} \{P\} M∼P P⇉[]M \{M'\} P⇉M' N⇉N' }\<%
\\
\>\AgdaComment{--   =  begin⇉}\<%
\\
\>\AgdaComment{--        P [ x ≔ N ]}\<%
\\
\>\AgdaComment{--      ⇉⟨ \{!!\} ⟩}\<%
\\
\>\AgdaComment{--        M' [ x ≔ N' ]}\<%
\\
\>\AgdaComment{--      ∎⇉}\<%
\\
%
\\
\>\AgdaComment{-- lemma⇉Subst : \{N N' : FTerm\}(x : V)(M : FTerm) → Psubst⇉ \{N\} \{N'\} x M}\<%
\\
\>\AgdaComment{-- lemma⇉Subst \{N\} \{N'\} x M = \{!!\}}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}

-- \begin{code}%
\>\<%
\\
\>\AgdaComment{-- RelF : Functor}\<%
\\
\>\AgdaComment{-- RelF = tF |x| tF}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}




==> GenericProgramming/GPBindings.tex <==
\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{GPBindings} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Function}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{fold}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Bool}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.List} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{unfold}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Unit}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Atom}\<%
\\
%
\\
\>\AgdaKeyword{infixr} \AgdaNumber{20} \AgdaInductiveConstructor{\_|+|\_}\<%
\\
\>\AgdaKeyword{infixr} \AgdaNumber{21} \AgdaInductiveConstructor{\_|x|\_}\<%
\\
%
\\
\>\AgdaFunction{Sort} \<[6]%
\>[6]\AgdaSymbol{=} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{V} \<[6]%
\>[6]\AgdaSymbol{=} \AgdaFunction{Atom}\<%
\\
\>\AgdaFunction{\_≟v\_} \<[6]%
\>[6]\AgdaSymbol{=} \AgdaFunction{Data.Nat.\_≟\_}\<%
\\
\>\AgdaFunction{\_≟S\_} \<[6]%
\>[6]\AgdaSymbol{=} \AgdaFunction{Data.Nat.\_≟\_}\<%
\end{code}

%<*functor>
\begin{code}%
\>\AgdaKeyword{data} \AgdaDatatype{Functor} \AgdaSymbol{:} \AgdaPrimitiveType{Set₁} \AgdaKeyword{where} \<[40]%
\>[40]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|1|} \<[9]%
\>[9]\AgdaSymbol{:} \<[34]%
\>[34]\AgdaDatatype{Functor}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|R|} \<[9]%
\>[9]\AgdaSymbol{:} \<[34]%
\>[34]\AgdaDatatype{Functor}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|E|} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaPrimitiveType{Set} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor} \<[49]%
\>[49]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|Ef|} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaDatatype{Functor} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor} \<[49]%
\>[49]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{\_|+|\_} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaDatatype{Functor} \<[20]%
\>[20]\AgdaSymbol{→} \AgdaDatatype{Functor} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor} \<[46]%
\>[46]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{\_|x|\_} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaDatatype{Functor} \<[20]%
\>[20]\AgdaSymbol{→} \AgdaDatatype{Functor} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|v|} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaFunction{Sort} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaInductiveConstructor{|B|} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaFunction{Sort} \<[20]%
\>[20]\AgdaSymbol{→} \AgdaDatatype{Functor} \<[31]%
\>[31]\AgdaSymbol{→} \<[34]%
\>[34]\AgdaDatatype{Functor}\<%
\end{code}
%</functor>

%<*interpret>
\begin{code}%
\>\AgdaKeyword{mutual}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦\_⟧} \AgdaSymbol{:} \AgdaDatatype{Functor} \AgdaSymbol{→} \AgdaPrimitiveType{Set} \AgdaSymbol{→} \AgdaPrimitiveType{Set} \<[38]%
\>[38]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|1|} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaSymbol{\_} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaRecord{⊤}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|R|} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaBound{A} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaBound{A}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|E|} \<[12]%
\>[12]\AgdaBound{B} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaSymbol{\_} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaBound{B}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|Ef|} \<[12]%
\>[12]\AgdaBound{F} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaSymbol{\_} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaDatatype{μ} \AgdaBound{F}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaBound{F} \AgdaInductiveConstructor{|+|} \<[12]%
\>[12]\AgdaBound{G} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaBound{A} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \<[31]%
\>[31]\AgdaDatatype{⊎} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaBound{A}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaBound{F} \AgdaInductiveConstructor{|x|} \<[12]%
\>[12]\AgdaBound{G} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaBound{A} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \<[31]%
\>[31]\AgdaFunction{×} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaBound{A}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|v|} \<[9]%
\>[9]\AgdaBound{S} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaSymbol{\_} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaFunction{V}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{⟦} \AgdaInductiveConstructor{|B|} \<[9]%
\>[9]\AgdaBound{S} \<[12]%
\>[12]\AgdaBound{G} \<[15]%
\>[15]\AgdaFunction{⟧} \AgdaBound{A} \<[20]%
\>[20]\AgdaSymbol{=} \AgdaFunction{V} \<[31]%
\>[31]\AgdaFunction{×} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaBound{A}\<%
\end{code}
%</interpret>

%<*mu>
\begin{code}%
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{data} \AgdaDatatype{μ} \AgdaSymbol{(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{:} \AgdaPrimitiveType{Set} \AgdaKeyword{where}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{⟨\_⟩} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F}\<%
\end{code}
%</mu>


%<*foldtermination>
\begin{code}%
\>\AgdaFunction{mapF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{A} \AgdaBound{B} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{A} \AgdaSymbol{→} \AgdaBound{B}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{B} \<[62]%
\>[62]\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[12]%
\>[12]\AgdaBound{S}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaBound{x} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{x}\<%
\\
\>\AgdaFunction{mapF} \AgdaInductiveConstructor{|1|} \<[19]%
\>[19]\AgdaBound{f} \AgdaInductiveConstructor{tt} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[12]%
\>[12]\AgdaBound{A}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{e}\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[12]%
\>[12]\AgdaBound{F}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{e}\<%
\\
\>\AgdaFunction{mapF} \AgdaInductiveConstructor{|R|} \<[19]%
\>[19]\AgdaBound{f} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{f} \AgdaBound{e}\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[14]%
\>[14]\AgdaBound{G₂}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{inj₁} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaFunction{mapF} \AgdaBound{G₁} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[14]%
\>[14]\AgdaBound{G₂}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaFunction{mapF} \AgdaBound{G₂} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)} \<[54]%
\>[54]\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[14]%
\>[14]\AgdaBound{G₂}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaFunction{mapF} \AgdaBound{G₁} \AgdaBound{f} \AgdaBound{e₁} \<[48]%
\>[48]\AgdaInductiveConstructor{,} \AgdaFunction{mapF} \AgdaBound{G₂} \<[59]%
\>[59]\AgdaBound{f} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{mapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \<[11]%
\>[11]\AgdaBound{S} \<[14]%
\>[14]\AgdaBound{G}\AgdaSymbol{)} \<[19]%
\>[19]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{x} \<[48]%
\>[48]\AgdaInductiveConstructor{,} \AgdaFunction{mapF} \AgdaBound{G} \<[59]%
\>[59]\AgdaBound{f} \AgdaBound{e}\<%
\end{code}
%</foldtermination>


%<*foldtermination2>
\begin{code}%
\>\AgdaSymbol{\{-\#} \AgdaKeyword{TERMINATING} \AgdaSymbol{\#-\}}\<%
\\
\>\AgdaFunction{foldT} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaBound{A}\<%
\\
\>\AgdaFunction{foldT} \AgdaBound{F} \AgdaBound{f} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \AgdaSymbol{=} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{mapF} \AgdaBound{F} \AgdaSymbol{(}\AgdaFunction{foldT} \AgdaBound{F} \AgdaBound{f}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}
%</foldtermination2>


--unfold : {F : Functor} → μ F → ⟦ F ⟧ (μ F)
--unfold ⟨ e ⟩ = e

%<*foldmap>
\begin{code}%
\>\AgdaFunction{foldmap} \AgdaSymbol{:} \<[11]%
\>[11]\AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaBound{G} \<[26]%
\>[26]\AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \<[40]%
\>[40]\AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{→} \<[57]%
\>[57]\AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaBound{A}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaInductiveConstructor{|1|} \<[24]%
\>[24]\AgdaBound{f} \AgdaInductiveConstructor{tt} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{tt} \<[43]%
\>[43]\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \<[24]%
\>[24]\AgdaBound{f} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{f} \<[46]%
\>[46]\AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{F} \<[61]%
\>[61]\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)} \<[66]%
\>[66]\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[17]%
\>[17]\AgdaBound{A}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaBound{e} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{e}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[17]%
\>[17]\AgdaBound{G}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaBound{e} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{e}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{inj₁} \<[46]%
\>[46]\AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G₁} \<[61]%
\>[61]\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{inj₂} \<[46]%
\>[46]\AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G₂} \<[61]%
\>[61]\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{f} \AgdaBound{e₁} \<[60]%
\>[60]\AgdaInductiveConstructor{,} \AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G₂} \<[76]%
\>[76]\AgdaBound{f} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[17]%
\>[17]\AgdaBound{S}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaBound{x} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{x}\<%
\\
\>\AgdaFunction{foldmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \<[19]%
\>[19]\AgdaBound{G}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{x} \<[60]%
\>[60]\AgdaInductiveConstructor{,} \AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \<[76]%
\>[76]\AgdaBound{f} \AgdaBound{e}\<%
\end{code}
%</foldmap>

%<*foldmap2>
\begin{code}%
\>\AgdaFunction{fold} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaBound{A} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaBound{A}\<%
\\
\>\AgdaFunction{fold} \AgdaBound{F} \AgdaBound{f} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{foldmap} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \AgdaBound{f} \AgdaBound{e} \<%
\end{code}
%</foldmap2>

Recursion

\begin{code}%
\>\AgdaFunction{recmap} \AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaBound{G} \<[25]%
\>[25]\AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)}\<%
\\
\>[4]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaBound{A} \AgdaFunction{×} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \<[32]%
\>[32]\<%
\\
\>[4]\AgdaIndent{7}{}\<[7]%
\>[7]\AgdaSymbol{→} \<[10]%
\>[10]\AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaBound{A} \AgdaFunction{×} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \<[40]%
\>[40]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaBound{x} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaBound{x} \<[44]%
\>[44]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaInductiveConstructor{|1|} \<[22]%
\>[22]\AgdaBound{f} \AgdaInductiveConstructor{tt} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaInductiveConstructor{tt} \<[44]%
\>[44]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{A}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaBound{e} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaBound{e} \<[44]%
\>[44]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaBound{e} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaBound{e} \<[44]%
\>[44]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \<[22]%
\>[22]\AgdaBound{f} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{F} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)} \AgdaInductiveConstructor{,} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaInductiveConstructor{inj₁} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{G₁} \<[62]%
\>[62]\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)} \<[67]%
\>[67]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \<[48]%
\>[48]\AgdaSymbol{(}\AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{G₂} \<[62]%
\>[62]\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{f} \AgdaBound{e₁} \<[60]%
\>[60]\AgdaInductiveConstructor{,} \AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{G₂} \AgdaBound{f} \AgdaBound{e₂} \<[79]%
\>[79]\<%
\\
\>\AgdaFunction{recmap} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[22]%
\>[22]\AgdaBound{f} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[39]%
\>[39]\AgdaSymbol{=} \AgdaBound{x} \<[60]%
\>[60]\AgdaInductiveConstructor{,} \AgdaFunction{recmap} \AgdaBound{F} \AgdaBound{G} \<[75]%
\>[75]\AgdaBound{f} \AgdaBound{e}\<%
\\
%
\\
\>\AgdaFunction{rec} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaBound{A} \AgdaFunction{×} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{A}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaBound{A}\<%
\\
\>\AgdaFunction{rec} \AgdaSymbol{\{}\AgdaArgument{F} \AgdaSymbol{=} \AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{f} \AgdaBound{e} \AgdaSymbol{=} \AgdaField{proj₁} \AgdaSymbol{(}\AgdaFunction{recmap} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}

Now the function $f$\ has an explicit context $\mu C$, and the returned type is a functorial one.

-- foldmapCtx  :  {C H : Functor}(F G  : Functor)
--             →  (μ C → ⟦ F ⟧ (μ H)  → μ H)
--             →  μ C →  ⟦ G ⟧ (μ F) → ⟦ G ⟧ (μ H)
-- foldmapCtx F (|v|   S)     f c x          =  x
-- foldmapCtx F |1|           f c tt         =  tt
-- foldmapCtx F (|E|   A)     f c e          =  e
-- foldmapCtx F (|Ef|  G)     f c e          =  e
-- foldmapCtx F |R|           f c ⟨ e ⟩      =  f c   (foldmapCtx F F   f c e) 
-- foldmapCtx F (G₁ |+|  G₂)  f c (inj₁ e)   =  inj₁  (foldmapCtx F G₁  f c e)
-- foldmapCtx F (G₁ |+|  G₂)  f c (inj₂ e)   =  inj₂  (foldmapCtx F G₂  f c e)
-- foldmapCtx F (G₁ |x|  G₂)  f c (e₁ , e₂)  =  foldmapCtx F G₁  f c e₁   , 
--                                              foldmapCtx F G₂  f c e₂
-- foldmapCtx F (|B| S   G)   f c (x , e)    =  x                        , 
--                                              foldmapCtx F G   f c e
-- foldCtx {C} {H} F f c = foldmapCtx {C} {H} F |R| f c

%<*foldCtx>
\begin{code}%
\>\AgdaFunction{foldCtx} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\<%
\\
\>\AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaSymbol{=} \AgdaFunction{fold} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)}\<%
\end{code}
%</foldCtx>

-- recmapCtx :  {C H : Functor}(F G  : Functor)
--               → (μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F))  → μ H)
--               → μ C →  ⟦ G ⟧ (μ F) → ⟦ G ⟧ (μ (|Ef| H |x| |Ef| F))
-- recmapCtx F (|v| S)      f c x          =  x
-- recmapCtx F |1|          f c tt         =  tt
-- recmapCtx F (|E| A)      f c e          =  e
-- recmapCtx F (|Ef| G)     f c e          =  e
-- recmapCtx F |R|          f c ⟨ e ⟩      =  ⟨ f c  (recmapCtx F F   f c e) , ⟨ e ⟩ ⟩
-- recmapCtx F (G₁ |+| G₂)  f c (inj₁ e)   =  inj₁   (recmapCtx F G₁  f c e)
-- recmapCtx F (G₁ |+| G₂)  f c (inj₂ e)   =  inj₂   (recmapCtx F G₂  f c e)
-- recmapCtx F (G₁ |x| G₂)  f c (e₁ , e₂)  =  recmapCtx F G₁  f c e₁  , 
--                                            recmapCtx F G₂  f c e₂
-- recmapCtx F (|B| S G)    f c (x , e)    =  x                      , 
--                                            recmapCtx F G   f c e

-- recCtx :  {C H : Functor}(F : Functor)
--            → (μ C → ⟦ F ⟧ (μ (|Ef| H |x| |Ef| F)) → μ H) -- (μ H × μ F)
--            → μ C → μ F → μ H
-- recCtx {C} {H} F f c e with recmapCtx {C} {H} F |R| f c e
-- ... | ⟨ h , _ ⟩ = h

Recursion with contexts.

\begin{code}%
\>\AgdaFunction{recCtx} \AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)}\<%
\\
\>[7]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H} \AgdaFunction{×} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaComment{-- (μ H × μ F)}\<%
\\
\>[7]\AgdaIndent{11}{}\<[11]%
\>[11]\AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\<%
\\
\>\AgdaFunction{recCtx} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaSymbol{=} \AgdaFunction{rec} \AgdaSymbol{\{}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)}\<%
\end{code}

-- fold fusion
-- lemma-foldSFusion : {C H : Functor}(F : Functor)(f : μ C → ⟦ F ⟧ (μ H) → μ H)
-- {μ C → μ F → μ H                f ∘ foldS F f c ≡ foldS F f' c'

-- mapFh : {F : Functor}(G : Functor)(P : μ F → Set) → ((a : μ F) → P a) → (x : ⟦ G ⟧ (μ F)) → fih G P x
-- mapFh (|v| S)    P f n        = tt

-- mapFh |1|        P f tt       = tt
-- mapFh (|E| B)    P f b        = tt
-- mapFh (|Ef| G)   P f b        = tt
-- mapFh |R|        P f x        = f x
-- mapFh (G |+| G') P f (inj₁ x) = mapFh G  P f x
-- mapFh (G |+| G') P f (inj₂ y) = mapFh G' P f y
-- mapFh (G |x| G') P f (x , y)  = mapFh G  P f x , mapFh G' P f y
-- mapFh (|B| S G)  P f (x , y)  = mapFh G  P f y

-- {-# TERMINATING #-}
-- foldInd : (F : Functor)(P : μ F → Set)    
--   → ((e : ⟦ F ⟧ (μ F)) → fih F P e →  P ⟨ e ⟩)  
--   → (e : μ F) → P e
-- foldInd F P hi ⟨ e ⟩ = hi e (mapFh F P (foldInd F P hi) e)

Primitive Induction

%<*primIndih>
\begin{code}%
\>\AgdaFunction{fih} \<[5]%
\>[5]\AgdaSymbol{:} \<[8]%
\>[8]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>\AgdaFunction{fih} \AgdaInductiveConstructor{|1|} \<[18]%
\>[18]\AgdaBound{P} \AgdaInductiveConstructor{tt} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fih} \AgdaInductiveConstructor{|R|} \<[18]%
\>[18]\AgdaBound{P} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaBound{P} \AgdaBound{e}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[11]%
\>[11]\AgdaBound{B}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[11]%
\>[11]\AgdaBound{G}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaBound{e} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[13]%
\>[13]\AgdaBound{G₂}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \<[27]%
\>[27]\AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaFunction{fih} \AgdaBound{G₁} \<[42]%
\>[42]\AgdaBound{P} \AgdaBound{e}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[13]%
\>[13]\AgdaBound{G₂}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \<[27]%
\>[27]\AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaFunction{fih} \AgdaBound{G₂} \<[42]%
\>[42]\AgdaBound{P} \AgdaBound{e} \<[46]%
\>[46]\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[13]%
\>[13]\AgdaBound{G₂}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \<[27]%
\>[27]\AgdaBound{e₂}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaFunction{fih} \AgdaBound{G₁} \<[42]%
\>[42]\AgdaBound{P} \AgdaBound{e₁} \AgdaFunction{×} \AgdaFunction{fih} \AgdaBound{G₂} \AgdaBound{P} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[11]%
\>[11]\AgdaBound{S}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaBound{x} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaRecord{⊤}\<%
\\
\>\AgdaFunction{fih} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \<[13]%
\>[13]\AgdaBound{G}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{P} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \<[27]%
\>[27]\AgdaBound{e}\AgdaSymbol{)} \<[32]%
\>[32]\AgdaSymbol{=} \AgdaFunction{fih} \AgdaBound{G} \<[42]%
\>[42]\AgdaBound{P} \AgdaBound{e}\<%
\end{code}
%</primIndih>

%<*primInd>
\begin{code}%
\>\AgdaFunction{foldmapFh} \AgdaSymbol{:} \<[13]%
\>[13]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)}\<%
\\
\>[11]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \AgdaSymbol{((}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaBound{F} \AgdaBound{P} \AgdaBound{e} \AgdaSymbol{→} \<[49]%
\>[49]\AgdaBound{P} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaBound{G} \AgdaBound{P} \AgdaBound{x}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaInductiveConstructor{|1|} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaInductiveConstructor{tt} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaBound{hi} \AgdaBound{e} \AgdaSymbol{(}\AgdaFunction{foldmapFh} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{F} \AgdaBound{P} \AgdaBound{hi} \AgdaBound{e}\AgdaSymbol{)} \<[74]%
\>[74]\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[17]%
\>[17]\AgdaBound{B}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{b} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[17]%
\>[17]\AgdaBound{F}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{b} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \<[36]%
\>[36]\AgdaBound{e}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaFunction{foldmapFh} \AgdaBound{G₁} \<[58]%
\>[58]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{e}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \<[36]%
\>[36]\AgdaBound{e}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaFunction{foldmapFh} \AgdaBound{G₂} \<[58]%
\>[58]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{e}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[19]%
\>[19]\AgdaBound{G₂}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaSymbol{(}\AgdaBound{e₁} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaFunction{foldmapFh} \AgdaBound{G₁} \<[58]%
\>[58]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaFunction{foldmapFh} \AgdaBound{G₂} \<[82]%
\>[82]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[17]%
\>[17]\AgdaBound{S}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{n} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{foldmapFh} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \<[19]%
\>[19]\AgdaBound{G}\AgdaSymbol{)} \<[24]%
\>[24]\AgdaBound{P} \AgdaBound{hi} \AgdaSymbol{(}\AgdaBound{x} \<[34]%
\>[34]\AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=} \<[44]%
\>[44]\AgdaFunction{foldmapFh} \AgdaBound{G} \<[58]%
\>[58]\AgdaBound{P} \AgdaBound{hi} \AgdaBound{e}\<%
\end{code}
%</primInd>


%<*primInd2>
\begin{code}%
\>\AgdaFunction{foldInd} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{P} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{((}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{fih} \AgdaBound{F} \AgdaBound{P} \AgdaBound{e} \AgdaSymbol{→} \<[75]%
\>[75]\AgdaBound{P} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaSymbol{(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaBound{P} \AgdaBound{e}\<%
\\
\>\AgdaFunction{foldInd} \AgdaBound{F} \AgdaBound{P} \AgdaBound{hi} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{foldmapFh} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \AgdaBound{P} \AgdaBound{hi} \AgdaBound{e}\<%
\end{code}
%</primInd2>



%</primInd>

Size

\begin{code}%
\>\AgdaFunction{sizeF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{e} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaNumber{1}\<%
\\
\>\AgdaFunction{sizeF} \AgdaInductiveConstructor{|1|} \<[18]%
\>[18]\AgdaBound{e} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaNumber{1}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaBound{e} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaNumber{1}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[18]%
\>[18]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaBound{F} \AgdaBound{e}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁} \AgdaPrimitive{+} \AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[18]%
\>[18]\AgdaSymbol{(}\AgdaBound{x} \<[22]%
\>[22]\AgdaInductiveConstructor{,} \AgdaBound{y}\AgdaSymbol{)} \<[29]%
\>[29]\AgdaSymbol{=} \AgdaInductiveConstructor{suc} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{y}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{size} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{ℕ}\<%
\\
\>\AgdaFunction{size} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{sizeF} \AgdaInductiveConstructor{|R|} \AgdaBound{e}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat.Properties}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{DecTotalOrder} \AgdaFunction{Data.Nat.decTotalOrder} \AgdaKeyword{using} \AgdaSymbol{()} \AgdaKeyword{renaming} \AgdaSymbol{(}refl \AgdaSymbol{to} ≤-refl\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{≤-Reasoning}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{begin\_} \AgdaSymbol{to} \AgdaFunction{start\_}\AgdaSymbol{;} \AgdaFunction{\_∎} \AgdaSymbol{to} \AgdaFunction{\_◽}\AgdaSymbol{;} \AgdaFunction{\_≡⟨\_⟩\_} \AgdaSymbol{to} \AgdaFunction{\_≤⟨\_⟩'\_}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \AgdaSymbol{→} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e} \AgdaFunction{>} \AgdaNumber{0}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaBound{e} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaBound{e} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[40]%
\>[40]\AgdaSymbol{=} \<[43]%
\>[43]\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaBound{e} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[40]%
\>[40]\AgdaSymbol{=} \AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{=} \<[44]%
\>[44]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{start}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{suc} \AgdaInductiveConstructor{zero}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{e₁} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaFunction{m≤m+n} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁}\AgdaSymbol{)} \AgdaPrimitive{+} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂}\AgdaSymbol{)} \<[34]%
\>[34]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaFunction{≤-refl} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{◽}\<%
\\
\>\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[41]%
\>[41]\AgdaSymbol{=}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{start}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{suc} \AgdaInductiveConstructor{zero} \<[13]%
\>[13]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaInductiveConstructor{s≤s} \AgdaInductiveConstructor{z≤n} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{suc} \AgdaSymbol{(}\AgdaInductiveConstructor{suc} \AgdaInductiveConstructor{zero}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaInductiveConstructor{s≤s} \AgdaSymbol{(}\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e}\AgdaSymbol{)} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaNumber{1} \AgdaPrimitive{+} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{≤⟨} \AgdaFunction{≤-refl} \AgdaFunction{⟩}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{sizeF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{◽}\<%
\end{code}


  
  


==> GenericProgramming/Swap.tex <==
Swap

\begin{code}%
\>\AgdaKeyword{module} \AgdaModule{Swap} \AgdaKeyword{where}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Atom}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{GPBindings} \<[23]%
\>[23]\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Nat.NatProperties}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Function}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Nat} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{fold}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Unit}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Empty}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Nullary}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Sum}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Data.Product} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaFunction{swap}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Relation.Binary.PropositionalEquality} \AgdaSymbol{as} \AgdaModule{PropEq} \AgdaKeyword{hiding} \AgdaSymbol{(}\AgdaInductiveConstructor{[\_]}\AgdaSymbol{)}\<%
\\
\>\AgdaKeyword{open} \AgdaModule{PropEq.}\AgdaModule{≡-Reasoning} \AgdaKeyword{renaming} \AgdaSymbol{(}\AgdaFunction{begin\_} \AgdaSymbol{to} \AgdaFunction{begin≡\_}\AgdaSymbol{;}\AgdaFunction{\_∎} \AgdaSymbol{to} \AgdaFunction{\_■}\AgdaSymbol{)}\<%
\end{code}

%<*swapF>
\begin{code}%
\>\AgdaFunction{swapF} \<[7]%
\>[7]\AgdaSymbol{:} \<[10]%
\>[10]\AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{Sort} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{swapF} \AgdaInductiveConstructor{|1|} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaInductiveConstructor{tt} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{tt}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{|R|} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{⟨} \AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \<[14]%
\>[14]\AgdaSymbol{\_)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{e}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \<[14]%
\>[14]\AgdaBound{G}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{⟨} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[15]%
\>[15]\AgdaBound{G₂}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G₁} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \<[15]%
\>[15]\AgdaBound{G₂}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G₂} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \<[15]%
\>[15]\AgdaBound{G₂}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaFunction{swapF} \AgdaBound{G₁} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e₁} \<[59]%
\>[59]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G₂} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e₂}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \<[14]%
\>[14]\AgdaBound{S'}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \<[11]%
\>[11]\AgdaSymbol{\_} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaFunction{（} \AgdaBound{a} \AgdaFunction{∙} \AgdaBound{b} \AgdaFunction{）ₐ} \AgdaBound{c}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[11]%
\>[11]\AgdaSymbol{\_} \<[37]%
\>[37]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{c}\<%
\\
\>\AgdaFunction{swapF} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \<[15]%
\>[15]\AgdaBound{G}\AgdaSymbol{)} \<[20]%
\>[20]\AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaBound{c} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟S} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \<[11]%
\>[11]\AgdaSymbol{\_} \<[36]%
\>[36]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaFunction{（} \AgdaBound{a} \AgdaFunction{∙} \AgdaBound{b} \AgdaFunction{）ₐ} \<[53]%
\>[53]\AgdaBound{c} \<[59]%
\>[59]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[11]%
\>[11]\AgdaSymbol{\_} \<[36]%
\>[36]\AgdaSymbol{=} \<[40]%
\>[40]\AgdaBound{c} \<[59]%
\>[59]\AgdaInductiveConstructor{,} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\<%
\end{code}
%</swapF>

%<*swap>
\begin{code}%
\>\AgdaFunction{swap} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Sort} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F}\<%
\\
\>\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{swapF} \AgdaInductiveConstructor{|R|} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\<%
\end{code}
%</swap>

\begin{code}%
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{a} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\})} \<[131]%
\>[131]\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S'}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{sym} \AgdaFunction{lemma（aa）b≡b}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{\}} \<[28]%
\>[28]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[46]%
\>[46]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaFunction{lemma（aa）b≡b}\AgdaSymbol{)} \<[80]%
\>[80]\AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<[114]%
\>[114]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapId} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaBound{b} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\})} \<[149]%
\>[149]\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S'}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{sym} \AgdaFunction{lemma（ab）（ab）c≡c}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaFunction{lemma（ab）（ab）c≡c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<[123]%
\>[123]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaBound{b} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{b} \AgdaBound{a} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\})} \<[149]%
\>[149]\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S'}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{lemma∙ₐcomm} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{\}} \<[30]%
\>[30]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[52]%
\>[52]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐcomm} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<[126]%
\>[126]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemmaSwapIdemComm} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaBound{b} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{e} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{b} \AgdaBound{a} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapIdemComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaSymbol{=} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{begin≡}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{b} \AgdaBound{a} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{lemmaSwapComm} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)\}} \AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaFunction{sym} \AgdaSymbol{(}\AgdaFunction{lemmaSwapIdem} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaFunction{⟩} \<[54]%
\>[54]\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{■}\AgdaSymbol{)}\<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaBound{d} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\> \AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{c} \AgdaBound{d} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{a} \AgdaFunction{∙} \AgdaBound{b} \AgdaFunction{）ₐ} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{（} \AgdaBound{a} \AgdaFunction{∙} \AgdaBound{b} \AgdaFunction{）ₐ} \AgdaBound{d}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\})} \<[200]%
\>[200]\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S'}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{lemma∙ₐdistributive} \AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaBound{d} \AgdaBound{e}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{\}} \<[39]%
\>[39]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[69]%
\>[69]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemma∙ₐdistributive} \AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaBound{d} \AgdaBound{x}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<[149]%
\>[149]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaSymbol{\_} \<[46]%
\>[46]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\})} \<%
\end{code}

\begin{code}%
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaBound{S'} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaBound{b} \AgdaBound{c} \AgdaBound{d} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{S} \AgdaFunction{≢} \AgdaBound{S'}\<%
\\
\>[2]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{→} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S'} \AgdaBound{a} \AgdaBound{b} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{c} \AgdaBound{d} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{c} \AgdaBound{d} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S'} \AgdaBound{a} \AgdaBound{b} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[74]%
\>[74]\AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[74]%
\>[74]\AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[74]%
\>[74]\AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[74]%
\>[74]\AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaSymbol{(}\AgdaInductiveConstructor{⟨\_⟩}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{S≢S'} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e'}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)} \<[232]%
\>[232]\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S''}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[75]%
\>[75]\AgdaBound{S≢S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{S''≡S}\AgdaSymbol{)} \AgdaBound{S''≡S'}\AgdaSymbol{))}\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[15]%
\>[15]\AgdaBound{S''≢S} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|v|} \AgdaBound{S''}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[75]%
\>[75]\AgdaBound{S≢S'}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{S''≢S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S} \AgdaSymbol{=} \AgdaInductiveConstructor{refl} \<[28]%
\>[28]\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[15]%
\>[15]\AgdaBound{S''≢S} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S''} \AgdaBound{G}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[75]%
\>[75]\AgdaBound{S≢S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S} \AgdaSymbol{=} \AgdaFunction{⊥-elim} \AgdaSymbol{(}\AgdaBound{S≢S'} \AgdaSymbol{(}\AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{sym} \AgdaBound{S''≡S}\AgdaSymbol{)} \AgdaBound{S''≡S'}\AgdaSymbol{))} \<[64]%
\>[64]\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[15]%
\>[15]\AgdaBound{S''≢S} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[83]%
\>[83]\AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S''} \AgdaBound{G}\AgdaSymbol{\}} \<[41]%
\>[41]\AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[75]%
\>[75]\AgdaBound{S≢S'}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[10]%
\>[10]\AgdaBound{S''≢S'} \AgdaKeyword{with} \AgdaBound{S''} \AgdaFunction{≟v} \AgdaBound{S}\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaBound{S''≡S} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[83]%
\>[83]\AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)} \<[109]%
\>[109]\<%
\\
\>\AgdaSymbol{...} \<[9]%
\>[9]\AgdaSymbol{|} \AgdaInductiveConstructor{no} \<[15]%
\>[15]\AgdaBound{S''≢S} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapDistributiveF≢} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[83]%
\>[83]\AgdaSymbol{\{}\AgdaBound{a}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{b}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{S≢S'}\AgdaSymbol{)}\<%
\end{code}

-- swap : (F : Functor) → Sort → V → V → μ F → μ F
-- swap F S a b = fold F (⟨_⟩ ∘ swapaux {F} F)
--   where
--   swapaux : {F : Functor}(G : Functor) → ⟦ G ⟧ (μ F) → ⟦ G ⟧ (μ F)
--   swapaux (|v| S')   c
--     with  S' ≟S S
--   ... | yes _                 = （ a ∙ b ）ₐ c
--   ... | no  _                 = c 
--   swapaux |1|        e        = e
--   swapaux (|E| A)    e        = e
--   swapaux (|Ef| G)   e        = e
--   swapaux |R|        e        = e
--   swapaux (G |+| G₁) e        = e
--   swapaux (G |x| G₁) e        =  e
--   swapaux (|B| S' G) (x , e)
--     with S' ≟v S
--   ... | yes _                 = （ a ∙ b ）ₐ  x , e
--   ... | no  _                 =              x , e

\begin{code}%
\>\AgdaFunction{lemmaSwapSize} \AgdaSymbol{:} \<[17]%
\>[17]\AgdaSymbol{(}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)(}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{)(}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))} \<[69]%
\>[69]\<%
\\
\>[4]\AgdaIndent{17}{}\<[17]%
\>[17]\AgdaSymbol{→} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S'}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaInductiveConstructor{|1|} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{A}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{lemmaSwapSize} \AgdaBound{G} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G} \AgdaInductiveConstructor{|+|} \AgdaBound{G₁}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G} \AgdaInductiveConstructor{|x|} \AgdaBound{G₁}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{e} \AgdaInductiveConstructor{,} \AgdaBound{e'}\AgdaSymbol{)} \<[44]%
\>[44]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaPrimitive{\_+\_} \AgdaSymbol{(}\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e'}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S'} \AgdaBound{G}\AgdaSymbol{)} \<[28]%
\>[28]\AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[43]%
\>[43]\AgdaKeyword{with} \AgdaBound{S'} \AgdaFunction{≟v} \AgdaBound{S} \<[56]%
\>[56]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \<[13]%
\>[13]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{suc} \AgdaSymbol{(}\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[13]%
\>[13]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{suc} \AgdaSymbol{(}\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
%
\\
\>\AgdaKeyword{mutual}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaKeyword{data} \AgdaDatatype{AccF} \AgdaSymbol{(}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{:} \AgdaSymbol{(}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaPrimitiveType{Set} \AgdaKeyword{where}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accv} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{a} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|v|} \AgdaBound{S}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaBound{a}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{acc1} \<[11]%
\>[11]\AgdaSymbol{:} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaInductiveConstructor{|1|} \<[71]%
\>[71]\AgdaInductiveConstructor{tt}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accE} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{A} \AgdaSymbol{:} \AgdaPrimitiveType{Set}\AgdaSymbol{\}\{}\AgdaBound{a} \AgdaSymbol{:} \AgdaBound{A}\AgdaSymbol{\}} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|E|} \AgdaBound{A}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaBound{a}\<%
\\
\>[2]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accEf} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}} \<[37]%
\>[37]\<%
\\
\>[4]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{→} \AgdaFunction{Accμ} \AgdaBound{e} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|Ef|} \AgdaBound{H}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accR} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaFunction{Accμ} \AgdaBound{e} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \<[71]%
\>[71]\AgdaBound{e}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{acc+₁} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaBound{G₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G₁} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{→} \<[17]%
\>[17]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{e} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{acc+₂} \<[11]%
\>[11]\AgdaSymbol{:} \<[14]%
\>[14]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaBound{G₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G₂} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{14}{}\<[14]%
\>[14]\AgdaSymbol{→} \<[17]%
\>[17]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G₂} \AgdaBound{e} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accx} \<[10]%
\>[10]\AgdaSymbol{:} \<[13]%
\>[13]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaBound{G₂} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{e₁} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G₁} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{e₂} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G₂} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \<[16]%
\>[16]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G₁} \AgdaBound{e₁} \AgdaSymbol{→} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G₂} \AgdaBound{e₂} \<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaInductiveConstructor{accB} \<[10]%
\>[10]\AgdaSymbol{:} \<[13]%
\>[13]\AgdaSymbol{\{}\AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[4]\AgdaIndent{13}{}\<[13]%
\>[13]\AgdaSymbol{→} \<[16]%
\>[16]\AgdaSymbol{((}\AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[13]\AgdaIndent{48}{}\<[48]%
\>[48]\AgdaSymbol{→} \<[51]%
\>[51]\AgdaDatatype{AccF} \AgdaBound{F} \AgdaSymbol{(}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{)} \<[71]%
\>[71]\AgdaSymbol{(}\AgdaBound{x} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{Accμ} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{F} \AgdaSymbol{→} \AgdaPrimitiveType{Set}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaFunction{Accμ} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \AgdaSymbol{=} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{F} \AgdaBound{e}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Induction.WellFounded}\<%
\\
%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{))(}\AgdaBound{n} \AgdaSymbol{:} \AgdaDatatype{ℕ}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{Acc} \AgdaFunction{\_<′\_} \AgdaBound{n} \AgdaSymbol{→} \AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e} \AgdaDatatype{≡} \AgdaBound{n} \AgdaSymbol{→} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaBound{G} \AgdaBound{e}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaBound{e} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{accv}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaBound{e} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{acc1}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{accR} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{e} \AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaBound{e} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{accE}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{accEf} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaBound{e} \AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁} \AgdaBound{e}\AgdaSymbol{)} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{acc+₁} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{e} \AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂} \AgdaBound{e}\AgdaSymbol{)} \<[35]%
\>[35]\AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n} \AgdaSymbol{=} \AgdaInductiveConstructor{acc+₂} \<[57]%
\>[57]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{e} \AgdaBound{n} \AgdaBound{accn} \AgdaBound{|e|≡n}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{(}\AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{.(}\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁} \AgdaPrimitive{+} \AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂} \AgdaSymbol{)} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaInductiveConstructor{acc} \AgdaBound{f}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \<[79]%
\>[79]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{accx} \<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{e₁} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₁} \AgdaBound{e₁}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemman>0→m+1≤m+n} \AgdaSymbol{(}\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{e₂}\AgdaSymbol{)))} \AgdaInductiveConstructor{refl}\AgdaSymbol{)} \<[115]%
\>[115]\<%
\\
\>[2]\AgdaIndent{10}{}\<[10]%
\>[10]\AgdaSymbol{(}\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{e₂} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G₂} \AgdaBound{e₂}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmam>0→n+1≤m+n} \AgdaSymbol{(}\AgdaFunction{lemmasizeF>0} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{e₁}\AgdaSymbol{)))} \AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{accFNat} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{(}\AgdaBound{x} \<[29]%
\>[29]\AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{)} \<[35]%
\>[35]\AgdaSymbol{.(}\AgdaInductiveConstructor{suc} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{))} \<[66]%
\>[66]\AgdaSymbol{(}\AgdaInductiveConstructor{acc} \AgdaBound{f}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \<[79]%
\>[79]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaInductiveConstructor{accB} \AgdaSymbol{(λ} \AgdaBound{y} \AgdaSymbol{→} \AgdaFunction{accFNat} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{sizeF} \AgdaBound{G} \AgdaBound{e}\AgdaSymbol{)} \AgdaInductiveConstructor{≤′-refl}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapSize} \AgdaBound{F} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
%
\\
\>\AgdaKeyword{open} \AgdaKeyword{import} \AgdaModule{Induction.Nat}\<%
\\
%
\\
\>\AgdaFunction{accF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}(}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{AccF} \AgdaBound{F} \AgdaInductiveConstructor{|R|} \AgdaBound{e}\<%
\\
\>\AgdaFunction{accF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{e} \AgdaSymbol{=} \AgdaFunction{accFNat} \AgdaBound{e} \AgdaSymbol{(}\AgdaFunction{size} \AgdaBound{e}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{Induction.Nat.<-well-founded} \AgdaSymbol{(}\AgdaFunction{size} \AgdaBound{e}\AgdaSymbol{))} \AgdaInductiveConstructor{refl}\<%
\\
%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}}\<%
\\
\>[2]\AgdaIndent{5}{}\<[5]%
\>[5]\AgdaSymbol{\{}\AgdaBound{f} \<[9]%
\>[9]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaSymbol{(\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \<[19]%
\>[19]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{→} \<[5]%
\>[5]\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{f}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \<[61]%
\>[61]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{cong} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{))} \AgdaBound{prf}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \<[36]%
\>[36]\AgdaSymbol{\_\}} \<[57]%
\>[57]\AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \<[36]%
\>[36]\AgdaSymbol{\_\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₁} \AgdaBound{x₁}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \<[61]%
\>[61]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[49]%
\>[49]\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaBound{y₁}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \<[61]%
\>[61]\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[49]%
\>[49]\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \<[25]%
\>[25]\AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \<[17]%
\>[17]\AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₁}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[61]%
\>[61]\<%
\\
\>[2]\AgdaIndent{17}{}\<[17]%
\>[17]\AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₂}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \<[43]%
\>[43]\<%
\\
\>[17]\AgdaIndent{40}{}\<[40]%
\>[40]\AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \<[57]%
\>[57]\AgdaBound{prf} \AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[82]%
\>[82]\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<%
\end{code}

%<*swapfoldequiv>
\begin{code}%
\>\AgdaFunction{lemmaSwapFoldEquiv} \<[20]%
\>[20]\AgdaSymbol{:} \<[23]%
\>[23]\AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}\{}\AgdaBound{f} \<[28]%
\>[28]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{→} \<[6]%
\>[6]\AgdaSymbol{(\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}} \<[19]%
\>[19]\AgdaSymbol{\{}\AgdaBound{e} \<[23]%
\>[23]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \<[38]%
\>[38]\<%
\\
\>[3]\AgdaIndent{19}{}\<[19]%
\>[19]\AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{→} \<[6]%
\>[6]\AgdaFunction{fold} \AgdaBound{F} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{fold} \AgdaBound{F} \AgdaBound{f} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}
%</swapfoldequiv>

\begin{code}%
\>\AgdaFunction{lemmaSwapFoldEquiv} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaFunction{lemmaSwapFoldEquivF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf}\<%
\\
%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{:} \<[26]%
\>[26]\AgdaSymbol{\{}\AgdaBound{F} \AgdaBound{G} \AgdaBound{H} \AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{G} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{)\}\{}\AgdaBound{f} \<[83]%
\>[83]\AgdaSymbol{:} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{V} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[3]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{\{}\AgdaBound{g} \<[26]%
\>[26]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}}\<%
\\
\>[3]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{→} \AgdaSymbol{(\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \<[38]%
\>[38]\AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}} \AgdaSymbol{→} \AgdaBound{f} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{g} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[3]\AgdaIndent{22}{}\<[22]%
\>[22]\AgdaSymbol{→} \AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swapF} \AgdaBound{G} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{G} \AgdaBound{g} \AgdaBound{e}\AgdaSymbol{)}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|v|} \AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|1|}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|R|}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{x} \AgdaSymbol{=} \AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{f}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaFunction{trans} \AgdaSymbol{(}\AgdaFunction{cong} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{x} \AgdaBound{y}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{))} \AgdaBound{prf}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|E|} \AgdaBound{x}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaArgument{G} \AgdaSymbol{=} \AgdaInductiveConstructor{|Ef|} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaInductiveConstructor{refl}\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₁} \AgdaBound{x₁}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₁} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[108]%
\>[108]\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|+|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaInductiveConstructor{inj₂} \AgdaBound{y₁}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=} \AgdaFunction{cong} \AgdaInductiveConstructor{inj₂} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[108]%
\>[108]\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁} \AgdaInductiveConstructor{|x|} \AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₁} \AgdaInductiveConstructor{,} \AgdaBound{e₂}\AgdaSymbol{\}} \AgdaBound{prf}\<%
\\
\>[0]\AgdaIndent{2}{}\<[2]%
\>[2]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₁}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e₂}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[110]%
\>[110]\<%
\\
\>\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{|B|} \AgdaBound{S} \AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{S} \AgdaSymbol{=} \AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{z} \AgdaInductiveConstructor{,} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaKeyword{with} \AgdaBound{S} \AgdaFunction{≟S} \AgdaBound{S'}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{yes} \AgdaSymbol{\_} \AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{S} \AgdaSymbol{=} \AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)}\<%
\\
\>\AgdaSymbol{...} \AgdaSymbol{|} \AgdaInductiveConstructor{no} \AgdaSymbol{\_} \<[12]%
\>[12]\AgdaSymbol{=} \AgdaFunction{cong₂} \AgdaSymbol{(}\AgdaInductiveConstructor{\_,\_}\AgdaSymbol{)} \AgdaInductiveConstructor{refl} \AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{S} \AgdaSymbol{=} \AgdaBound{S'}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaArgument{e} \AgdaSymbol{=} \AgdaBound{e}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)}\<%
\end{code}

-- lemmaSwapFoldSEquivF :  {C H F G : Functor}{S : Sort}{x y : V}
--    {e : ⟦ G ⟧ (μ F)}{f  : μ C → ⟦ F ⟧ (μ H) → μ H}{c : μ C}
--    → ({x y : V}{e  : ⟦ F ⟧ (μ H)} → f (swap {C} S x y c) (swapF F S x y e) ≡ swap {H} S x y (f c e))
--    → foldmapCtx F G f (swap {C} S x y c) (swapF G S x y e) ≡ swapF G S x y (foldmapCtx F G f c e)
-- lemmaSwapFoldSEquivF {G = |v| x} prf = refl
-- lemmaSwapFoldSEquivF {G = |1|} prf =  refl
-- lemmaSwapFoldSEquivF {C} {H} {F} {|R|} {S} {x} {y} {⟨ e ⟩} {f} {c} prf
--   =  begin≡
--        f (swap {C} S x y c) (foldmapCtx F F f (swap {C} S x y c) (swapF F S x y e))
--      ≡⟨ cong (f (swap {C} S x y c)) (lemmaSwapFoldSEquivF {C} {H} {F} {F} {S} {x} {y} {e} {f} {c} prf) ⟩
--        f (swap {C} S x y c) (swapF F S x y (foldmapCtx F F f c e))
--      ≡⟨ prf ⟩
--        swapF |R| S x y (f c (foldmapCtx F F f c e))
--      ■
-- lemmaSwapFoldSEquivF {G = |E| x} prf =  refl
-- lemmaSwapFoldSEquivF {G = |Ef| G} {e = ⟨ e ⟩} prf =  refl
-- lemmaSwapFoldSEquivF {G = G |+| G₁} {e = inj₁ e} prf = cong inj₁ (lemmaSwapFoldSEquivF {G = G } {e = e} prf)
-- lemmaSwapFoldSEquivF {G = G |+| G₁} {e = inj₂ e} prf = cong inj₂ (lemmaSwapFoldSEquivF {G = G₁ } {e = e} prf)
-- lemmaSwapFoldSEquivF {G = G |x| G₁} {e = e , e₁} prf
--   = cong₂ (_,_) (lemmaSwapFoldSEquivF {G = G} {e = e} prf) (lemmaSwapFoldSEquivF {G = G₁} {e = e₁} prf)
-- lemmaSwapFoldSEquivF {G = |B| S G} {S = S'} {e = z , e} prf with S ≟S S'
-- ... | yes _ = cong₂ (_,_) refl (lemmaSwapFoldSEquivF {G = G} {S = S'} {e = e} prf) 
-- ... | no _ = cong₂ (_,_) refl (lemmaSwapFoldSEquivF {G = G} {S = S'} {e = e} prf) 


%<*swapfoldCtx>
\begin{code}%
\>\AgdaFunction{lemmaSwapFoldCtxEquiv} \AgdaSymbol{:} \AgdaSymbol{\{}\AgdaBound{C} \AgdaBound{H} \AgdaBound{F} \<[32]%
\>[32]\AgdaSymbol{:} \AgdaDatatype{Functor}\AgdaSymbol{\}\{}\AgdaBound{S} \AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}}\<%
\\
\>[2]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaSymbol{\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{F}\AgdaSymbol{\}\{}\AgdaBound{f} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C} \AgdaSymbol{→} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)} \AgdaSymbol{→} \AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{\}\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{→} \<[6]%
\>[6]\AgdaSymbol{(\{}\AgdaBound{c} \AgdaSymbol{:} \AgdaDatatype{μ} \AgdaBound{C}\AgdaSymbol{\}\{}\AgdaBound{S} \<[20]%
\>[20]\AgdaSymbol{:} \AgdaFunction{Sort}\AgdaSymbol{\}\{}\AgdaBound{x} \AgdaBound{y} \AgdaSymbol{:} \AgdaFunction{V}\AgdaSymbol{\}\{}\AgdaBound{e} \AgdaSymbol{:} \AgdaFunction{⟦} \AgdaBound{F} \AgdaFunction{⟧} \AgdaSymbol{(}\AgdaDatatype{μ} \AgdaBound{H}\AgdaSymbol{)\}}\<%
\\
\>[3]\AgdaIndent{20}{}\<[20]%
\>[20]\AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaSymbol{→} \<[6]%
\>[6]\AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{)} \AgdaDatatype{≡} \AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaBound{e}\AgdaSymbol{)}\<%
\end{code}
%</swapfoldCtx>

%<*swapfoldCtxproof>
\begin{code}%
\>\AgdaFunction{lemmaSwapFoldCtxEquiv} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{f}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{prf} \AgdaSymbol{=}\<%
\\
\>[3]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{begin≡}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaInductiveConstructor{refl} \<[66]%
\>[66]\AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaBound{f} \<[9]%
\>[9]\AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \<[28]%
\>[28]\<%
\\
\>[6]\AgdaIndent{9}{}\<[9]%
\>[9]\AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaInductiveConstructor{|R|} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{))} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{3}{}\<[3]%
\>[3]\AgdaFunction{≡⟨} \AgdaFunction{cong} \<[12]%
\>[12]\AgdaSymbol{(}\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{))} \<[35]%
\>[35]\<%
\\
\>[3]\AgdaIndent{12}{}\<[12]%
\>[12]\AgdaSymbol{(}\AgdaFunction{lemmaSwapFoldEquivCtxF} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{F}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{S}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}} \AgdaSymbol{\{}\AgdaBound{e}\AgdaSymbol{\}} \<[64]%
\>[64]\<%
\\
\>[12]\AgdaIndent{21}{}\<[21]%
\>[21]\AgdaSymbol{\{λ} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{→} \AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)\}} \AgdaSymbol{\{}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{\}} \AgdaBound{prf}\AgdaSymbol{)} \<[66]%
\>[66]\AgdaFunction{⟩}\<%
\\
\>[0]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaBound{f} \AgdaSymbol{(}\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{C}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaBound{c}\AgdaSymbol{)} \AgdaSymbol{(}\AgdaFunction{swapF} \AgdaBound{F} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{foldmap} \AgdaBound{F} \AgdaBound{F} \AgdaSymbol{(}\AgdaBound{f} \AgdaBound{c}\AgdaSymbol{)} \AgdaBound{e}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{≡⟨} \AgdaBound{prf} \<[66]%
\>[66]\AgdaFunction{⟩}\<%
\\
\>[4]\AgdaIndent{6}{}\<[6]%
\>[6]\AgdaFunction{swap} \AgdaSymbol{\{}\AgdaBound{H}\AgdaSymbol{\}} \AgdaBound{S} \AgdaBound{x} \AgdaBound{y} \AgdaSymbol{(}\AgdaFunction{foldCtx} \AgdaBound{F} \AgdaBound{f} \AgdaBound{c} \AgdaInductiveConstructor{⟨} \AgdaBound{e} \AgdaInductiveConstructor{⟩}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaIndent{4}{}\<[4]%
\>[4]\AgdaFunction{■}\<%
\end{code}
%</swapfoldCtxproof>

-- \begin{code}%
\>\AgdaComment{-- --lemmaSwapFoldSEquiv \{C\} \{H\} \{F\} \{S\} \{x\} \{y\} \{⟨ e ⟩\} \{f\} \{c\} prf}\<%
\\
\>\AgdaComment{-- -- begin≡}\<%
\\
\>\AgdaComment{-- --       foldCtx F f (swap \{C\} S x y c) (swap \{F\} S x y ⟨ e ⟩)}\<%
\\
\>\AgdaComment{-- --     ≡⟨ refl ⟩}\<%
\\
\>\AgdaComment{-- --       f (swap \{C\} S x y c) (foldmapCtx F F f (swapF |R| S x y c) (swapF F S x y e))}\<%
\\
\>\AgdaComment{-- --     ≡⟨ cong (f (swap \{C\} S x y c)) (lemmaSwapFoldSEquivF \{C\} \{H\} \{F\} \{F\} \{S\} \{x\} \{y\} \{e\} \{f\} \{c\} prf) ⟩}\<%
\\
\>\AgdaComment{-- --       f (swap \{C\} S x y c) (swapF F S x y (foldmapCtx F F f c e))}\<%
\\
\>\AgdaComment{-- --     ≡⟨ prf ⟩}\<%
\\
\>\AgdaComment{-- --       swap \{H\} S x y (foldCtx F f c ⟨ e ⟩)}\<%
\\
\>\AgdaComment{-- --     ■}\<%
\\
\>\AgdaComment{-- }\<%
\end{code}



==> eptcsdata.tex <==
\providecommand{\firstpage}{11}
\providecommand{\publicationstatus}{F. Blanqui and G. Reis (Eds.): LFMTP'18\\
EPTCS 274, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.274.2}{10.4204/EPTCS.274.2}}
\pdfoutput=1

